RESOLVE and ECO: Finding Low-Metallicity $z\sim0$ Dwarf AGN Candidates Using Optimized Emission-Line Diagnostics

Existing star-forming vs. active galactic nucleus (AGN) classification schemes using optical emission-line diagnostics mostly fail for low-metallicity and/or highly star-forming galaxies, missing AGN in typical $z\sim0$ dwarfs. To recover AGN in dwarfs with strong emission lines (SELs), we present a classification scheme optimizing the use of existing optical diagnostics. We use SDSS emission-line catalogs overlapping the volume- and mass-limited RESOLVE and ECO surveys to determine the AGN percentage in SEL dwarfs. Our photoionization grids show that the [O III]/H$\beta$ versus [S II]/H$\alpha$ diagram (SII plot) and [O III]/H$\beta$ versus [O I]/H$\alpha$ diagram (OI plot) are less metallicity sensitive and more successful in identifying dwarf AGN than the popular [O III]/H$\beta$ versus [N II]/H$\alpha$ diagnostic (NII plot or "BPT diagram"). We identify a new category of "star-forming AGN" (SF-AGN) classified as star-forming by the NII plot but as AGN by the SII and/or OI plots. Including SF-AGN, we find the $z\sim0$ AGN percentage in dwarfs with SELs to be $\sim$3-16\%, far exceeding most previous optical estimates ($\sim$1\%). The large range in our dwarf AGN percentage reflects differences in spectral fitting methodologies between catalogs. The highly complete nature of RESOLVE and ECO allows us to normalize strong emission-line galaxy statistics to the full galaxy population, reducing the dwarf AGN percentage to $\sim$0.6-3.0\%. The newly identified SF-AGN are mostly gas-rich dwarfs with halo mass $ < 10^{11.5} M_\odot$, where highly efficient cosmic gas accretion is expected. Almost all SF-AGN also have low metallicities (Z $\lesssim 0.4$ Z$_\odot$), demonstrating the advantage of our method.

==> References.tex <==
@article{Richardson22,
	doi = {10.3847/1538-4357/ac510c},
	url = {https://doi.org/10.3847/1538-4357/ac510c},
	year = 2022,
	month = {mar},
	publisher = {American Astronomical Society},
	volume = {927},
	number = {2},
	pages = {165},
	author = {Chris T. Richardson and Connor Simpson and Mugdha S. Polimera and Sheila J. Kannappan and Jillian M. Bellovary and Christopher Greene and Sam Jenkins},
	title = {Optical and {JWST} Mid-{IR} Emission Line Diagnostics for Simultaneous {IMBH} and Stellar Excitation in z $\sim$ 0 Dwarf Galaxies{\ast}},
	journal = {The Astrophysical Journal},
	abstract = {Current observational facilities have yet to conclusively detect 103–104 M ⊙ intermediate-mass black holes (IMBHs) that fill in the evolutionary gap between seed black holes in the early universe and z ∼ 0 supermassive black holes. Dwarf galaxies present an opportunity to reveal active IMBHs amidst persistent star formation. We introduce photoionization simulations tailored to address key physical uncertainties: coincident versus noncoincident mixing of IMBH and starlight excitation, open versus closed geometries of surrounding gas clouds, and different shapes of the spectral energy distribution of active galactic nuclei (AGN). We examine possible AGN emission line diagnostics in the optical and mid-IR, and find that the diagnostics are often degenerate with respect to the investigated physical uncertainties. In spite of these setbacks, and in contrast to recent work, we are able to show that [O iii]/Hβ typically remains bright for dwarf AGN powered by IMBHs down to 103 M ⊙. Dwarf AGN are predicted to have inconsistent star-forming and Seyfert/LINER classifications using the most common optical diagnostics. In the mid-IR, [O iv] 25.9 μm and [Ar ii] 6.98 μm are less sensitive to physical uncertainties than are optical diagnostics. Based on these emission lines, we provide several diagrams of mid-IR emission line diagnostic diagrams with demarcations for separating starbursts and AGN with varying levels of activity. The diagrams are valid over a wide range of ionization parameters and metallicities out to z ∼ 0.1, so will prove useful for future JWST observations of local dwarf AGN in the search for IMBHs. We make our photoionization simulation suite freely available.}
}

@ARTICLE{Ferland86,
       author = {{Ferland}, G.~J. and {Osterbrock}, D.~E.},
        title = "{IUE Spectra and a Resulting Model of Seyfert 2 Galaxies}",
      journal = {\apj},
     keywords = {Iue, Seyfert Galaxies, Ultraviolet Astronomy, Chemical Composition, Continuous Spectra, Emission Spectra, H Lines, Lyman Spectra, Nonthermal Radiation, Photoionization, Ultraviolet Spectra, X Ray Spectra, Astrophysics, GALAXIES: SEYFERT, ULTRAVIOLET: SPECTRA},
         year = 1986,
        month = jan,
       volume = {300},
        pages = {658},
          doi = {10.1086/163841},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1986ApJ...300..658F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Haidar22,
       author = {{Haidar}, Houda and {Habouzit}, M{\'e}lanie and {Volonteri}, Marta and {Mezcua}, Mar and {Greene}, Jenny and {Neumayer}, Nadine and {Angl{\'e}s-Alc{\'a}zar}, Daniel and {Martin-Navarro}, Ignacio and {Hoyer}, Nils and {Dubois}, Yohan and {Dav{\'e}}, Romeel},
        title = "{The black hole population in low-mass galaxies in large-scale cosmological simulations}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = jan,
          eid = {arXiv:2201.09888},
        pages = {arXiv:2201.09888},
archivePrefix = {arXiv},
       eprint = {2201.09888},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220109888H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jarrett13,
       author = {{Jarrett}, T.~H. and {Masci}, F. and {Tsai}, C.~W. and {Petty}, S. and {Cluver}, M.~E. and {Assef}, Roberto J. and {Benford}, D. and {Blain}, A. and {Bridge}, C. and {Donoso}, E. and {Eisenhardt}, P. and {Koribalski}, B. and {Lake}, S. and {Neill}, James D. and {Seibert}, M. and {Sheth}, K. and {Stanford}, S. and {Wright}, E.},
        title = "{Extending the Nearby Galaxy Heritage with WISE: First Results from the WISE Enhanced Resolution Galaxy Atlas}",
      journal = {\aj},
     keywords = {galaxies: fundamental parameters, galaxies: statistics, infrared: galaxies, surveys, techniques: image processing, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = jan,
       volume = {145},
       number = {1},
          eid = {6},
        pages = {6},
          doi = {10.1088/0004-6256/145/1/6},
archivePrefix = {arXiv},
       eprint = {1210.3628},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013AJ....145....6J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kacharov18,
       author = {{Kacharov}, Nikolay and {Neumayer}, Nadine and {Seth}, Anil C. and {Cappellari}, Michele and {McDermid}, Richard and {Walcher}, C. Jakob and {B{\"o}ker}, Torsten},
        title = "{Stellar populations and star formation histories of the nuclear star clusters in six nearby galaxies}",
      journal = {\mnras},
     keywords = {techniques: spectroscopic, galaxies: individual: NGC 247, NGC 300, NGC 3621, NGC 5102, NGC 5206, NGC 7793, galaxies: nuclei, galaxies: star formation, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = oct,
       volume = {480},
       number = {2},
        pages = {1973-1998},
          doi = {10.1093/mnras/sty1985},
archivePrefix = {arXiv},
       eprint = {1807.08765},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.480.1973K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Boker04,
       author = {{B{\"o}ker}, Torsten and {Sarzi}, Marc and {McLaughlin}, Dean E. and {van der Marel}, Roeland P. and {Rix}, Hans-Walter and {Ho}, Luis C. and {Shields}, Joseph C.},
        title = "{A Hubble Space Telescope Census of Nuclear Star Clusters in Late-Type Spiral Galaxies. II. Cluster Sizes and Structural Parameter Correlations}",
      journal = {\aj},
     keywords = {Galaxies: Nuclei, Galaxies: Spiral, Galaxies: Star Clusters, Astrophysics},
         year = 2004,
        month = jan,
       volume = {127},
       number = {1},
        pages = {105-118},
          doi = {10.1086/380231},
archivePrefix = {arXiv},
       eprint = {astro-ph/0309761},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004AJ....127..105B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lee09,
       author = {{Lee}, Janice C. and {Gil de Paz}, Armando and {Tremonti}, Christy and {Kennicutt}, Robert C., Jr. and {Salim}, Samir and {Bothwell}, Matthew and {Calzetti}, Daniela and {Dalcanton}, Julianne and {Dale}, Daniel and {Engelbracht}, Chad and {Funes}, S.~J. Jos{\'e} G. and {Johnson}, Benjamin and {Sakai}, Shoko and {Skillman}, Evan and {van Zee}, Liese and {Walter}, Fabian and {Weisz}, Daniel},
        title = "{Comparison of H{\ensuremath{\alpha}} and UV Star Formation Rates in the Local Volume: Systematic Discrepancies for Dwarf Galaxies}",
      journal = {\apj},
     keywords = {galaxies: dwarf, galaxies: evolution, galaxies: photometry, stars: formation, surveys, ultraviolet: galaxies, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2009,
        month = nov,
       volume = {706},
       number = {1},
        pages = {599-613},
          doi = {10.1088/0004-637X/706/1/599},
archivePrefix = {arXiv},
       eprint = {0909.5205},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...706..599L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Salim16,
       author = {{Salim}, Samir and {Lee}, Janice C. and {Janowiecki}, Steven and {da Cunha}, Elisabete and {Dickinson}, Mark and {Boquien}, M{\'e}d{\'e}ric and {Burgarella}, Denis and {Salzer}, John J. and {Charlot}, St{\'e}phane},
        title = "{GALEX-SDSS-WISE Legacy Catalog (GSWLC): Star Formation Rates, Stellar Masses, and Dust Attenuations of 700,000 Low-redshift Galaxies}",
      journal = {\apjs},
     keywords = {galaxies: fundamental parameters, galaxies: star formation, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = nov,
       volume = {227},
       number = {1},
          eid = {2},
        pages = {2},
          doi = {10.3847/0067-0049/227/1/2},
archivePrefix = {arXiv},
       eprint = {1610.00712},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJS..227....2S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Simmonds21,
       author = {{Simmonds}, Charlotte and {Schaerer}, Daniel and {Verhamme}, Anne},
        title = "{Can nebular HeII emission be explained by ultra-luminous X-ray sources?}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = aug,
          eid = {arXiv:2108.12438},
        pages = {arXiv:2108.12438},
archivePrefix = {arXiv},
       eprint = {2108.12438},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210812438S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{Sarzi17,
       author = {{Sarzi}, Marc and {Falc{\'o}n-Barroso}, Jes{\'u}s and {Davies}, Roger L. and {Bacon}, Roland and {Bureau}, Martin and {Cappellari}, Michele and {de Zeeuw}, P. Tim and {Emsellem}, Eric and {Fathi}, Kambiz and {Krajnovi{\"A}}, Davor and {Kuntschner}, Harald and {McDermid}, Richard M. and {Peletier}, Reynier F.},
        title = "{GANDALF: Gas AND Absorption Line Fitting}",
     keywords = {Software},
         year = 2017,
        month = aug,
          eid = {ascl:1708.012},
        pages = {ascl:1708.012},
archivePrefix = {ascl},
       eprint = {1708.012},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ascl.soft08012S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Cappellari04,
       author = {{Cappellari}, Michele and {Emsellem}, Eric},
        title = "{Parametric Recovery of Line-of-Sight Velocity Distributions from Absorption-Line Spectra of Galaxies via Penalized Likelihood}",
      journal = {\pasp},
     keywords = {Galaxies: Individual: NGC Number: NGC 3384, Galaxies: Kinematics and Dynamics, line: profiles, Methods: Numerical, Astrophysics},
         year = 2004,
        month = feb,
       volume = {116},
       number = {816},
        pages = {138-147},
          doi = {10.1086/381875},
archivePrefix = {arXiv},
       eprint = {astro-ph/0312201},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004PASP..116..138C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lin17,
       author = {{Lin}, Lin and {Li}, Cheng and {He}, Yanqin and {Xiao}, Ting and {Wang}, Enci},
        title = "{Bar-induced Central Star Formation as Revealed by Integral Field Spectroscopy from CALIFA}",
      journal = {\apj},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: spiral, galaxies: stellar content, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = apr,
       volume = {838},
       number = {2},
          eid = {105},
        pages = {105},
          doi = {10.3847/1538-4357/aa657a},
archivePrefix = {arXiv},
       eprint = {1609.05287},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...838..105L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wang12,
       author = {{Wang}, Jing and {Kauffmann}, Guinevere and {Overzier}, Roderik and {Tacconi}, Linda J. and {Kong}, Xu and {Saintonge}, Amelie and {Catinella}, Barbara and {Schiminovich}, David and {Moran}, Sean M. and {Johnson}, Benjamin},
        title = "{Quantifying the role of bars in the build-up of central mass concentrations in disc galaxies}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: structure, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2012,
        month = jul,
       volume = {423},
       number = {4},
        pages = {3486-3501},
          doi = {10.1111/j.1365-2966.2012.21147.x},
archivePrefix = {arXiv},
       eprint = {1205.0932},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.423.3486W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tacchella16,
       author = {{Tacchella}, Sandro and {Dekel}, Avishai and {Carollo}, C. Marcella and {Ceverino}, Daniel and {DeGraf}, Colin and {Lapiner}, Sharon and {Mandelker}, Nir and {Primack}, Joel R.},
        title = "{Evolution of density profiles in high-z galaxies: compaction and quenching inside-out}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: high-redshift, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = may,
       volume = {458},
       number = {1},
        pages = {242-263},
          doi = {10.1093/mnras/stw303},
archivePrefix = {arXiv},
       eprint = {1509.00017},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.458..242T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zolotov15,
       author = {{Zolotov}, Adi and {Dekel}, Avishai and {Mandelker}, Nir and {Tweed}, Dylan and {Inoue}, Shigeki and {DeGraf}, Colin and {Ceverino}, Daniel and {Primack}, Joel R. and {Barro}, Guillermo and {Faber}, Sandra M.},
        title = "{Compaction and quenching of high-z galaxies in cosmological simulations: blue and red nuggets}",
      journal = {\mnras},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: kinematics and dynamics, galaxies: spiral, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = jul,
       volume = {450},
       number = {3},
        pages = {2327-2353},
          doi = {10.1093/mnras/stv740},
archivePrefix = {arXiv},
       eprint = {1412.4783},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.450.2327Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dekel14,
       author = {{Dekel}, A. and {Burkert}, A.},
        title = "{Wet disc contraction to galactic blue nuggets and quenching to red nuggets}",
      journal = {\mnras},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: kinematics and dynamics, galaxies: spiral, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = feb,
       volume = {438},
       number = {2},
        pages = {1870-1879},
          doi = {10.1093/mnras/stt2331},
archivePrefix = {arXiv},
       eprint = {1310.1074},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.438.1870D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Thomas19,
       author = {{Thomas}, Adam D. and {Kewley}, Lisa J. and {Dopita}, Michael A. and {Groves}, Brent A. and {Hopkins}, Andrew M. and {Sutherland}, Ralph S.},
        title = "{The Mass-Metallicity Relation of Local Active Galaxies}",
      journal = {\apj},
     keywords = {galaxies: abundances, galaxies: active, galaxies: ISM, galaxies: Seyfert, quasars: emission lines, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = mar,
       volume = {874},
       number = {1},
          eid = {100},
        pages = {100},
          doi = {10.3847/1538-4357/ab08a1},
archivePrefix = {arXiv},
       eprint = {1902.06368},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...874..100T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Croton06,
       author = {{Croton}, Darren J. and {Springel}, Volker and {White}, Simon D.~M. and {De Lucia}, G. and {Frenk}, C.~S. and {Gao}, L. and {Jenkins}, A. and {Kauffmann}, G. and {Navarro}, J.~F. and {Yoshida}, N.},
        title = "{The many lives of active galactic nuclei: cooling flows, black holes and the luminosities and colours of galaxies}",
      journal = {\mnras},
     keywords = {black hole physics, galaxies: active, cooling flows, galaxies: evolution, galaxies: formation, cosmology: theory, Astrophysics},
         year = 2006,
        month = jan,
       volume = {365},
       number = {1},
        pages = {11-28},
          doi = {10.1111/j.1365-2966.2005.09675.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0508046},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MNRAS.365...11C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DiMatteo05,
       author = {{Di Matteo}, Tiziana and {Springel}, Volker and {Hernquist}, Lars},
        title = "{Energy input from quasars regulates the growth and activity of black holes and their host galaxies}",
      journal = {\nat},
     keywords = {Astrophysics},
         year = 2005,
        month = feb,
       volume = {433},
       number = {7026},
        pages = {604-607},
          doi = {10.1038/nature03335},
archivePrefix = {arXiv},
       eprint = {astro-ph/0502199},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005Natur.433..604D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Silk98,
       author = {{Silk}, Joseph and {Rees}, Martin J.},
        title = "{Quasars and galaxy formation}",
      journal = {\aap},
     keywords = {GALAXY FORMATION: SUPERMASSIVE BLACK HOLES, QUASARS: OUTFLOWS, Astrophysics},
         year = 1998,
        month = mar,
       volume = {331},
        pages = {L1-L4},
archivePrefix = {arXiv},
       eprint = {astro-ph/9801013},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998A&A...331L...1S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Allen08,
       author = {{Allen}, Mark G. and {Groves}, Brent A. and {Dopita}, Michael A. and {Sutherland}, Ralph S. and {Kewley}, Lisa J.},
        title = "{The MAPPINGS III Library of Fast Radiative Shock Models}",
      journal = {\apjs},
     keywords = {galaxies: nuclei, galaxies: Seyfert, hydrodynamics, infrared: ISM, ISM: abundances, shock waves, ultraviolet: ISM, X-rays: ISM, Astrophysics},
         year = 2008,
        month = sep,
       volume = {178},
       number = {1},
        pages = {20-55},
          doi = {10.1086/589652},
archivePrefix = {arXiv},
       eprint = {0805.0204},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJS..178...20A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bellovary21,
       author = {{Bellovary}, Jillian M. and {Hayoune}, Sarra and {Chafla}, Katheryn and {Vincent}, Donovan and {Brooks}, Alyson and {Christensen}, Charlotte and {Munshi}, Ferah and {Tremmel}, Michael and {Quinn}, Thomas R. and {Van Nest}, Jordan and {Sligh}, Serena K. and {Luzuriaga}, Michelle},
        title = "{The Origins of Off-Center Massive Black Holes in Dwarf Galaxies}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2021,
        month = feb,
          eid = {arXiv:2102.09566},
        pages = {arXiv:2102.09566},
archivePrefix = {arXiv},
       eprint = {2102.09566},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210209566B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@article{Ho97,
	doi = {10.1086/304638},
	url = {https://doi.org/10.1086/304638},
	year = 1997,
	month = {oct},
	publisher = {American Astronomical Society},
	volume = {487},
	number = {2},
	pages = {568--578},
	author = {Luis C. Ho and Alexei V. Filippenko and Wallace L. W. Sargent},
	title = {A Search for {\textquotedblleft}Dwarf{\textquotesingle}{\textquotesingle} Seyfert Nuclei. V. Demographics of Nuclear Activity in Nearby Galaxies},
	journal = {The Astrophysical Journal},
	abstract = {We use the sample of emission-line nuclei derived from a recently completed optical spectroscopic survey of nearby galaxies to quantify the incidence of local (z ≈ 0) nuclear activity. Particular attention is paid to obtaining accurate measurements of the emission lines and reliable spectral classifications. The resulting database contains the largest collection of star-forming nuclei and active galactic nuclei (AGNs) currently known for nearby galaxies. It consists of 420 emission-line nuclei detected from a nearly complete, magnitude-limited sample of 486 galaxies with BT ≤ 12.5 mag and declination greater than 0°; the equivalent width detection limit of the brightest emission line, usually Hα, is ~0.25 Å.

As is consistent with previous studies, we find detectable amounts of ionized gas in the central few hundred parsecs of most galaxies (86%); emission lines are present in essentially every spiral galaxy and in a large fraction of ellipticals and lenticulars. Based on their narrow-line spectra, half of the objects can be classified as H II or star-forming nuclei and the other half as some form of AGN, of which we distinguish three classes: Seyfert nuclei, low-ionization nuclear emission-line regions (LINERs), and transition objects that we assume to be composite LINER/H II-nucleus systems. The population of AGNs is consequently very large; approximately 43% of the galaxies in our survey can be regarded as “active,” although, for a number of reasons, this fraction is still rather uncertain. Most of the objects have much lower luminosities than commonly studied AGNs; the median luminosity of the narrow Hα line, after correcting for extinction, is only 2 × 1039 ergs s-1. Our sample therefore occupies the extreme faint end of the AGN luminosity function.

We detect signatures of a broad-line region, as revealed by visible broad Hα emission, in ~20% of the AGN sample. Seyfert nuclei, both type 1 and type 2, reside in ~10% of all galaxies. LINERs make up the bulk (1/2-3/4) of the AGN population and a significant fraction (1/5-1/3) of all galaxies. A nonnegligible subset of LINERs emit broad Hα emission, furnishing direct evidence that a least some LINERs are indeed physically related to the AGN phenomenon.

The dominant ionization mechanism of the nuclear emission depends strongly on the morphological type and luminosity of the host galaxy. AGNs are found predominantly in luminous, early-type (E-Sbc) galaxies, while H II nuclei prefer less luminous, late-type (Sbc and later) systems. The various AGN subclasses have broadly similar host galaxies.}
}

@ARTICLE{Kauffmann03mass,
       author = {{Kauffmann}, Guinevere and {Heckman}, Timothy M. and {White}, Simon D.~M. and {Charlot}, St{\'e}phane and {Tremonti}, Christy and {Peng}, Eric W. and {Seibert}, Mark and {Brinkmann}, Jon and {Nichol}, Robert C. and {SubbaRao}, Mark and {York}, Don},
        title = "{The dependence of star formation history and internal structure on stellar mass for {}10$^{5}$ low-redshift galaxies}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, galaxies: stellar content, Astrophysics},
         year = 2003,
        month = may,
       volume = {341},
       number = {1},
        pages = {54-69},
          doi = {10.1046/j.1365-8711.2003.06292.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0205070},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003MNRAS.341...54K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dekel86,
       author = {{Dekel}, A. and {Silk}, J.},
        title = "{The Origin of Dwarf Galaxies, Cold Dark Matter, and Biased Galaxy Formation}",
      journal = {\apj},
     keywords = {Abundance, Cold Plasmas, Dark Matter, Dwarf Galaxies, Galactic Evolution, Stellar Winds, Virgo Galactic Cluster, Big Bang Cosmology, Galactic Structure, Local Group (Astronomy), Mass To Light Ratios, Stellar Evolution, Supernovae, Astrophysics, COSMOLOGY, GALAXIES: CLUSTERING, GALAXIES: FORMATION, GALAXIES: INTERNAL MOTIONS, GALAXIES: STRUCTURE},
         year = 1986,
        month = apr,
       volume = {303},
        pages = {39},
          doi = {10.1086/164050},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1986ApJ...303...39D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Stasinska06,
       author = {{Stasi{\'n}ska}, Gra{\.z}yna and {Cid Fernandes}, Roberto and {Mateus}, Ab{\'\i}lio and {Sodr{\'e}}, Laerte and {Asari}, Natalia V.},
        title = "{Semi-empirical analysis of Sloan Digital Sky Survey galaxies - III. How to distinguish AGN hosts}",
      journal = {\mnras},
     keywords = {galaxies: active: galaxies: starburst, galaxies: active, galaxies: starburst, Astrophysics},
         year = 2006,
        month = sep,
       volume = {371},
       number = {2},
        pages = {972-982},
          doi = {10.1111/j.1365-2966.2006.10732.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0606724},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MNRAS.371..972S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Molina21,
       author = {{Molina}, M. and {Reines}, A.~E. and {Greene}, J.~E. and {Darling}, J. and {Condon}, J.~J.},
        title = "{Outflows, Shocks and Coronal Line Emission in a Radio-Selected AGN in a Dwarf Galaxy}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = jan,
          eid = {arXiv:2101.12217},
        pages = {arXiv:2101.12217},
archivePrefix = {arXiv},
       eprint = {2101.12217},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210112217M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Hopkins02,
	doi = {10.1086/341584},
	url = {https://doi.org/10.1086/341584},
	year = 2002,
	month = {aug},
	publisher = {American Astronomical Society},
	volume = {124},
	number = {2},
	pages = {862--876},
	author = {A. M. Hopkins and R. E. Schulte-Ladbeck and I. O. Drozdovsky},
	title = {Star Formation Rates of Local Blue Compact Dwarf Galaxies. I. 1.4 {GH}[{CLC}]z[/{CLC}] and 60 Micron Luminosities},
	journal = {The Astronomical Journal},
	abstract = {We determine and examine the star formation rates of 50 well-known, local blue compact dwarf (BCD) galaxies based on their 1.4 GHz and 60 μm luminosities. We find that in cases for which both radio and far-infrared luminosities are available, the resulting star formation rates agree extremely well with one another. We determine that the star formation rates of the BCD galaxies in our sample span nearly 5 orders of magnitude, from approximately a few times 10-3 to several times 101 M⊙ yr-1, with a median SFR of about 0.3 M⊙ yr-1. We discuss trends of metallicity (primarily oxygen abundance) with star formation rate and explore the connections between SFR and galaxy mass estimates.}
}
@ARTICLE{Greene20,
       author = {{Greene}, Jenny E. and {Strader}, Jay and {Ho}, Luis C.},
        title = "{Intermediate-Mass Black Holes}",
      journal = {\araa},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = aug,
       volume = {58},
        pages = {257-312},
          doi = {10.1146/annurev-astro-032620-021835},
archivePrefix = {arXiv},
       eprint = {1911.09678},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ARA&A..58..257G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zaw19,
       author = {{Zaw}, Ingyin and {Chen}, Yan-Ping and {Farrar}, Glennys R.},
        title = "{A Uniformly Selected, All-sky, Optical AGN Catalog}",
      journal = {\apj},
     keywords = {catalogs, galaxies: active, line: identification, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = feb,
       volume = {872},
       number = {2},
          eid = {134},
        pages = {134},
          doi = {10.3847/1538-4357/aaffaf},
archivePrefix = {arXiv},
       eprint = {1902.03799},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...872..134Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chen18,
       author = {{Chen}, Yan-Ping and {Zaw}, Ingyin and {Farrar}, Glennys R.},
        title = "{Dependence of Optical Active Galactic Nuclei Identification on Stellar Population Models}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: nuclei, techniques: spectroscopic, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = jul,
       volume = {861},
       number = {1},
          eid = {67},
        pages = {67},
          doi = {10.3847/1538-4357/aac8e1},
archivePrefix = {arXiv},
       eprint = {1805.12373},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...861...67C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reichardt01,
       author = {{Reichardt}, Christian and {Jimenez}, Raul and {Heavens}, Alan F.},
        title = "{Recovering physical parameters from galaxy spectra using MOPED}",
      journal = {\mnras},
     keywords = {METHODS: DATA ANALYSIS, METHODS: STATISTICAL, GALAXIES: FUNDAMENTAL PARAMETERS, GALAXIES: STATISTICS, GALAXIES: STELLAR CONTENT, Astrophysics},
         year = 2001,
        month = nov,
       volume = {327},
       number = {3},
        pages = {849-867},
          doi = {10.1046/j.1365-8711.2001.04768.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0101074},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001MNRAS.327..849R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maraston11,
       author = {{Maraston}, C. and {Str{\"o}mb{\"a}ck}, G.},
        title = "{Stellar population models at high spectral resolution}",
      journal = {\mnras},
     keywords = {stars: evolution, stars: fundamental parameters, galaxies: stellar content, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = dec,
       volume = {418},
       number = {4},
        pages = {2785-2811},
          doi = {10.1111/j.1365-2966.2011.19738.x},
archivePrefix = {arXiv},
       eprint = {1109.0543},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.418.2785M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bruzual03,
       author = {{Bruzual}, G. and {Charlot}, S.},
        title = "{Stellar population synthesis at the resolution of 2003}",
      journal = {\mnras},
     keywords = {stars: evolution, galaxies: evolution, galaxies: formation, galaxies: stellar content, Astrophysics},
         year = 2003,
        month = oct,
       volume = {344},
       number = {4},
        pages = {1000-1028},
          doi = {10.1046/j.1365-8711.2003.06897.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0309134},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003MNRAS.344.1000B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brinchmann08,
       author = {{Brinchmann}, J. and {Kunth}, D. and {Durret}, F.},
        title = "{Galaxies with Wolf-Rayet signatures in the low-redshift Universe. A survey using the Sloan Digital Sky Survey}",
      journal = {\aap},
     keywords = {stars: Wolf-Rayet, galaxies: abundances, galaxies: evolution, galaxies: starburst, galaxies:, fundamental parameters, Astrophysics},
         year = 2008,
        month = jul,
       volume = {485},
       number = {3},
        pages = {657-677},
          doi = {10.1051/0004-6361:200809783},
archivePrefix = {arXiv},
       eprint = {0805.1073},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...485..657B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lehmer21,
       author = {{Lehmer}, Bret D. and {Eufrasio}, Rafael T. and {Basu-Zych}, Antara and {Doore}, Keith and {Fragos}, Tassos and {Garofali}, Kristen and {Kovlakas}, Konstantinos and {Williams}, Benjamin F. and {Zezas}, Andreas and {Santana-Silva}, Luidhy},
        title = "{The Metallicity Dependence of the High-mass X-Ray Binary Luminosity Function}",
      journal = {\apj},
     keywords = {High mass x-ray binary stars, Metallicity, Star formation, Spiral galaxies, X-ray binary stars, X-ray astronomy, Compact objects, 733, 1031, 1569, 1560, 1811, 1810, 288, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = jan,
       volume = {907},
       number = {1},
          eid = {17},
        pages = {17},
          doi = {10.3847/1538-4357/abcec1},
archivePrefix = {arXiv},
       eprint = {2011.09476},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...907...17L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Senchyna20,
       author = {{Senchyna}, Peter and {Stark}, Daniel P. and {Mirocha}, Jordan and {Reines}, Amy E. and {Charlot}, St{\'e}phane and {Jones}, Tucker and {Mulchaey}, John S.},
        title = "{High-mass X-ray binaries in nearby metal-poor galaxies: on the contribution to nebular He II emission}",
      journal = {\mnras},
     keywords = {galaxies: stellar content, X-rays: binaries, X-rays: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = may,
       volume = {494},
       number = {1},
        pages = {941-957},
          doi = {10.1093/mnras/staa586},
archivePrefix = {arXiv},
       eprint = {1909.10574},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.494..941S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Eckert17,
       author = {{Eckert}, Kathleen D. and {Kannappan}, Sheila J. and {Lagos}, Claudia del P. and {Baker}, Ashley D. and {Berlind}, Andreas A. and {Stark}, David V. and {Moffett}, Amanda J. and {Nasipak}, Zachary and {Norris}, Mark A.},
        title = "{The Baryonic Collapse Efficiency of Galaxy Groups in the RESOLVE and ECO Surveys}",
      journal = {\apj},
     keywords = {galaxies: halos, galaxies: luminosity function, mass function, surveys, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = nov,
       volume = {849},
       number = {1},
          eid = {20},
        pages = {20},
          doi = {10.3847/1538-4357/aa8e97},
archivePrefix = {arXiv},
       eprint = {1709.07462},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...849...20E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Buat11,
       author = {{Buat}, V. and {Giovannoli}, E. and {Heinis}, S. and {Charmandaris}, V. and {Coia}, D. and {Daddi}, E. and {Dickinson}, M. and {Elbaz}, D. and {Hwang}, H.~S. and {Morrison}, G. and {Dasyra}, K. and {Aussel}, H. and {Altieri}, B. and {Dannerbauer}, H. and {Kartaltepe}, J. and {Leiton}, R. and {Magdis}, G. and {Magnelli}, B. and {Popesso}, P.},
        title = "{GOODS-Herschel: evidence of a UV extinction bump in galaxies at z > 1}",
      journal = {\aap},
     keywords = {galaxies: high-redshift, galaxies: ISM, ultraviolet: galaxies, infrared: galaxies, dust, extinction, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = sep,
       volume = {533},
          eid = {A93},
        pages = {A93},
          doi = {10.1051/0004-6361/201117264},
archivePrefix = {arXiv},
       eprint = {1107.1049},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...533A..93B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{GildePaz03,
       author = {{Gil de Paz}, A. and {Madore}, B.~F. and {Pevunova}, O.},
        title = "{Palomar/Las Campanas Imaging Atlas of Blue Compact Dwarf Galaxies. I. Images and Integrated Photometry}",
      journal = {\apjs},
     keywords = {Atlases, Galaxies: Dwarf, Galaxies: Evolution, Galaxies: Fundamental Parameters, Galaxies: Photometry, Galaxies: Starburst, Astrophysics},
         year = 2003,
        month = jul,
       volume = {147},
       number = {1},
        pages = {29-59},
          doi = {10.1086/374737},
archivePrefix = {arXiv},
       eprint = {astro-ph/0302221},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJS..147...29G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Panda19,
       author = {{Panda}, Swayamtrupta and {Czerny}, Bo{\.z}ena and {Done}, Chris and {Kubota}, Aya},
        title = "{CLOUDY View of the Warm Corona}",
      journal = {\apj},
     keywords = {accretion, accretion disks, galaxies: active, quasars: emission lines, radiative transfer, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = apr,
       volume = {875},
       number = {2},
          eid = {133},
        pages = {133},
          doi = {10.3847/1538-4357/ab11cb},
archivePrefix = {arXiv},
       eprint = {1901.02962},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...875..133P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@misc{Vasiliev20,
      title={Far-infrared nebular spectral features from growing massive black holes}, 
      author={Evgenii O. Vasiliev and Yuri A. Shchekinov and Biman B. Nath},
      year={2020},
      eprint={2003.14036},
      archivePrefix={arXiv},
      primaryClass={astro-ph.GA}
}

@ARTICLE{Abel08,
       author = {{Abel}, N.~P. and {van Hoof}, P.~A.~M. and {Shaw}, G. and {Ferland
        }, G.~J. and {Elwert}, T.},
        title = "{Sensitivity of PDR Calculations to Microphysical Details}",
      journal = {\apj},
     keywords = {dust, extinction, infrared: ISM, ISM: lines and bands, ISM: molecules, ISM: structure, submillimeter, Astrophysics},
         year = 2008,
        month = oct,
       volume = {686},
       number = {2},
        pages = {1125-1136},
          doi = {10.1086/591505},
archivePrefix = {arXiv},
       eprint = {0808.2532},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...686.1125A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jenkins09,
       author = {{Jenkins}, Edward B.},
        title = "{A Unified Representation of Gas-Phase Element Depletions in the Interstellar Medium}",
      journal = {\apj},
     keywords = {ISM: abundances, ISM: atoms, ultraviolet: ISM, Astrophysics - Galaxy Astrophysics},
         year = 2009,
        month = aug,
       volume = {700},
       number = {2},
        pages = {1299-1348},
          doi = {10.1088/0004-637X/700/2/1299},
archivePrefix = {arXiv},
       eprint = {0905.3173},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...700.1299J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Baldwin91,
       author = {{Baldwin}, Jack A. and {Ferland}, Gary J. and {Martin}, P.~G. and
         {Corbin}, Michael R. and {Cota}, Stephen A. and {Peterson}, Bradley M. and
         {Slettebak}, Arne},
        title = "{Physical Conditions in the Orion Nebula and an Assessment of Its Helium Abundance}",
      journal = {\apj},
     keywords = {Abundance, H Ii Regions, Helium Ions, Orion Nebula, Hydrogen Ions, Photoionization, Spectrophotometry, Astrophysics, NEBULAE: ABUNDANCES, NEBULAE: H II REGIONS, NEBULAE: ORION NEBULA},
         year = 1991,
        month = jun,
       volume = {374},
        pages = {580},
          doi = {10.1086/170146},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1991ApJ...374..580B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kubota18,
       author = {{Kubota}, Aya and {Done}, Chris},
        title = "{A physical model of the broad-band continuum of AGN and its implications for the UV/X relation and optical variability}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, galaxies: Seyfert, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = oct,
       volume = {480},
       number = {1},
        pages = {1247-1262},
          doi = {10.1093/mnras/sty1890},
archivePrefix = {arXiv},
       eprint = {1804.00171},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.480.1247K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Liu19,
       author = {{Liu}, He-Yang and {Liu}, Wen-Juan and {Dong}, Xiao-Bo and
         {Zhou}, Hongyan and {Wang}, Tinggui and {Lu}, Honglin and
         {Yuan}, Weimin},
        title = "{A Comprehensive and Uniform Sample of Broad-line Active Galactic Nuclei from the SDSS DR7}",
      journal = {\apjs},
     keywords = {galaxies: active, galaxies: nuclei, galaxies: Seyfert, quasars: emission lines, surveys, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = aug,
       volume = {243},
       number = {2},
          eid = {21},
        pages = {21},
          doi = {10.3847/1538-4365/ab298b},
archivePrefix = {arXiv},
       eprint = {1906.05597},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJS..243...21L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Flesch15,
       author = {{Flesch}, Eric W.},
        title = "{The Half Million Quasars (HMQ) Catalogue}",
      journal = {\pasa},
     keywords = {catalogues, quasars: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2015,
        month = mar,
       volume = {32},
          eid = {e010},
        pages = {e010},
          doi = {10.1017/pasa.2015.10},
archivePrefix = {arXiv},
       eprint = {1502.06303},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015PASA...32...10F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Veron06,
       author = {{V{\'e}ron-Cetty}, M. -P. and {V{\'e}ron}, P.},
        title = "{A catalogue of quasars and active nuclei: 12th edition}",
      journal = {\aap},
     keywords = {galaxies: quasars: general, galaxies: Seyfert, galaxies: BL Lacertae objects: general},
         year = 2006,
        month = aug,
       volume = {455},
       number = {2},
        pages = {773-777},
          doi = {10.1051/0004-6361:20065177},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006A&A...455..773V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Yan11,
	doi = {10.1088/0004-6256/142/5/153},
	url = {https://doi.org/10.1088%2F0004-6256%2F142%2F5%2F153},
	year = 2011,
	month = {sep},
	publisher = {{IOP} Publishing},
	volume = {142},
	number = {5},
	pages = {153},
	author = {Renbin Yan},
	title = {{PRECISION} {SPECTROPHOTOMETRY} {AT} {THE} {LEVEL} {OF} 0.1{\%}},
	journal = {The Astronomical Journal},
	abstract = {Accurate relative spectrophotometry is critical for many science applications. Small wavelength-scale residuals in the flux calibration can significantly impact the measurements of weak emission and absorption features in the spectra. Using Sloan Digital Sky Survey data, we demonstrate that the average spectra of carefully selected red-sequence galaxies can be used as a spectroscopic standard to improve the relative spectrophotometry precision to 0.1% on small wavelength scales (from a few to hundreds of Angstroms). We achieve this precision by comparing stacked spectra across tiny redshift intervals. The redshift intervals must be small enough that any systematic stellar population evolution is minimized and is less than the spectrophotometric uncertainty. This purely empirical technique does not require any theoretical knowledge of true galaxy spectra. It can be applied to all large spectroscopic galaxy redshift surveys that sample a large number of galaxies in a uniform population.}
}
@ARTICLE{Grupe10,
       author = {{Grupe}, Dirk and {Komossa}, Stefanie and {Leighly}, Karen M. and
         {Page}, Kim L.},
        title = "{The Simultaneous Optical-to-X-Ray Spectral Energy Distribution of Soft X-Ray Selected Active Galactic Nuclei Observed by Swift}",
      journal = {\apjs},
     keywords = {galaxies: active, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2010,
        month = mar,
       volume = {187},
       number = {1},
        pages = {64-106},
          doi = {10.1088/0067-0049/187/1/64},
archivePrefix = {arXiv},
       eprint = {1001.3140},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJS..187...64G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{Peterson97,
       author = {{Peterson}, Bradley M.},
        title = "{An Introduction to Active Galactic Nuclei}",
         year = 1997,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997iagn.book.....P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{RemyRuyer14,
       author = {{R{\'e}my-Ruyer}, A. and {Madden}, S.~C. and {Galliano}, F. and
         {Galametz}, M. and {Takeuchi}, T.~T. and {Asano}, R.~S. and
         {Zhukovska}, S. and {Lebouteiller}, V. and {Cormier}, D. and
         {Jones}, A. and {Bocchio}, M. and {Baes}, M. and {Bendo}, G.~J. and
         {Boquien}, M. and {Boselli}, A. and {DeLooze}, I. and
         {Doublier-Pritchard}, V. and {Hughes}, T. and {Karczewski}, O. {\L}. and
         {Spinoglio}, L.},
        title = "{Gas-to-dust mass ratios in local galaxies over a 2 dex metallicity range}",
      journal = {\aap},
     keywords = {evolution, galaxies: dwarf, galaxies: evolution, galaxies: ISM, infrared: ISM, dust, extinction, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = mar,
       volume = {563},
          eid = {A31},
        pages = {A31},
          doi = {10.1051/0004-6361/201322803},
archivePrefix = {arXiv},
       eprint = {1312.3442},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...563A..31R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Concas19,
       author = {{Concas}, A. and {Popesso}, P. and {Brusa}, M. and {Mainieri}, V. and
         {Thomas}, D.},
        title = "{Two-face(s): ionized and neutral gas winds in the local Universe}",
      journal = {\aap},
     keywords = {ISM: jets and outflows, ISM: lines and bands, galaxies: general, galaxies: active, galaxies: ISM, galaxies: star formation},
         year = 2019,
        month = feb,
       volume = {622},
          eid = {A188},
        pages = {A188},
          doi = {10.1051/0004-6361/201732152},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...622A.188C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Izotov12,
       author = {{Izotov}, Y.~I. and {Thuan}, T.~X. and {Privon}, G.},
        title = "{The detection of [Ne V] emission in five blue compact dwarf galaxies}",
      journal = {\mnras},
     keywords = {ISM: abundances, H II regions, galaxies: abundances, galaxies: evolution, galaxies: formation, galaxies: irregular, galaxies: ISM, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2012,
        month = dec,
       volume = {427},
       number = {2},
        pages = {1229-1237},
          doi = {10.1111/j.1365-2966.20
          ..22051.x},
archivePrefix = {arXiv},
       eprint = {1209.5265},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.427.1229I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Richardson19,
       author = {{Richardson}, Chris T. and {Polimera}, Mugdha S. and
         {Kannappan}, Sheila J. and {Moffett}, Amanda J. and
         {Bittner}, Ashley S.},
        title = "{Addressing the [O III]/H{\ensuremath{\beta}} offset of dwarf galaxies in the RESOLVE survey}",
      journal = {\mnras},
     keywords = {galaxies: dwarf, galaxies: ISM, galaxies: starburst, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = jul,
       volume = {486},
       number = {3},
        pages = {3541-3549},
          doi = {10.1093/mnras/stz1085},
archivePrefix = {arXiv},
       eprint = {1904.05912},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.486.3541R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Stanway16,
       author = {{Stanway}, Elizabeth R. and {Eldridge}, J.~J. and {Becker}, George D.},
        title = "{Stellar population effects on the inferred photon density at reionization}",
      journal = {\mnras},
     keywords = {binaries: general, stars: evolution, galaxies: high-redshift, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2016,
        month = feb,
       volume = {456},
       number = {1},
        pages = {485-499},
          doi = {10.1093/mnras/stv2661},
archivePrefix = {arXiv},
       eprint = {1511.03268},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.456..485S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{LaMassa13,
       author = {{LaMassa}, Stephanie M. and {Urry}, C. Megan and {Cappelluti}, Nico and
         {Civano}, Francesca and {Ranalli}, Piero and {Glikman}, Eilat and
         {Treister}, Ezequiel and {Richards}, Gordon and {Ballantyne}, David and
         {Stern}, Daniel and {Comastri}, Andrea and {Cardamone}, Carie and
         {Schawinski}, Kevin and {B{\"o}hringer}, Hans and {Chon}, Gayoung and
         {Murray}, Stephen S. and {Green}, Paul and {Nandra}, Kirpal},
        title = "{Finding rare AGN: XMM-Newton and Chandra observations of SDSS Stripe 82}",
      journal = {\mnras},
     keywords = {catalogues, surveys, galaxies: active, quasars: general, quasars: supermassive black holes, X-rays: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = dec,
       volume = {436},
       number = {4},
        pages = {3581-3601},
          doi = {10.1093/mnras/stt1837},
archivePrefix = {arXiv},
       eprint = {1309.7048},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.436.3581L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Evans20,
       author = {{Evans}, I.~N. and {Primini}, F.~A. and {Miller}, J.~B. and
         {Evans}, J.~D. and {Allen}, C.~E. and {Anderson}, C.~S. and
         {Becker}, G. and {Budynkiewicz}, J.~A. and {Burke}, D. and
         {Chen}, J.~C. and {Civano}, F. and {D'Abrusco}, R. and {Doe}, S.~M. and
         {Fabbiano}, G. and {Martinez Galarza}, J. and {Gibbs}, D.~G., II and
         {Glotfelty}, K.~J. and {Graessle}, D.~E. and {Grier}, J.~D., Jr. and
         {Hain}, R.~M. and {Hall}, D.~M. and {Harbo}, P.~N. and {Houck}, J.~C. and
         {Lauer}, J.~L. and {Laurino}, O. and {Lee}, N.~P. and
         {McCollough}, M.~L. and {McDowell}, J.~C. and {McLaughlin}, W. and
         {Morgan}, D.~L. and {Mossman}, A.~E. and {Nguyen}, D.~T. and
         {Nichols}, J.~S. and {Nowak}, M.~A. and {Paxson}, C. and
         {Perdikeas}, M. and {Plummer}, D.~A. and {Rots}, A.~H. and
         {Siemiginowska}, A.~L. and {Sundheim}, B.~A. and {Thong}, S. and
         {Tibbetts}, M.~S. and {Van Stone}, D.~W. and {Winkelman}, S.~L. and
         {Zografou}, P.},
        title = "{The Chandra Source Catalog {\textemdash} A Billion X-ray Photons}",
    booktitle = {American Astronomical Society Meeting Abstracts},
         year = 2020,
       series = {American Astronomical Society Meeting Abstracts},
        month = jan,
          eid = {154.05},
        pages = {154.05},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020AAS...23515405E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rosen16,
       author = {{Rosen}, S.~R. and {Webb}, N.~A. and {Watson}, M.~G. and {Ballet}, J. and
         {Barret}, D. and {Braito}, V. and {Carrera}, F.~J. and
         {Ceballos}, M.~T. and {Coriat}, M. and {Della Ceca}, R. and
         {Denkinson}, G. and {Esquej}, P. and {Farrell}, S.~A. and
         {Freyberg}, M. and {Gris{\'e}}, F. and {Guillout}, P. and {Heil}, L. and
         {Koliopanos}, F. and {Law-Green}, D. and {Lamer}, G. and {Lin}, D. and
         {Martino}, R. and {Michel}, L. and {Motch}, C. and
         {Nebot Gomez-Moran}, A. and {Page}, C.~G. and {Page}, K. and
         {Page}, M. and {Pakull}, M.~W. and {Pye}, J. and {Read}, A. and
         {Rodriguez}, P. and {Sakano}, M. and {Saxton}, R. and {Schwope}, A. and
         {Scott}, A.~E. and {Sturm}, R. and {Traulsen}, I. and {Yershov}, V. and
         {Zolotukhin}, I.},
        title = "{The XMM-Newton serendipitous survey. VII. The third XMM-Newton serendipitous source catalogue}",
      journal = {\aap},
     keywords = {catalogs, astronomical databases: miscellaneous, surveys, X-rays: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = may,
       volume = {590},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201526416},
archivePrefix = {arXiv},
       eprint = {1504.07051},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...590A...1R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Blanton11,
       author = {{Blanton}, Michael R. and {Kazin}, Eyal and {Muna}, Demitri and
         {Weaver}, Benjamin A. and {Price-Whelan}, Adrian},
        title = "{Improved Background Subtraction for the Sloan Digital Sky Survey Images}",
      journal = {\aj},
     keywords = {atmospheric effects, galaxies: photometry, methods: data analysis, techniques: image processing, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2011,
        month = jul,
       volume = {142},
       number = {1},
          eid = {31},
        pages = {31},
          doi = {10.1088/0004-6256/142/1/31},
archivePrefix = {arXiv},
       eprint = {1105.1960},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011AJ....142...31B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lupi20,
       author = {{Lupi}, Alessandro and {Sbarrato}, Tullia and {Carniani}, Stefano},
        title = "{Difficulties in mid-infrared selection of AGNs in dwarf galaxies}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: dwarf, galaxies: evolution, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = feb,
       volume = {492},
       number = {2},
        pages = {2528-2534},
          doi = {10.1093/mnras/stz3636},
archivePrefix = {arXiv},
       eprint = {2001.02234},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.492.2528L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Heckman14,
       author = {{Heckman}, Timothy M. and {Best}, Philip N.},
        title = "{The Coevolution of Galaxies and Supermassive Black Holes: Insights from Surveys of the Contemporary Universe}",
      journal = {\araa},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = aug,
       volume = {52},
        pages = {589-660},
          doi = {10.1146/annurev-astro-081913-035722},
archivePrefix = {arXiv},
       eprint = {1403.4620},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ARA&A..52..589H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Bittner19,
       author = {{Bittner}, A. and {Falc{\'o}n-Barroso}, J. and {Nedelchev}, B. and
         {Dorta}, A. and {Gadotti}, D.~A. and {Sarzi}, M. and
         {Molaeinezhad}, A. and {Iodice}, E. and {Rosado-Belza}, D. and
         {de Lorenzo-C{\'a}ceres}, A. and {Fragkoudi}, F. and
         {Gal{\'a}n-de Anta}, P.~M. and {Husemann}, B. and
         {M{\'e}ndez-Abreu}, J. and {Neumann}, J. and {Pinna}, F. and
         {Querejeta}, M. and {S{\'a}nchez-Bl{\'a}zquez}, P. and {Seidel}, M.~K.},
        title = "{The GIST pipeline: A multi-purpose tool for the analysis and visualisation of (integral-field) spectroscopic data}",
      journal = {\aap},
     keywords = {methods: data analysis, techniques: spectroscopic, galaxies: individual: NGC 1433, galaxies: stellar content, galaxies: kinematics and dynamics, galaxies: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2019",
        month = "Aug",
       volume = {628},
          eid = {A117},
        pages = {A117},
          doi = {10.1051/0004-6361/201935829},
archivePrefix = {arXiv},
       eprint = {1906.04746},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...628A.117B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reines19,
       author = {{Reines}, Amy E. and {Condon}, James J. and {Darling}, Jeremy and {Greene}, Jenny E.},
        title = "{A New Sample of (Wandering) Massive Black Holes in Dwarf Galaxies from High-resolution Radio Observations}",
      journal = {\apj},
     keywords = {Intermediate-mass black holes, Dwarf galaxies, Radio sources, Very Large Array, Active galactic nuclei, AGN host galaxies, Dwarf irregular galaxies, Supermassive black holes, 816, 416, 1358, 1766, 16, 2017, 417, 1663, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = jan,
       volume = {888},
       number = {1},
          eid = {36},
        pages = {36},
          doi = {10.3847/1538-4357/ab4999},
archivePrefix = {arXiv},
       eprint = {1909.04670},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...888...36R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Schramm13,
       author = {{Schramm}, M. and {Silverman}, J.~D. and {Greene}, J.~E. and {Brand
        t}, W.~N. and {Luo}, B. and {Xue}, Y.~Q. and {Capak}, P. and
         {Kakazu}, Y. and {Kartaltepe}, J. and {Mainieri}, V.},
        title = "{Unveiling a Population of Galaxies Harboring Low-mass Black Holes with X-Rays}",
      journal = {\apj},
     keywords = {galaxies: active, X-rays: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2013",
        month = "Aug",
       volume = {773},
       number = {2},
          eid = {150},
        pages = {150},
          doi = {10.1088/0004-637X/773/2/150},
archivePrefix = {arXiv},
       eprint = {1305.3826},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...773..150S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lemons15,
       author = {{Lemons}, Sean M. and {Reines}, Amy E. and {Plotkin}, Richard M. and
         {Gallo}, Elena and {Greene}, Jenny E.},
        title = "{An X-Ray Selected Sample of Candidate Black Holes in Dwarf Galaxies}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: dwarf, galaxies: nuclei, X-rays: binaries, X-rays: galaxies, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2015",
        month = "May",
       volume = {805},
       number = {1},
          eid = {12},
        pages = {12},
          doi = {10.1088/0004-637X/805/1/12},
archivePrefix = {arXiv},
       eprint = {1502.06958},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...805...12L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reines11,
       author = {{Reines}, Amy E. and {Sivakoff}, Gregory R. and {Johnson}, Kelsey E. and
         {Brogan}, Crystal L.},
        title = "{An actively accreting massive black hole in the dwarf starburst galaxy Henize2-10}",
      journal = {\nat},
     keywords = {Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2011",
        month = "Feb",
       volume = {470},
       number = {7332},
        pages = {66-68},
          doi = {10.1038/nature09724},
archivePrefix = {arXiv},
       eprint = {1101.1309},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011Natur.470...66R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reines12,
       author = {{Reines}, Amy E. and {Deller}, Adam T.},
        title = "{Parsec-scale Radio Emission from the Low-luminosity Active Galactic Nucleus in the Dwarf Starburst Galaxy Henize 2-10}",
      journal = {\apjl},
     keywords = {galaxies: active, galaxies: dwarf, galaxies: individual: He 2-10, galaxies: starburst, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2012",
        month = "May",
       volume = {750},
       number = {1},
          eid = {L24},
        pages = {L24},
          doi = {10.1088/2041-8205/750/1/L24},
archivePrefix = {arXiv},
       eprint = {1204.1970},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...750L..24R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mineo12,
       author = {{Mineo}, S. and {Gilfanov}, M. and {Sunyaev}, R.},
        title = "{X-ray emission from star-forming galaxies - I. High-mass X-ray binaries}",
      journal = {\mnras},
     keywords = {stars: formation, galaxies: irregular, galaxies: spiral, galaxies: starburst, X-rays: binaries, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2012",
        month = "Jan",
       volume = {419},
       number = {3},
        pages = {2095-2115},
          doi = {10.1111/j.1365-2966.2011.19862.x},
archivePrefix = {arXiv},
       eprint = {1105.4610},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.419.2095M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Latimer19,
       author = {{Latimer}, Colin J. and {Reines}, Amy E. and {Plotkin}, Richard M. and
         {Russell}, Thomas D. and {Condon}, James J.},
        title = "{An X-ray + Radio Search for Massive Black Holes in Blue Compact Dwarf Galaxies}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Jul",
          eid = {arXiv:1907.12585},
        pages = {arXiv:1907.12585},
archivePrefix = {arXiv},
       eprint = {1907.12585},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190712585L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Brandt15,
       author = {{Brandt}, W.~N. and {Alexander}, D.~M.},
        title = "{Cosmic X-ray surveys of distant active galaxies. The demographics, physics, and ecology of growing supermassive black holes}",
      journal = {\aapr},
     keywords = {Surveys, Cosmology: observations, Galaxies: active, Galaxies: nuclei, Galaxies: Seyfert, Galaxies: quasars, Galaxies: evolution, Black hole physics, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2015",
        month = "Jan",
       volume = {23},
          eid = {1},
        pages = {1},
          doi = {10.1007/s00159-014-0081-z},
archivePrefix = {arXiv},
       eprint = {1501.01982},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&ARv..23....1B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Pardo16,
   author = {{Pardo}, K. and {Goulding}, A.~D. and {Greene}, J.~E. and {Somerville}, R.~S. and 
	{Gallo}, E. and {Hickox}, R.~C. and {Miller}, B.~P. and {Reines}, A.~E. and 
	{Silverman}, J.~D.},
    title = "{X-Ray Detected Active Galactic Nuclei in Dwarf Galaxies at 0 $\lt$ z $\lt$ 1}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1603.01622},
 keywords = {galaxies: active, galaxies: dwarf, X-rays: galaxies},
     year = 2016,
    month = nov,
   volume = 831,
      eid = {203},
    pages = {203},
      doi = {10.3847/0004-637X/831/2/203},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...831..203P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Satyapal18,
       author = {{Satyapal}, Shobita and {Abel}, Nicholas P. and {Secrest}, Nathan J.},
        title = "{Star-forming Galaxies as AGN Imposters? A Theoretical Investigation of the Mid-infrared Colors of AGNs and Extreme Starbursts}",
      journal = {\apj},
     keywords = {dust, extinction, galaxies: active, galaxies: ISM, infrared: ISM, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "May",
       volume = {858},
       number = {1},
          eid = {38},
        pages = {38},
          doi = {10.3847/1538-4357/aab7f8},
archivePrefix = {arXiv},
       eprint = {1803.05980},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...858...38S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rupke17,
       author = {{Rupke}, David S.~N. and {G{\"u}ltekin}, Kayhan and {Veilleux}, Sylvain},
        title = "{Quasar-mode Feedback in Nearby Type 1 Quasars: Ubiquitous Kiloparsec-scale Outflows and Correlations with Black Hole Properties}",
      journal = {\apj},
     keywords = {galaxies: evolution, ISM: jets and outflows, quasars: general, quasars: supermassive black holes, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Nov",
       volume = {850},
       number = {1},
          eid = {40},
        pages = {40},
          doi = {10.3847/1538-4357/aa94d1},
archivePrefix = {arXiv},
       eprint = {1708.05139},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...850...40R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dubois16,
       author = {{Dubois}, Yohan and {Peirani}, S{\'e}bastien and {Pichon}, Christophe and
         {Devriendt}, Julien and {Gavazzi}, Rapha{\"e}l and {Welker}, Charlotte and
         {Volonteri}, Marta},
        title = "{The HORIZON-AGN simulation: morphological diversity of galaxies promoted by AGN feedback}",
      journal = {\mnras},
     keywords = {methods: numerical, galaxies: active, galaxies: evolution, galaxies: formation, galaxies: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Dec",
       volume = {463},
       number = {4},
        pages = {3948-3964},
          doi = {10.1093/mnras/stw2265},
archivePrefix = {arXiv},
       eprint = {1606.03086},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.463.3948D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Angles-Alcazar15,
       author = {{Angl{\'e}s-Alc{\'a}zar}, Daniel and {{\"O}zel}, Feryal and
         {Dav{\'e}}, Romeel and {Katz}, Neal and {Kollmeier}, Juna A. and
         {Oppenheimer}, Benjamin D.},
        title = "{Torque-limited Growth of Massive Black Holes in Galaxies across Cosmic Time}",
      journal = {\apj},
     keywords = {black hole physics, galaxies: active, galaxies: evolution, quasars: general, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2015",
        month = "Feb",
       volume = {800},
       number = {2},
          eid = {127},
        pages = {127},
          doi = {10.1088/0004-637X/800/2/127},
archivePrefix = {arXiv},
       eprint = {1309.5963},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...800..127A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Desroches09,
       author = {{Desroches}, Louis-Benoit and {Greene}, Jenny E. and {Ho}, Luis C.},
        title = "{X-Ray Properties of Intermediate-Mass Black Holes in Active Galaxies. II. X-Ray-Bright Accretion and Possible Evidence for Slim Disks}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: nuclei, galaxies: Seyfert, galaxies: statistics, X-rays: galaxies, Astrophysics - Galaxy Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = "2009",
        month = "Jun",
       volume = {698},
       number = {2},
        pages = {1515-1522},
          doi = {10.1088/0004-637X/698/2/1515},
archivePrefix = {arXiv},
       eprint = {0903.2257},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...698.1515D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lira99,
       author = {{Lira}, P. and {Lawrence}, A. and {O'Brien}, P. and {Johnson}, R.~A. and
         {Terlevich}, R. and {Bannister}, N.},
        title = "{Optical and X-ray variability in the least luminous active galactic nucleus, NGC 4395}",
      journal = {\mnras},
     keywords = {GALAXIES: INDIVIDUAL: NGC 4395, GALAXIES: NUCLEI, GALAXIES: SEYFERT, X-RAYS: GALAXIES, Astrophysics},
         year = "1999",
        month = "May",
       volume = {305},
       number = {1},
        pages = {109-124},
          doi = {10.1046/j.1365-8711.1999.02388.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/9901348},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999MNRAS.305..109L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Martin19,
   author = {{Martin}, G. and {Kaviraj}, S. and {Laigle}, C. and {Devriendt}, J.~E.~G. and 
	{Jackson}, R.~A. and {Peirani}, S. and {Dubois}, Y. and {Pichon}, C. and 
	{Slyz}, A.},
    title = "{The formation and evolution of low-surface-brightness galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1902.04580},
 keywords = {Galaxies: evolution, formation, dwarf, structure},
     year = 2019,
    month = may,
   volume = 485,
    pages = {796-818},
      doi = {10.1093/mnras/stz356},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.485..796M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Koudmani19,
       author = {{Koudmani}, Sophie and {Sijacki}, Debora and {Bourne}, Martin A. and
         {Smith}, Matthew C.},
        title = "{Fast and energetic AGN-driven outflows in simulated dwarf galaxies}",
      journal = {\mnras},
     keywords = {methods: numerical, galaxies: active, galaxies: dwarf, galaxies: formation, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Apr",
       volume = {484},
       number = {2},
        pages = {2047-2066},
          doi = {10.1093/mnras/stz097},
archivePrefix = {arXiv},
       eprint = {1812.04629},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.484.2047K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kaviraj19,
       author = {{Kaviraj}, Sugata and {Martin}, Garreth and {Silk}, Joseph},
        title = "{AGN in dwarf galaxies: frequency, triggering processes and the plausibility of AGN feedback}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: dwarf, galaxies: evolution, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Oct",
       volume = {489},
       number = {1},
        pages = {L12-L16},
          doi = {10.1093/mnrasl/slz102},
archivePrefix = {arXiv},
       eprint = {1906.10697},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.489L..12K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Baldassare15,
	doi = {10.1088/2041-8205/809/1/l14},
	url = {https://doi.org/10.1088%2F2041-8205%2F809%2F1%2Fl14},
	year = 2015,
	month = {aug},
	publisher = {{IOP} Publishing},
	volume = {809},
	number = {1},
	pages = {L14},
	author = {Vivienne F. Baldassare and Amy E. Reines and Elena Gallo and Jenny E. Greene},
	title = {A $\sim$50,000M$\odot${SOLAR} {MASS} {BLACK} {HOLE} {IN} {THE} {NUCLEUS} {OF} {RGG} 118},
	journal = {The Astrophysical Journal}
}

@INPROCEEDINGS{Shields08,
       author = {{Shields}, Joseph C. and {Walcher}, Carl Jakob and {B{\"o}ker}, Torsten and
         {Ho}, Luis C. and {Rix}, Hans-Walter and {van der Marel}, Roeland P.},
        title = "{An accreting black hole in the nucleus of the bulgeless galaxy NGC 1042}",
     keywords = {galaxies: nuclei, galaxies: active, galaxies: star clusters},
    booktitle = {Formation and Evolution of Galaxy Bulges},
         year = "2008",
       editor = {{Bureau}, Martin and {Athanassoula}, E. and {Barbuy}, Beatriz},
       series = {IAU Symposium},
       volume = {245},
        month = "Jul",
        pages = {259-260},
          doi = {10.1017/S1743921308017869},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008IAUS..245..259S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Greene05,
   author = {{Greene}, J.~E. and {Ho}, L.~C.},
    title = "{Estimating Black Hole Masses in Active Galaxies Using the H{$\alpha$} Emission Line}",
  journal = {\apj},
   eprint = {astro-ph/0508335},
 keywords = {Galaxies: Active, Galaxies: Jets, Galaxies: Nuclei, Galaxies: Seyfert, Galaxies: Quasars: General},
     year = 2005,
    month = sep,
   volume = 630,
    pages = {122-129},
      doi = {10.1086/431897},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...630..122G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@Inbook{Peterson2006,
author="Peterson, B.M.",
editor="Alloin, Danielle
and Johnson, Rachel
and Lira, Paulina",
title="The Broad-Line Region in Active Galactic Nuclei",
bookTitle="Physics of Active Galactic Nuclei at all Scales",
year="2006",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="77--100",
abstract="We review the basic observed and inferred properties of the broad emission-line region in AGNs, as well as the basics of the reverberation-mapping technique that can be used to determine the size and structure of the region. We argue that the current best evidence points to a multi-component line-emitting region, with a disk-like structure, possibly an extension of the accretion disk itself, and a disk wind being strong candidates for the origin of the broad-line emission.",
isbn="978-3-540-34621-0",
doi="10.1007/3-540-34621-X_3",
url="https://doi.org/10.1007/3-540-34621-X_3"
}

@ARTICLE{Seth10,
       author = {{Seth}, Anil C. and {Cappellari}, Michele and {Neumayer}, Nadine and
         {Caldwell}, Nelson and {Bastian}, Nate and {Olsen}, Knut and
         {Blum}, Robert D. and {Debattista}, Victor P. and {McDermid}, Richard and
         {Puzia}, Thomas and {Stephens}, Andrew},
        title = "{The NGC 404 Nucleus: Star Cluster and Possible Intermediate-mass Black Hole}",
      journal = {\apj},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: formation, galaxies: individual: NGC 404, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: structure, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2010",
        month = "May",
       volume = {714},
       number = {1},
        pages = {713-731},
          doi = {10.1088/0004-637X/714/1/713},
archivePrefix = {arXiv},
       eprint = {1003.0680},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...714..713S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Valluri05,
       author = {{Valluri}, Monica and {Ferrarese}, Laura and {Merritt}, David and
         {Joseph}, Charles L.},
        title = "{The Low End of the Supermassive Black Hole Mass Function: Constraining the Mass of a Nuclear Black Hole in NGC 205 via Stellar Kinematics}",
      journal = {\apj},
     keywords = {Galaxies: Elliptical and Lenticular, cD, Galaxies: Nuclei, Galaxies: Structure, Stellar Dynamics, Astrophysics},
         year = "2005",
        month = "Jul",
       volume = {628},
       number = {1},
        pages = {137-152},
          doi = {10.1086/430752},
archivePrefix = {arXiv},
       eprint = {astro-ph/0502493},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...628..137V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barth09,
       author = {{Barth}, Aaron J. and {Strigari}, Louis E. and {Bentz}, Misty C. and
         {Greene}, Jenny E. and {Ho}, Luis C.},
        title = "{Dynamical Constraints on the Masses of the Nuclear Star Cluster and Black Hole in the Late-Type Spiral Galaxy NGC 3621}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: individual: NGC 3621, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: spiral, Astrophysics},
         year = "2009",
        month = "Jan",
       volume = {690},
       number = {1},
        pages = {1031-1044},
          doi = {10.1088/0004-637X/690/1/1031},
archivePrefix = {arXiv},
       eprint = {0809.1066},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...690.1031B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barth04,
       author = {{Barth}, Aaron J. and {Ho}, Luis C. and {Rutledge}, Robert E. and
         {Sargent}, Wallace L.~W.},
        title = "{POX 52: A Dwarf Seyfert 1 Galaxy with an Intermediate-Mass Black Hole}",
      journal = {\apj},
     keywords = {Galaxies: Active, Galaxies: Dwarf, Galaxies: Individual: Alphanumeric: POX 52, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei, Galaxies: Seyfert, Astrophysics},
         year = "2004",
        month = "May",
       volume = {607},
       number = {1},
        pages = {90-102},
          doi = {10.1086/383302},
archivePrefix = {arXiv},
       eprint = {astro-ph/0402110},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...607...90B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Filippenko89,
       author = {{Filippenko}, Alexei V. and {Sargent}, Wallace L.~W.},
        title = "{Discovery of an Extremely Low Luminosity Seyfert 1 Nucleus in the Dwarf Galaxy NGC 4395}",
      journal = {\apjl},
     keywords = {Dwarf Galaxies, Galactic Nuclei, Light (Visible Radiation), Seyfert Galaxies, Stellar Luminosity, Emission Spectra, H Alpha Line, H Ii Regions, Line Spectra, Astrophysics, GALAXIES: INDIVIDUAL NGC NUMBER: NGC 4395, GALAXIES: NUCLEI, GALAXIES: SEYFERT, LINE PROFILES, SPECTROPHOTOMETRY},
         year = "1989",
        month = "Jul",
       volume = {342},
        pages = {L11},
          doi = {10.1086/185472},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1989ApJ...342L..11F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Barth08,
       author = {{Barth}, Aaron J. and {Greene}, Jenny E. and {Ho}, Luis C.},
        title = "{Low-Mass Seyfert 2 Galaxies in the Sloan Digital Sky Survey}",
      journal = {\aj},
     keywords = {galaxies: active, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: Seyfert, Astrophysics},
         year = "2008",
        month = "Sep",
       volume = {136},
       number = {3},
        pages = {1179-1200},
          doi = {10.1088/0004-6256/136/3/1179},
archivePrefix = {arXiv},
       eprint = {0807.3316},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008AJ....136.1179B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Power11,
       author = {{Power}, Chris and {Nayakshin}, Sergei and {King}, Andrew},
        title = "{The accretion disc particle method for simulations of black hole feeding and feedback}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, methods: numerical, galaxies: active, galaxies: formation, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2011",
        month = "Mar",
       volume = {412},
       number = {1},
        pages = {269-276},
          doi = {10.1111/j.1365-2966.2010.17901.x},
archivePrefix = {arXiv},
       eprint = {1003.0605},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.412..269P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dave19,
       author = {{Dav{\'e}}, Romeel and {Angl{\'e}s-Alc{\'a}zar}, Daniel and
         {Narayanan}, Desika and {Li}, Qi and {Rafieferantsoa}, Mika H. and
         {Appleby}, Sarah},
        title = "{SIMBA: Cosmological simulations with black hole growth and feedback}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2019",
        month = "Jun",
       volume = {486},
       number = {2},
        pages = {2827-2849},
          doi = {10.1093/mnras/stz937},
archivePrefix = {arXiv},
       eprint = {1901.10203},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.486.2827D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Booth09,
       author = {{Booth}, C.~M. and {Schaye}, Joop},
        title = "{Cosmological simulations of the growth of supermassive black holes and feedback from active galactic nuclei: method and tests}",
      journal = {\mnras},
     keywords = {hydrodynamics, galaxies: active, galaxies: evolution, galaxies: formation, quasars: general, cosmology: theory, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2009",
        month = "Sep",
       volume = {398},
       number = {1},
        pages = {53-74},
          doi = {10.1111/j.1365-2966.2009.15043.x},
archivePrefix = {arXiv},
       eprint = {0904.2572},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.398...53B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bondi52,
       author = {{Bondi}, H.},
        title = "{On spherically symmetrical accretion}",
      journal = {\mnras},
         year = "1952",
        month = "Jan",
       volume = {112},
        pages = {195},
          doi = {10.1093/mnras/112.2.195},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1952MNRAS.112..195B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nguyen18,
       author = {{Nguyen}, Dieu D. and {Seth}, Anil C. and {Neumayer}, Nadine and
         {Kamann}, Sebastian and {Voggel}, Karina T. and {Cappellari}, Michele and
         {Picotti}, Arianna and {Nguyen}, Phuong M. and {B{\"o}ker}, Torsten and
         {Debattista}, Victor and {Caldwell}, Nelson and {McDermid}, Richard and
         {Bastian}, Nathan and {Ahn}, Christopher C. and {Pechetti}, Renuka},
        title = "{Nearby Early-type Galactic Nuclei at High Resolution: Dynamical Black Hole and Nuclear Star Cluster Mass Measurements}",
      journal = {\apj},
     keywords = {galaxies: individual: NGC 221 (M32, NGC 205, NGC 5102, and NGC 5206, galaxies: kinematics and dynamics, galaxies: nuclei, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "May",
       volume = {858},
       number = {2},
          eid = {118},
        pages = {118},
          doi = {10.3847/1538-4357/aabe28},
archivePrefix = {arXiv},
       eprint = {1711.04314},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...858..118N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Miller15,
       author = {{Miller}, Brendan P. and {Gallo}, Elena and {Greene}, Jenny E. and
         {Kelly}, Brandon C. and {Treu}, Tommaso and {Woo}, Jong-Hak and
         {Baldassare}, Vivienne},
        title = "{X-Ray Constraints on the Local Supermassive Black Hole Occupation Fraction}",
      journal = {\apj},
     keywords = {black hole physics, galaxies: nuclei, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2015",
        month = "Jan",
       volume = {799},
       number = {1},
          eid = {98},
        pages = {98},
          doi = {10.1088/0004-637X/799/1/98},
archivePrefix = {arXiv},
       eprint = {1403.4246},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...799...98M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Magorrian98,
       author = {{Magorrian}, John and {Tremaine}, Scott and {Richstone}, Douglas and
         {Bender}, Ralf and {Bower}, Gary and {Dressler}, Alan and
         {Faber}, S.~M. and {Gebhardt}, Karl and {Green}, Richard and
         {Grillmair}, Carl and {Kormendy}, John and {Lauer}, Tod},
        title = "{The Demography of Massive Dark Objects in Galaxy Centers}",
      journal = {\aj},
     keywords = {COSMOLOGY: DARK MATTER, GALAXIES: NUCLEI, Astrophysics},
         year = "1998",
        month = "Jun",
       volume = {115},
       number = {6},
        pages = {2285-2305},
          doi = {10.1086/300353},
archivePrefix = {arXiv},
       eprint = {astro-ph/9708072},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998AJ....115.2285M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Greene12,
       author = {{Greene}, Jenny E.},
        title = "{Low-mass black holes as the remnants of primordial black hole formation}",
      journal = {Nature Communications},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "Dec",
       volume = {3},
          eid = {1304},
        pages = {1304},
          doi = {10.1038/ncomms2314},
archivePrefix = {arXiv},
       eprint = {1211.7082},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012NatCo...3.1304G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Volonteri09,
       author = {{Volonteri}, Marta and {Natarajan}, Priyamvada},
        title = "{Journey to the M$_{BH}$-{\ensuremath{\sigma}} relation: the fate of low-mass black holes in the Universe}",
      journal = {\mnras},
     keywords = {accretion, accretion discs, black hole physics, hydrodynamics, instabilities, galaxies: formation, cosmology: theory, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2009",
        month = "Dec",
       volume = {400},
       number = {4},
        pages = {1911-1918},
          doi = {10.1111/j.1365-2966.2009.15577.x},
archivePrefix = {arXiv},
       eprint = {0903.2262},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.400.1911V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lodato06,
       author = {{Lodato}, Giuseppe and {Natarajan}, Priyamvada},
        title = "{Supermassive black hole formation during the assembly of pre-galactic discs}",
      journal = {\mnras},
     keywords = {accretion, accretion discs: black hole physics: hydrodynamics: instabilities: galaxies: formation: cosmology: theory, accretion discs, black hole physics, hydrodynamics, instabilities, galaxies: formation, cosmology: theory, Astrophysics},
         year = "2006",
        month = "Oct",
       volume = {371},
       number = {4},
        pages = {1813-1823},
          doi = {10.1111/j.1365-2966.2006.10801.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0606159},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MNRAS.371.1813L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ferrarese00,
       author = {{Ferrarese}, Laura and {Merritt}, David},
        title = "{A Fundamental Relation between Supermassive Black Holes and Their Host Galaxies}",
      journal = {\apjl},
     keywords = {Black Hole Physics, Galaxies: Evolution, Galaxies: Kinematics and Dynamics, Astrophysics},
         year = "2000",
        month = "Aug",
       volume = {539},
       number = {1},
        pages = {L9-L12},
          doi = {10.1086/312838},
archivePrefix = {arXiv},
       eprint = {astro-ph/0006053},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...539L...9F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tremaine02,
       author = {{Tremaine}, Scott and {Gebhardt}, Karl and {Bender}, Ralf and
         {Bower}, Gary and {Dressler}, Alan and {Faber}, S.~M. and
         {Filippenko}, Alexei V. and {Green}, Richard and {Grillmair}, Carl and
         {Ho}, Luis C. and {Kormendy}, John and {Lauer}, Tod R. and
         {Magorrian}, John and {Pinkney}, Jason and {Richstone}, Douglas},
        title = "{The Slope of the Black Hole Mass versus Velocity Dispersion Correlation}",
      journal = {\apj},
     keywords = {Black Hole Physics, Galaxies: Bulges, Galaxies: Fundamental Parameters, Galaxies: Nuclei, Galaxy: Bulge, Galaxy: Kinematics and Dynamics, Astrophysics},
         year = "2002",
        month = "Aug",
       volume = {574},
       number = {2},
        pages = {740-753},
          doi = {10.1086/341002},
archivePrefix = {arXiv},
       eprint = {astro-ph/0203468},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...574..740T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gultekin09,
       author = {{G{\"u}ltekin}, Kayhan and {Richstone}, Douglas O. and {Gebhardt}, Karl and
         {Lauer}, Tod R. and {Tremaine}, Scott and {Aller}, M.~C. and
         {Bender}, Ralf and {Dressler}, Alan and {Faber}, S.~M. and
         {Filippenko}, Alexei V. and {Green}, Richard and {Ho}, Luis C. and
         {Kormendy}, John and {Magorrian}, John and {Pinkney}, Jason and
         {Siopis}, Christos},
        title = "{The M-{\ensuremath{\sigma}} and M-L Relations in Galactic Bulges, and Determinations of Their Intrinsic Scatter}",
      journal = {\apj},
     keywords = {black hole physics, galaxies: general, galaxies: nuclei, galaxies: statistics, stellar dynamics, Astrophysics - Galaxy Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = "2009",
        month = "Jun",
       volume = {698},
       number = {1},
        pages = {198-221},
          doi = {10.1088/0004-637X/698/1/198},
archivePrefix = {arXiv},
       eprint = {0903.4897},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...698..198G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Volonteri15,
       author = {{Volonteri}, Marta and {Capelo}, Pedro R. and {Netzer}, Hagai and
         {Bellovary}, Jillian and {Dotti}, Massimo and {Governato}, Fabio},
        title = "{Growing black holes and galaxies: black hole accretion versus star formation rate}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: interactions, galaxies: nuclei, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2015",
        month = "May",
       volume = {449},
       number = {2},
        pages = {1470-1485},
          doi = {10.1093/mnras/stv387},
archivePrefix = {arXiv},
       eprint = {1502.06363},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.449.1470V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jones19,
       author = {{Jones}, Mackenzie L. and {Hickox}, Ryan C. and {Mutch}, Simon J. and
         {Croton}, Darren J. and {Ptak}, Andrew F. and {DiPompeo}, Michael A.},
        title = "{Evolution of Black Hole and Galaxy Growth in a Semi-numerical Galaxy Formation Model}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: evolution, quasars: general, X-rays: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Aug",
       volume = {881},
       number = {2},
          eid = {110},
        pages = {110},
          doi = {10.3847/1538-4357/ab2d9f},
archivePrefix = {arXiv},
       eprint = {1907.00981},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...881..110J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lasker16,
       author = {{L{\"a}sker}, Ronald and {Greene}, Jenny E. and {Seth}, Anil and
         {van de Ven}, Glenn and {Braatz}, James A. and {Henkel}, Christian and
         {Lo}, K.~Y.},
        title = "{The Black Hole-Bulge Mass Relation in Megamaser Host Galaxies}",
      journal = {\apj},
     keywords = {galaxies: bulges, galaxies: photometry, galaxies: structure, methods: observational, techniques: photometric, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Jul",
       volume = {825},
       number = {1},
          eid = {3},
        pages = {3},
          doi = {10.3847/0004-637X/825/1/3},
archivePrefix = {arXiv},
       eprint = {1602.06960},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...825....3L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Nguyen19,
       author = {{Nguyen}, Dieu D. and {Seth}, Anil C. and {Neumayer}, Nadine and
         {Iguchi}, Satoru and {Cappellari}, Michelle and {Strader}, Jay and
         {Chomiuk}, Laura and {Tremou}, Evangelia and {Pacucci}, Fabio and
         {Nakanishi}, Kouichiro and {Bahramian}, Arash and {Nguyen}, Phuong M. and
         {den Brok}, Mark and {Ahn}, Christopher C. and {Voggel}, Karina T. and
         {Kacharov}, Nikolay and {Tsukui}, Takafumi and {Ly}, Cuc K. and
         {Dumont}, Antoine and {Pechetti}, Renuka},
        title = "{Improved Dynamical Constraints on the Masses of the Central Black Holes in Nearby Low-mass Early-type Galactic Nuclei and the First Black Hole Determination for NGC 205}",
      journal = {\apj},
     keywords = {galaxies: individual: NGC 205, NGC 5102, and NGC 5206, galaxies: kinematics and dynamics, galaxies: nuclei, quasars: supermassive black holes, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Feb",
       volume = {872},
       number = {1},
          eid = {104},
        pages = {104},
          doi = {10.3847/1538-4357/aafe7a},
archivePrefix = {arXiv},
       eprint = {1901.05496},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...872..104N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Schutte19,
       author = {{Schutte}, Zachary and {Reines}, Amy and {Greene}, Jenny},
        title = "{The Black Hole -- Bulge Mass Relation including Dwarf Galaxies Hosting Active Galactic Nuclei}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Jul",
          eid = {arXiv:1908.00020},
        pages = {arXiv:1908.00020},
archivePrefix = {arXiv},
       eprint = {1908.00020},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190800020S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Natarajan14,
       author = {{Natarajan}, Priyamvada},
        title = "{Seeds to monsters: tracing the growth of black holes in the universe}",
      journal = {General Relativity and Gravitation},
     keywords = {Black holes, Galaxy formation, Quasars},
         year = "2014",
        month = "May",
       volume = {46},
          eid = {1702},
        pages = {1702},
          doi = {10.1007/s10714-014-1702-6},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014GReGr..46.1702N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Volonteri08,
       author = {{Volonteri}, Marta and {Lodato}, Giuseppe and {Natarajan}, Priyamvada},
        title = "{The evolution of massive black hole seeds}",
      journal = {\mnras},
     keywords = {black hole physics, galaxies: evolution, quasars: general, cosmology: miscellaneous, Astrophysics},
         year = "2008",
        month = "Jan",
       volume = {383},
       number = {3},
        pages = {1079-1088},
          doi = {10.1111/j.1365-2966.2007.12589.x},
archivePrefix = {arXiv},
       eprint = {0709.0529},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008MNRAS.383.1079V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Neymayer12,
       author = {{Neumayer}, Nadine and {Walcher}, C. Jakob},
        title = "{Are Nuclear Star Clusters the Precursors of Massive Black Holes?}",
      journal = {Advances in Astronomy},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "Jan",
       volume = {2012},
          eid = {709038},
        pages = {709038},
          doi = {10.1155/2012/709038},
archivePrefix = {arXiv},
       eprint = {1201.4950},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012AdAst2012E..15N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INBOOK{Jogee06,
       author = {{Jogee}, S.},
        title = "{The Fueling and Evolution of AGN: Internal and External Triggers}",
     keywords = {Astrophysics},
    booktitle = {Physics of Active Galactic Nuclei at all Scales, edited by Danielle Alloin, Rachel Johnson and Paulina Lira.  Lecture Notes in Physics, Vol. 693. ISBN-10 3-540-31207-2; ISBN-13 978-3-540-31207-9; ISSN 0075-8450. Library of Congress Catalog Card No. 2006925838. Published by Springer, Berlin and Heidelberg, 2006, p.143},
         year = "2006",
       editor = {{Alloin}, Danielle},
       volume = {693},
        pages = {143},
          doi = {10.1007/3-540-34621-X_6},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006LNP...693..143J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hopkins08,
       author = {{Hopkins}, Philip F. and {Hernquist}, Lars and {Cox}, Thomas J. and
         {Kere{\v{s}}}, Du{\v{s}}an},
        title = "{A Cosmological Framework for the Co-Evolution of Quasars, Supermassive Black Holes, and Elliptical Galaxies. I. Galaxy Mergers and Quasar Activity}",
      journal = {\apjs},
     keywords = {cosmology: theory, galaxies: active, galaxies: evolution, quasars: general, Astrophysics},
         year = "2008",
        month = "Apr",
       volume = {175},
       number = {2},
        pages = {356-389},
          doi = {10.1086/524362},
archivePrefix = {arXiv},
       eprint = {0706.1243},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJS..175..356H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Silk98,
       author = {{Silk}, Joseph and {Rees}, Martin J.},
        title = "{Quasars and galaxy formation}",
      journal = {\aap},
     keywords = {GALAXY FORMATION: SUPERMASSIVE BLACK HOLES, QUASARS: OUTFLOWS, Astrophysics},
         year = "1998",
        month = "Mar",
       volume = {331},
        pages = {L1-L4},
archivePrefix = {arXiv},
       eprint = {astro-ph/9801013},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998A&A...331L...1S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Izotov08,
       author = {{Izotov}, Yuri I. and {Thuan}, Trinh X.},
        title = "{Active Galactic Nuclei in Four Metal-poor Dwarf Emission-Line Galaxies}",
      journal = {\apj},
     keywords = {galaxies: abundances, galaxies: active, galaxies: irregular, galaxies: ISM, H II regions, ISM: kinematics and dynamics, Astrophysics},
         year = "2008",
        month = "Nov",
       volume = {687},
       number = {1},
        pages = {133-140},
          doi = {10.1086/591660},
archivePrefix = {arXiv},
       eprint = {0807.2029},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...687..133I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fathi06,
       author = {{Fathi}, Kambiz and {Storchi-Bergmann}, Thaisa and {Riffel}, Rogemar A. and
         {Winge}, Claudia and {Axon}, David J. and {Robinson}, Andrew and
         {Capetti}, Alessandro and {Marconi}, Alessandro},
        title = "{Streaming Motions toward the Supermassive Black Hole in NGC 1097}",
      journal = {\apjl},
     keywords = {Galaxies: Active, Galaxies: Kinematics and Dynamics, Galaxies: Nuclei, Astrophysics},
         year = "2006",
        month = "Apr",
       volume = {641},
       number = {1},
        pages = {L25-L28},
          doi = {10.1086/503832},
archivePrefix = {arXiv},
       eprint = {astro-ph/0602002},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...641L..25F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dumas07,
       author = {{Dumas}, Ga{\"e}lle and {Mundell}, Carole G. and {Emsellem}, Eric and
         {Nagar}, Neil M.},
        title = "{Central kiloparsec of Seyfert and inactive host galaxies: a comparison of two-dimensional stellar and gaseous kinematics}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: kinematics and dynamics, galaxies: Seyfert, galaxies: spiral, galaxies: structure, Astrophysics},
         year = "2007",
        month = "Aug",
       volume = {379},
       number = {4},
        pages = {1249-1278},
          doi = {10.1111/j.1365-2966.2007.12014.x},
archivePrefix = {arXiv},
       eprint = {0705.4162},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007MNRAS.379.1249D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dekel09,
       author = {{Dekel}, Avishai and {Sari}, Re'em and {Ceverino}, Daniel},
        title = "{Formation of Massive Galaxies at High Redshift: Cold Streams, Clumpy Disks, and Compact Spheroids}",
      journal = {\apj},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, galaxies: formation, galaxies: halos, galaxies: spiral, Astrophysics - Galaxy Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = "2009",
        month = "Sep",
       volume = {703},
       number = {1},
        pages = {785-801},
          doi = {10.1088/0004-637X/703/1/785},
archivePrefix = {arXiv},
       eprint = {0901.2458},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...703..785D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bournaud11,
       author = {{Bournaud}, Fr{\'e}d{\'e}ric and {Dekel}, Avishai and
         {Teyssier}, Romain and {Cacciato}, Marcello and {Daddi}, Emanuele and
         {Juneau}, St{\'e}phanie and {Shankar}, Francesco},
        title = "{Black Hole Growth and Active Galactic Nuclei Obscuration by Instability-driven Inflows in High-redshift Disk Galaxies Fed by Cold Streams}",
      journal = {\apjl},
     keywords = {galaxies: active, galaxies: formation, galaxies: high-redshift, galaxies: nuclei, X-rays: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2011",
        month = "Nov",
       volume = {741},
       number = {2},
          eid = {L33},
        pages = {L33},
          doi = {10.1088/2041-8205/741/2/L33},
archivePrefix = {arXiv},
       eprint = {1107.1483},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...741L..33B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hopkins11,
       author = {{Hopkins}, Philip F. and {Quataert}, Eliot},
        title = "{An analytic model of angular momentum transport by gravitational torques: from galaxies to massive black holes}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: evolution, quasars: general, cosmology: theory, Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - Galaxy Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2011",
        month = "Aug",
       volume = {415},
       number = {2},
        pages = {1027-1050},
          doi = {10.1111/j.1365-2966.2011.18542.x},
archivePrefix = {arXiv},
       eprint = {1007.2647},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.415.1027H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Angles-Alcazar17,
       author = {{Angl{\'e}s-Alc{\'a}zar}, Daniel and {Dav{\'e}}, Romeel and
         {Faucher-Gigu{\`e}re}, Claude-Andr{\'e} and {{\"O}zel}, Feryal and
         {Hopkins}, Philip F.},
        title = "{Gravitational torque-driven black hole growth and feedback in cosmological simulations}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: evolution, galaxies: formation, intergalactic medium, quasars: supermassive black holes, cosmology: theory, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2017",
        month = "Jan",
       volume = {464},
       number = {3},
        pages = {2840-2853},
          doi = {10.1093/mnras/stw2565},
archivePrefix = {arXiv},
       eprint = {1603.08007},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.464.2840A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Englmaier04,
       author = {{Englmaier}, Peter and {Shlosman}, Isaac},
        title = "{Dynamical Decoupling of Nested Bars: Self-gravitating Gaseous Nuclear Bars}",
      journal = {\apjl},
     keywords = {Galaxies: Active, Galaxies: Evolution, Galaxies: Kinematics and Dynamics, Galaxies: Spiral, Galaxies: Starburst, Hydrodynamics, Astrophysics},
         year = "2004",
        month = "Dec",
       volume = {617},
       number = {2},
        pages = {L115-L118},
          doi = {10.1086/427280},
archivePrefix = {arXiv},
       eprint = {astro-ph/0410283},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...617L.115E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maciejewski04,
       author = {{Maciejewski}, Witold},
        title = "{Nuclear spirals in galaxies: gas response to an asymmetric potential - II. Hydrodynamical models}",
      journal = {\mnras},
     keywords = {hydrodynamics, galaxies: ISM, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: spiral, galaxies: structure, Astrophysics},
         year = "2004",
        month = "Nov",
       volume = {354},
       number = {3},
        pages = {892-904},
          doi = {10.1111/j.1365-2966.2004.08254.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0408100},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.354..892M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Milosavljevic06,
       author = {{Milosavljevi{\'c}}, Milo{\v{s}} and {Merritt}, David and {Ho}, Luis C.},
        title = "{Contribution of Stellar Tidal Disruptions to the X-Ray Luminosity Function of Active Galaxies}",
      journal = {\apj},
     keywords = {Accretion, Accretion Disks, Black Hole Physics, Cosmology: Observations, Galaxies: Active, Galaxies: Nuclei, Astrophysics},
         year = "2006",
        month = "Nov",
       volume = {652},
       number = {1},
        pages = {120-125},
          doi = {10.1086/508134},
archivePrefix = {arXiv},
       eprint = {astro-ph/0602289},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...652..120M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Davies09,
       author = {{Davies}, R.~I. and {Maciejewski}, W. and {Hicks}, E.~K.~S. and
         {Tacconi}, L.~J. and {Genzel}, R. and {Engel}, H.},
        title = "{Stellar and Molecular Gas Kinematics Of NGC 1097: Inflow Driven by a Nuclear Spiral}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: individual: NGC 1097, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: spiral, infrared: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2009",
        month = "Sep",
       volume = {702},
       number = {1},
        pages = {114-128},
          doi = {10.1088/0004-637X/702/1/114},
archivePrefix = {arXiv},
       eprint = {0903.0313},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...702..114D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Muller-Sanchez09,
       author = {{M{\"u}ller S{\'a}nchez}, F. and {Davies}, R.~I. and {Genzel}, R. and
         {Tacconi}, L.~J. and {Eisenhauer}, F. and {Hicks}, E.~K.~S. and
         {Friedrich}, S. and {Sternberg}, A.},
        title = "{Molecular Gas Streamers Feeding and Obscuring the Active Nucleus of NGC 1068}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: individual: NGC 1068, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: Seyfert, infrared: galaxies, Astrophysics},
         year = "2009",
        month = "Jan",
       volume = {691},
       number = {1},
        pages = {749-759},
          doi = {10.1088/0004-637X/691/1/749},
archivePrefix = {arXiv},
       eprint = {0809.4943},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...691..749M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Fernandes04,
   author = {{Cid Fernandes}, R. and {Gonz{\'a}lez Delgado}, R.~M. and {Schmitt}, H. and 
	{Storchi-Bergmann}, T. and {Martins}, L.~P. and {P{\'e}rez}, E. and 
	{Heckman}, T. and {Leitherer}, C. and {Schaerer}, D.},
    title = "{The Stellar Populations of Low-Luminosity Active Galactic Nuclei. I. Ground-based Observations}",
  journal = {\apj},
   eprint = {astro-ph/0401416},
 keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Starburst, Galaxies: Stellar Content},
     year = 2004,
    month = apr,
   volume = 605,
    pages = {105-126},
      doi = {10.1086/382217},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...605..105C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}@ARTICLE{Davies07,
       author = {{Davies}, R.~I. and {M{\"u}ller S{\'a}nchez}, F. and {Genzel}, R. and
         {Tacconi}, L.~J. and {Hicks}, E.~K.~S. and {Friedrich}, S. and
         {Sternberg}, A.},
        title = "{A Close Look at Star Formation around Active Galactic Nuclei}",
      journal = {\apj},
     keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert, Galaxies: Starburst, Infrared: Galaxies, Astrophysics},
         year = "2007",
        month = "Dec",
       volume = {671},
       number = {2},
        pages = {1388-1412},
          doi = {10.1086/523032},
archivePrefix = {arXiv},
       eprint = {0704.1374},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...671.1388D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hopkins12,
       author = {{Hopkins}, Philip F. and {Hernquist}, Lars and
         {Hayward}, Christopher C. and {Narayanan}, Desika},
        title = "{Why are active galactic nuclei and host galaxies misaligned?}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: evolution, quasars: general, cosmology: theory, Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2012",
        month = "Sep",
       volume = {425},
       number = {2},
        pages = {1121-1128},
          doi = {10.1111/j.1365-2966.2012.21449.x},
archivePrefix = {arXiv},
       eprint = {1111.1236},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.425.1121H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Alexander12,
       author = {{Alexander}, D.~M. and {Hickox}, R.~C.},
        title = "{What drives the growth of black holes?}",
      journal = {\nar},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "Jun",
       volume = {56},
       number = {4},
        pages = {93-121},
          doi = {10.1016/j.newar.2011.11.003},
archivePrefix = {arXiv},
       eprint = {1112.1949},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012NewAR..56...93A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Neumayer12,
       author = {{Neumayer}, Nadine and {Walcher}, C. Jakob},
        title = "{Are Nuclear Star Clusters the Precursors of Massive Black Holes?}",
      journal = {Advances in Astronomy},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "Jan",
       volume = {2012},
          eid = {709038},
        pages = {709038},
          doi = {10.1155/2012/709038},
archivePrefix = {arXiv},
       eprint = {1201.4950},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012AdAst2012E..15N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Trump15,
       author = {{Trump}, Jonathan R. and {Sun}, Mouyuan and {Zeimann}, Gregory R. and
         {Luck}, Cuyler and {Bridge}, Joanna S. and {Grier}, Catherine J. and
         {Hagen}, Alex and {Juneau}, Stephanie and {Montero-Dorta}, Antonio and
         {Rosario}, David J. and {Brandt}, W. Niel and {Ciardullo}, Robin and
         {Schneider}, Donald P.},
        title = "{The Biases of Optical Line-Ratio Selection for Active Galactic Nuclei and the Intrinsic Relationship between Black Hole Accretion and Galaxy Star Formation}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: evolution, galaxies: nuclei, galaxies: Seyfert, quasars: emission lines, Astrophysics - Astrophysics of Galaxies},
         year = "2015",
        month = "Sep",
       volume = {811},
       number = {1},
          eid = {26},
        pages = {26},
          doi = {10.1088/0004-637X/811/1/26},
archivePrefix = {arXiv},
       eprint = {1501.02801},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...811...26T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Baldassare18,
       author = {{Baldassare}, Vivienne F. and {Geha}, Marla and {Greene}, Jenny},
        title = "{Identifying AGNs in Low-mass Galaxies via Long-term Optical Variability}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: photometry, quasars: supermassive black holes, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Dec",
       volume = {868},
       number = {2},
          eid = {152},
        pages = {152},
          doi = {10.3847/1538-4357/aae6cf},
archivePrefix = {arXiv},
       eprint = {1808.09578},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...868..152B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reines15,
       author = {{Reines}, Amy E. and {Volonteri}, Marta},
        title = "{Relations between Central Black Hole Mass and Total Galaxy Stellar Mass in the Local Universe}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: evolution, galaxies: nuclei, galaxies: Seyfert, Astrophysics - Astrophysics of Galaxies},
         year = "2015",
        month = "Nov",
       volume = {813},
       number = {2},
          eid = {82},
        pages = {82},
          doi = {10.1088/0004-637X/813/2/82},
archivePrefix = {arXiv},
       eprint = {1508.06274},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...813...82R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Greene04,
       author = {{Greene}, Jenny E. and {Ho}, Luis C.},
        title = "{Active Galactic Nuclei with Candidate Intermediate-Mass Black Holes}",
      journal = {\apj},
     keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert, Astrophysics},
         year = "2004",
        month = "Aug",
       volume = {610},
       number = {2},
        pages = {722-736},
          doi = {10.1086/421719},
archivePrefix = {arXiv},
       eprint = {astro-ph/0404110},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...610..722G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Singh13,
       author = {{Singh}, R. and {van de Ven}, G. and {Jahnke}, K. and {Lyubenova}, M. and
         {Falc{\'o}n-Barroso}, J. and {Alves}, J. and {Cid Fernandes}, R. and
         {Galbany}, L. and {Garc{\'\i}a-Benito}, R. and {Husemann}, B. and
         {Kennicutt}, R.~C. and {Marino}, R.~A. and {M{\'a}rquez}, I. and
         {Masegosa}, J. and {Mast}, D. and {Pasquali}, A. and
         {S{\'a}nchez}, S.~F. and {Walcher}, J. and {Wild}, V. and
         {Wisotzki}, L. and {Ziegler}, B.},
        title = "{The nature of LINER galaxies:. Ubiquitous hot old stars and rare accreting black holes}",
      journal = {\aap},
     keywords = {galaxies: active, galaxies: ISM, galaxies: nuclei, stars: AGB and post-AGB, Astrophysics - Galaxy Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = "2013",
        month = "Oct",
       volume = {558},
          eid = {A43},
        pages = {A43},
          doi = {10.1051/0004-6361/201322062},
archivePrefix = {arXiv},
       eprint = {1308.4271},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...558A..43S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Dickey19,
       author = {{Dickey}, C. and {Geha}, M. and {Wetzel}, A. and {El-Badry}, K.},
        title = "{AGN All the Way Down? AGN-like Line Ratios are Common In the Lowest-Mass Isolated Quiescent Galaxies}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = feb,
          eid = {arXiv:1902.01401},
        pages = {arXiv:1902.01401},
archivePrefix = {arXiv},
       eprint = {1902.01401},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190201401D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ranalli03,
       author = {{Ranalli}, P. and {Comastri}, A. and {Setti}, G.},
        title = "{The 2-10 keV luminosity as a Star Formation Rate indicator}",
      journal = {\aap},
     keywords = {X-rays: galaxies, radio continuum: galaxies, galaxies: high-redshift, infrared: galaxies -, galaxies: fundamental parameters, galaxies: starburst, Astrophysics},
         year = 2003,
        month = feb,
       volume = {399},
        pages = {39-50},
          doi = {10.1051/0004-6361:20021600},
archivePrefix = {arXiv},
       eprint = {astro-ph/0211304},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...399...39R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bryant15,
       author = {{Bryant}, J.~J. and {Owers}, M.~S. and {Robotham}, A.~S.~G. and
         {Croom}, S.~M. and {Driver}, S.~P. and {Drinkwater}, M.~J. and
         {Lorente}, N.~P.~F. and {Cortese}, L. and {Scott}, N. and
         {Colless}, M. and {Schaefer}, A. and {Taylor}, E.~N. and
         {Konstantopoulos}, I.~S. and {Allen}, J.~T. and {Baldry}, I. and
         {Barnes}, L. and {Bauer}, A.~E. and {Bland-Hawthorn}, J. and
         {Bloom}, J.~V. and {Brooks}, A.~M. and {Brough}, S. and {Cecil}, G. and
         {Couch}, W. and {Croton}, D. and {Davies}, R. and {Ellis}, S. and
         {Fogarty}, L.~M.~R. and {Foster}, C. and {Glazebrook}, K. and
         {Goodwin}, M. and {Green}, A. and {Gunawardhana}, M.~L. and
         {Hampton}, E. and {Ho}, I. -T. and {Hopkins}, A.~M. and {Kewley}, L. and
         {Lawrence}, J.~S. and {Leon-Saval}, S.~G. and {Leslie}, S. and
         {McElroy}, R. and {Lewis}, G. and {Liske}, J. and
         {L{\'o}pez-S{\'a}nchez}, {\'A}. R. and {Mahajan}, S. and
         {Medling}, A.~M. and {Metcalfe}, N. and {Meyer}, M. and {Mould}, J. and
         {Obreschkow}, D. and {O'Toole}, S. and {Pracy}, M. and
         {Richards}, S.~N. and {Shanks}, T. and {Sharp}, R. and {Sweet}, S.~M. and
         {Thomas}, A.~D. and {Tonini}, C. and {Walcher}, C.~J.},
        title = "{The SAMI Galaxy Survey: instrument specification and target selection}",
      journal = {\mnras},
     keywords = {instrumentation: miscellaneous, instrumentation: spectrographs, techniques: imaging spectroscopy, surveys, galaxies: evolution, galaxies: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = mar,
       volume = {447},
       number = {3},
        pages = {2857-2879},
          doi = {10.1093/mnras/stu2635},
archivePrefix = {arXiv},
       eprint = {1407.7335},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.447.2857B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Thomas13,
       author = {{Thomas}, D. and {Steele}, O. and {Maraston}, C. and {Johansson}, J. and
         {Beifiori}, A. and {Pforr}, J. and {Str{\"o}mb{\"a}ck}, G. and
         {Tremonti}, C.~A. and {Wake}, D. and {Bizyaev}, D. and {Bolton}, A. and
         {Brewington}, H. and {Brownstein}, J.~R. and {Comparat}, J. and
         {Kneib}, J. -P. and {Malanushenko}, E. and {Malanushenko}, V. and
         {Oravetz}, D. and {Pan}, K. and {Parejko}, J.~K. and
         {Schneider}, D.~P. and {Shelden}, A. and {Simmons}, A. and
         {Snedden}, S. and {Tanaka}, M. and {Weaver}, B.~A. and {Yan}, R.},
        title = "{Stellar velocity dispersions and emission line properties of SDSS-III/BOSS galaxies}",
      journal = {\mnras},
     keywords = {surveys, galaxies: active, galaxies: evolution, galaxies: general, galaxies: ISM, galaxies: kinematics and dynamics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = may,
       volume = {431},
       number = {2},
        pages = {1383-1397},
          doi = {10.1093/mnras/stt261},
archivePrefix = {arXiv},
       eprint = {1207.6115},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.431.1383T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Yan12,
       author = {{Yan}, Renbin and {Blanton}, Michael R.},
        title = "{The Nature of LINER-like Emission in Red Galaxies}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: elliptical and lenticular, cD, galaxies: ISM, ISM: kinematics and dynamics, stars: AGB and post-AGB, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2012,
        month = mar,
       volume = {747},
       number = {1},
          eid = {61},
        pages = {61},
          doi = {10.1088/0004-637X/747/1/61},
archivePrefix = {arXiv},
       eprint = {1109.1280},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...747...61Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Palumbo20,
       author = {{Palumbo}, Michael L. and {Kannappan}, Sheila J. and
         {Frazer}, Elaine M. and {Eckert}, Kathleen D. and {Norman}, Dara J. and
         {Fraga}, Luciano and {Quint}, Bruno C. and {Amram}, Philippe and
         {Mendes de Oliveira}, Claudia and {Bittner}, Ashley S. and
         {Moffett}, Amanda J. and {Stark}, David V. and {Norris}, Mark A. and
         {Cleaves}, Nathaniel T. and {Carr}, Derrick S.},
        title = "{Linking compact dwarf starburst galaxies in the resolve survey to downsized blue nuggets}",
      journal = {\mnras},
     keywords = {galaxies: starburst, galaxies: evolution, galaxies: interactions, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = apr,
          doi = {10.1093/mnras/staa899},
archivePrefix = {arXiv},
       eprint = {2003.12891},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.tmp..167P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Hainline16,
       author = {{Hainline}, Kevin N. and {Reines}, Amy E. and {Greene}, Jenny E. and
         {Stern}, Daniel},
        title = "{Mid-infrared Colors of Dwarf Galaxies: Young Starbursts Mimicking Active Galactic Nuclei}",
      journal = {\apj},
     keywords = {cosmology: observations, galaxies: dwarf, galaxies: evolution, galaxies: nuclei, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = dec,
       volume = {832},
       number = {2},
          eid = {119},
        pages = {119},
          doi = {10.3847/0004-637X/832/2/119},
archivePrefix = {arXiv},
       eprint = {1609.06721},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...832..119H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Habouzit17,
       author = {{Habouzit}, M{\'e}lanie and {Volonteri}, Marta and {Dubois}, Yohan},
        title = "{Blossoms from black hole seeds: properties and early growth regulated by supernova feedback}",
      journal = {\mnras},
     keywords = {black hole physics, methods: numerical, galaxies: evolution, galaxies: formation, galaxies: high redshift, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = jul,
       volume = {468},
       number = {4},
        pages = {3935-3948},
          doi = {10.1093/mnras/stx666},
archivePrefix = {arXiv},
       eprint = {1605.09394},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.468.3935H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Cole00,
    author = {Cole, Shaun and Lacey, Cedric G. and Baugh, Carlton M. and Frenk, Carlos S.},
    title = "{Hierarchical galaxy formation}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {319},
    number = {1},
    pages = {168-204},
    year = {2000},
    month = {11},
    abstract = "{We describe the GALFORM semi-analytic model for calculating the formation and evolution of galaxies in hierarchical clustering cosmologies. It improves upon, and extends, the earlier scheme developed by Cole et al. The model employs a new Monte Carlo algorithm to follow the merging evolution of dark matter haloes with arbitrary mass resolution. It incorporates realistic descriptions of the density profiles of dark matter haloes and the gas they contain; it follows the chemical evolution of gas and stars, and the associated production of dust; and it includes a detailed calculation of the sizes of discs and spheroids. Wherever possible, our prescriptions for modelling individual physical processes are based on results of numerical simulations. They require a number of adjustable parameters, which we fix by reference to a small subset of local galaxy data. This results in a fully specified model of galaxy formation which can be tested against other data. We apply our methods to the ΛCDM cosmology  and find good agreement with a wide range of properties of the local galaxy population: the B- and K-band luminosity functions, the distribution of colours for the population as a whole, the ratio of ellipticals to spirals, the distribution of disc sizes, and the current cold gas content of discs. In spite of the overall success of the model, some interesting discrepancies remain: the colour-magnitude relation for ellipticals in clusters is significantly flatter than observed at bright magnitudes (although the scatter is about right), and the model predicts galaxy circular velocities, at a given luminosity, that are about 30 per cent larger than is observed. It is unclear whether these discrepancies represent fundamental shortcomings of the model, or whether they result from the various approximations and uncertainties inherent in the technique. Our more detailed methods do not change our earlier conclusion that just over half the stars in the Universe are expected to have formed since }",
    issn = {0035-8711},
    doi = {10.1046/j.1365-8711.2000.03879.x},
    url = {https://doi.org/10.1046/j.1365-8711.2000.03879.x},
    eprint = {https://academic.oup.com/mnras/article-pdf/319/1/168/3734609/319-1-168.pdf},
}



@ARTICLE{Kewley02,
   author = {{Kewley}, L.~J. and {Dopita}, M.~A.},
    title = "{Using Strong Lines to Estimate Abundances in Extragalactic H II Regions and Starburst Galaxies}",
  journal = {\apjs},
   eprint = {astro-ph/0206495},
 keywords = {Galaxies: Abundances, Galaxies: Evolution, Galaxies: Starburst, ISM: Abundances},
     year = 2002,
    month = sep,
   volume = 142,
    pages = {35-52},
      doi = {10.1086/341326},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJS..142...35K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Baldassare17,
       author = {{Baldassare}, Vivienne F. and {Reines}, Amy E. and {Gallo}, Elena and
         {Greene}, Jenny E.},
        title = "{X-ray and Ultraviolet Properties of AGNs in Nearby Dwarf Galaxies}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: dwarf, quasars: supermassive black holes, ultraviolet: galaxies, X-rays: galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Feb",
       volume = {836},
       number = {1},
          eid = {20},
        pages = {20},
          doi = {10.3847/1538-4357/836/1/20},
archivePrefix = {arXiv},
       eprint = {1609.07148},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...836...20B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Greene07,
       author = {{Greene}, Jenny E. and {Ho}, Luis C.},
        title = "{A New Sample of Low-Mass Black Holes in Active Galaxies}",
      journal = {\apj},
     keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert, Astrophysics},
         year = "2007",
        month = "Nov",
       volume = {670},
       number = {1},
        pages = {92-104},
          doi = {10.1086/522082},
archivePrefix = {arXiv},
       eprint = {0707.2617},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...670...92G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jiang11,
       author = {{Jiang}, Yan-Fei and {Greene}, Jenny E. and {Ho}, Luis C. and
         {Xiao}, Ting and {Barth}, Aaron J.},
        title = "{The Host Galaxies of Low-mass Black Holes}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: bulges, galaxies: nuclei, galaxies: photometry, galaxies: Seyfert, galaxies: structure, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = "2011",
        month = "Dec",
       volume = {742},
       number = {2},
          eid = {68},
        pages = {68},
          doi = {10.1088/0004-637X/742/2/68},
archivePrefix = {arXiv},
       eprint = {1107.4105},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...742...68J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dong12,
       author = {{Dong}, Xiao-Bo and {Ho}, Luis C. and {Yuan}, Weimin and
         {Wang}, Ting-Gui and {Fan}, Xiaohui and {Zhou}, Hongyan and
         {Jiang}, Ning},
        title = "{A Uniformly Selected Sample of Low-mass Black Holes in Seyfert 1 Galaxies}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: nuclei, galaxies: Seyfert, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "Aug",
       volume = {755},
       number = {2},
          eid = {167},
        pages = {167},
          doi = {10.1088/0004-637X/755/2/167},
archivePrefix = {arXiv},
       eprint = {1206.3843},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...755..167D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Liu18,
       author = {{Liu}, He-Yang and {Yuan}, Weimin and {Dong}, Xiao-Bo and
         {Zhou}, Hongyan and {Liu}, Wen-Juan},
        title = "{A Uniformly Selected Sample of Low-mass Black Holes in Seyfert 1 Galaxies. II. The SDSS DR7 Sample}",
      journal = {\apjs},
     keywords = {galaxies: active, galaxies: nuclei, galaxies: Seyfert, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Apr",
       volume = {235},
       number = {2},
          eid = {40},
        pages = {40},
          doi = {10.3847/1538-4365/aab88e},
archivePrefix = {arXiv},
       eprint = {1803.04330},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..235...40L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Liu17,
   author = {{Liu}, W.-J. and {Qian}, L. and {Dong}, X.-B. and {Jiang}, N. and 
	{Lira}, P. and {Cai}, Z. and {Wang}, F. and {Yang}, J. and {Xiao}, T. and 
	{Kim}, M.},
    title = "{A Ringed Dwarf LINER 1 Galaxy Hosting an Intermediate-mass Black Hole with Large-scale Rotation-like H{$\alpha$} Emission}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1702.01033},
 keywords = {galaxies: active, galaxies: dwarf, galaxies: individual: SDSS J083803.68+540642.0, galaxies: nuclei, galaxies: Seyfert},
     year = 2017,
    month = mar,
   volume = 837,
      eid = {109},
    pages = {109},
      doi = {10.3847/1538-4357/aa5eb6},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...837..109L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Kormendy04,
       author = {{Kormendy}, John and {Kennicutt}, Robert C., Jr.},
        title = "{Secular Evolution and the Formation of Pseudobulges in Disk Galaxies}",
      journal = {\araa},
     keywords = {Astrophysics},
         year = "2004",
        month = "Sep",
       volume = {42},
       number = {1},
        pages = {603-683},
          doi = {10.1146/annurev.astro.42.053102.134024},
archivePrefix = {arXiv},
       eprint = {astro-ph/0407343},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ARA&A..42..603K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Manzano-King19,
       author = {{Manzano-King}, Christina and {Canalizo}, Gabriela and {Sales}, Laura V.},
        title = "{AGN-Driven Outflows in Dwarf Galaxies}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "May",
          eid = {arXiv:1905.09287},
        pages = {arXiv:1905.09287},
archivePrefix = {arXiv},
       eprint = {1905.09287},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190509287M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Trebitsch18,
       author = {{Trebitsch}, Maxime and {Volonteri}, Marta and {Dubois}, Yohan and
         {Madau}, Piero},
        title = "{Escape of ionizing radiation from high-redshift dwarf galaxies: role of AGN feedback}",
      journal = {\mnras},
     keywords = {radiative transfer, galaxies: formation, galaxies: high-redshift, quasars: supermassive black holes, dark ages, reionization, first stars, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2018",
        month = "Aug",
       volume = {478},
       number = {4},
        pages = {5607-5625},
          doi = {10.1093/mnras/sty1406},
archivePrefix = {arXiv},
       eprint = {1712.05804},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.478.5607T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bower06,
       author = {{Bower}, R.~G. and {Benson}, A.~J. and {Malbon}, R. and {Helly}, J.~C. and
         {Frenk}, C.~S. and {Baugh}, C.~M. and {Cole}, S. and {Lacey}, C.~G.},
        title = "{Breaking the hierarchy of galaxy formation}",
      journal = {\mnras},
     keywords = {galaxies: evolution: galaxies: formation: galaxies: luminosity function, galaxies: evolution, galaxies: formation, galaxies: luminosity function, Astrophysics},
         year = "2006",
        month = "Aug",
       volume = {370},
       number = {2},
        pages = {645-655},
          doi = {10.1111/j.1365-2966.2006.10519.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0511338},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MNRAS.370..645B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dashyan18,
       author = {{Dashyan}, Gohar and {Silk}, Joseph and {Mamon}, Gary A. and
         {Dubois}, Yohan and {Hartwig}, Tilman},
        title = "{AGN feedback in dwarf galaxies?}",
      journal = {\mnras},
     keywords = {black hole physics, methods: analytical, galaxies: active, galaxies: dwarf, galaxies: evolution, galaxies: luminosity function, mass function, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Feb",
       volume = {473},
       number = {4},
        pages = {5698-5703},
          doi = {10.1093/mnras/stx2716},
archivePrefix = {arXiv},
       eprint = {1710.05900},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.473.5698D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bradford18,
       author = {{Bradford}, Jeremy D. and {Geha}, Marla C. and {Greene}, Jenny E. and
         {Reines}, Amy E. and {Dickey}, Claire M.},
        title = "{The Effect of AGNs on the Global H I Content of Isolated Low-mass Galaxies}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: evolution, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Jul",
       volume = {861},
       number = {1},
          eid = {50},
        pages = {50},
          doi = {10.3847/1538-4357/aac88d},
archivePrefix = {arXiv},
       eprint = {1805.10874},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...861...50B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Penny18,
       author = {{Penny}, Samantha J. and {Masters}, Karen L. and {Smethurst}, Rebecca and
         {Nichol}, Robert C. and {Krawczyk}, Coleman M. and {Bizyaev}, Dmitry and
         {Greene}, Olivia and {Liu}, Charles and {Marinelli}, Mariarosa and
         {Rembold}, Sandro B. and {Riffel}, Rogemar A. and
         {Ilha}, Gabriele da Silva and {Wylezalek}, Dominika and
         {Andrews}, Brett H. and {Bundy}, Kevin and {Drory}, Niv and
         {Oravetz}, Daniel and {Pan}, Kaike},
        title = "{SDSS-IV MaNGA: evidence of the importance of AGN feedback in low-mass galaxies}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: dwarf, galaxies: evolution, galaxies: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "May",
       volume = {476},
       number = {1},
        pages = {979-998},
          doi = {10.1093/mnras/sty202},
archivePrefix = {arXiv},
       eprint = {1710.07568},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.476..979P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Vogt17,
       author = {{Vogt}, F.~P.~A. and {P{\'e}rez}, E. and {Dopita}, M.~A. and
         {Verdes-Montenegro}, L. and {Borthakur}, S.},
        title = "{Evidence for azimuthal variations of the oxygen-abundance gradient tracing the spiral structure of the galaxy HCG 91c}",
      journal = {\aap},
     keywords = {ISM: abundances, HII regions, galaxies: groups: individual: HCG 91, galaxies: ISM, galaxies: spiral, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "May",
       volume = {601},
          eid = {A61},
        pages = {A61},
          doi = {10.1051/0004-6361/201629853},
archivePrefix = {arXiv},
       eprint = {1701.01728},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...601A..61V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lacerda18,
       author = {{Lacerda}, E.~A.~D. and {Cid Fernandes}, R. and {Couto}, G.~S. and
         {Stasi{\'n}ska}, G. and {Garc{\'\i}a-Benito}, R. and {Vale Asari}, N. and
         {P{\'e}rez}, E. and {Gonz{\'a}lez Delgado}, R.~M. and
         {S{\'a}nchez}, S.~F. and {de Amorim}, A.~L.},
        title = "{Diffuse ionized gas in galaxies across the Hubble sequence at the CALIFA resolution}",
      journal = {\mnras},
     keywords = {surveys, ISM: general, galaxies: ISM, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Mar",
       volume = {474},
       number = {3},
        pages = {3727-3739},
          doi = {10.1093/mnras/stx3022},
archivePrefix = {arXiv},
       eprint = {1711.07844},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.474.3727L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kaplan16,
       author = {{Kaplan}, Kyle F. and {Jogee}, Shardha and {Kewley}, Lisa and
         {Blanc}, Guillermo A. and {Weinzirl}, Tim and {Song}, Mimi and
         {Drory}, Niv and {Luo}, Rongxin and {van den Bosch}, Remco C.~E.},
        title = "{The VIRUS-P Exploration of Nearby Galaxies (VENGA): spatially resolved gas-phase metallicity distributions in barred and unbarred spirals}",
      journal = {\mnras},
     keywords = {galaxies: abundances, galaxies: ISM, galaxies: spiral, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Oct",
       volume = {462},
       number = {2},
        pages = {1642-1682},
          doi = {10.1093/mnras/stw1422},
archivePrefix = {arXiv},
       eprint = {1606.05713},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.462.1642K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mierkiewicz06,
       author = {{Mierkiewicz}, E.~J. and {Reynolds}, R.~J. and {Roesler}, F.~L. and
         {Harlander}, J.~M. and {Jaehnig}, K.~P.},
        title = "{Detection of Diffuse Interstellar [O II] Emission from the Milky Way Using Spatial Heterodyne Spectroscopy}",
      journal = {\apjl},
     keywords = {ISM: General, ISM: Structure},
         year = "2006",
        month = "Oct",
       volume = {650},
       number = {1},
        pages = {L63-L66},
          doi = {10.1086/508745},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...650L..63M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reynolds92,
       author = {{Reynolds}, R.~J. and {Cox}, D.~P.},
        title = "{Heating the Warm Ionized Medium}",
      journal = {\apjl},
     keywords = {H I Regions, Heating, Interstellar Matter, Ionized Gases, Photoionization, Cosmic Dust, Electron Density (Concentration), Forbidden Bands, Interstellar Gas, Astrophysics, ATOMIC PROCESSES, GALAXIES: INTERSTELLAR MATTER, ISM: H II REGIONS, ISM: GENERAL},
         year = "1992",
        month = "Nov",
       volume = {400},
        pages = {L33},
          doi = {10.1086/186642},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992ApJ...400L..33R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zhang17,
       author = {{Zhang}, Kai and {Yan}, Renbin and {Bundy}, Kevin and
         {Bershady}, Matthew and {Haffner}, L. Matthew and
         {Walterbos}, Ren{\'e} and {Maiolino}, Roberto and {Tremonti}, Christy and
         {Thomas}, Daniel and {Drory}, Niv and {Jones}, Amy and
         {Belfiore}, Francesco and {S{\'a}nchez}, Sebastian F. and
         {Diamond-Stanic}, Aleksandar M. and {Bizyaev}, Dmitry and
         {Nitschelm}, Christian and {Andrews}, Brett and {Brinkmann}, Jon and
         {Brownstein}, Joel R. and {Cheung}, Edmond and {Li}, Cheng and
         {Law}, David R. and {Roman Lopes}, Alexandre and {Oravetz}, Daniel and
         {Pan}, Kaike and {Storchi Bergmann}, Thaisa and {Simmons}, Audrey},
        title = "{SDSS-IV MaNGA: the impact of diffuse ionized gas on emission-line ratios, interpretation of diagnostic diagrams and gas metallicity measurements}",
      journal = {\mnras},
     keywords = {galaxies: abundances, galaxies: active, galaxies: evolution, galaxies: fundamental parameters, galaxies: ISM, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Apr",
       volume = {466},
       number = {3},
        pages = {3217-3243},
          doi = {10.1093/mnras/stw3308},
archivePrefix = {arXiv},
       eprint = {1612.02000},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.466.3217Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Heckman80,
       author = {{Heckman}, T.~M.},
        title = "{An optical and radio survey of the nuclei of bright galaxies. Activity in normal galactic nuclei.}",
      journal = {\aap},
     keywords = {Astronomical Spectroscopy, Galactic Nuclei, Optical Measurement, Radio Astronomy, Radio Galaxies, Emission Spectra, H Ii Regions, Luminous Intensity, Nonthermal Radiation, Seyfert Galaxies, Shock Wave Propagation, Spectral Line Width, Spectrophotometry, Astrophysics},
         year = "1980",
        month = "Jul",
       volume = {500},
        pages = {187-199},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1980A&A....87..152H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ho03,
       author = {{Ho}, Luis C. and {Filippenko}, Alexei V. and {Sargent}, Wallace L.~W.},
        title = "{A Search for ``Dwarf'' Seyfert Nuclei. VI. Properties of Emission-Line Nuclei in Nearby Galaxies}",
      journal = {\apj},
     keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert, Galaxies: Starburst, Surveys, Astrophysics},
         year = "2003",
        month = "Jan",
       volume = {583},
       number = {1},
        pages = {159-177},
          doi = {10.1086/345354},
archivePrefix = {arXiv},
       eprint = {astro-ph/0210048},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...583..159H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Goulding09,
       author = {{Goulding}, A.~D. and {Alexander}, D.~M.},
        title = "{Towards a complete census of AGN in nearby Galaxies: a large population of optically unidentified AGN}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: evolution, galaxies: nuclei, infrared: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2009",
        month = "Sep",
       volume = {398},
       number = {3},
        pages = {1165-1193},
          doi = {10.1111/j.1365-2966.2009.15194.x},
archivePrefix = {arXiv},
       eprint = {0906.0772},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009MNRAS.398.1165G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Sarzi10,
       author = {{Sarzi}, Marc and {Shields}, Joseph C. and {Schawinski}, Kevin and
         {Jeong}, Hyunjin and {Shapiro}, Kristen and {Bacon}, Roland and
         {Bureau}, Martin and {Cappellari}, Michele and {Davies}, Roger L. and
         {de Zeeuw}, P. Tim and {Emsellem}, Eric and
         {Falc{\'o}n-Barroso}, Jes{\'u}s and {Krajnovi{\'c}}, Davor and
         {Kuntschner}, Harald and {McDermid}, Richard M. and
         {Peletier}, Reynier F. and {van den Bosch}, Remco C.~E. and
         {van de Ven}, Glen and {Yi}, Sukyoung K.},
        title = "{The SAURON project - XVI. On the sources of ionization for the gas in elliptical and lenticular galaxies}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: elliptical and lenticular, cD, galaxies: ISM, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2010",
        month = "Mar",
       volume = {402},
       number = {4},
        pages = {2187-2210},
          doi = {10.1111/j.1365-2966.2009.16039.x},
archivePrefix = {arXiv},
       eprint = {0912.0275},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.402.2187S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dopita95,
       author = {{Dopita}, Michael A. and {Sutherland}, Ralph S.},
        title = "{Spectral Signatures of Fast Shocks. II. Optical Diagnostic Diagrams}",
      journal = {\apj},
     keywords = {GALAXIES: ACTIVE, GALAXIES: SEYFERT, SHOCK WAVES},
         year = "1995",
        month = "Dec",
       volume = {455},
        pages = {468},
          doi = {10.1086/176596},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...455..468D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Ho08,
       author = {{Ho}, L.~C.},
        title = "{Nuclear activity in nearby galaxies.}",
      journal = {\araa},
     keywords = {Astrophysics},
         year = "2008",
        month = "Sep",
       volume = {46},
        pages = {475-539},
          doi = {10.1146/annurev.astro.45.051806.110546},
archivePrefix = {arXiv},
       eprint = {0803.2268},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ARA&A..46..475H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rupke11,
       author = {{Rupke}, David S.~N. and {Veilleux}, Sylvain},
        title = "{Integral Field Spectroscopy of Massive, Kiloparsec-scale Outflows in the Infrared-luminous QSO Mrk 231}",
      journal = {\apjl},
     keywords = {galaxies: evolution, galaxies: ISM, galaxies: jets, galaxies: kinematics and dynamics, quasars: individual: Mrk 231, Astrophysics - Galaxy Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = "2011",
        month = "Mar",
       volume = {729},
       number = {2},
          eid = {L27},
        pages = {L27},
          doi = {10.1088/2041-8205/729/2/L27},
archivePrefix = {arXiv},
       eprint = {1102.4349},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...729L..27R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Heckman87,
   author = {{Heckman}, T.~M. and {Armus}, L. and {Miley}, G.~K.},
    title = "{Evidence for large-scale winds from starburst galaxies. II - an optical investigation of powerful far-infrared galaxies}",
  journal = {\aj},
 keywords = {Far Infrared Radiation, Galactic Evolution, Infrared Spectra, Star Formation, Starburst Galaxies, Stellar Winds, Visible Spectrum, Astronomical Models, Astronomical Spectroscopy, H Alpha Line, H Ii Regions, Spectral Energy Distribution},
     year = 1987,
    month = feb,
   volume = 93,
    pages = {276-283},
      doi = {10.1086/114310},
   adsurl = {https://ui.adsabs.harvard.edu/abs/1987AJ.....93..276H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Cecil02,
       author = {{Cecil}, Gerald and {Dopita}, Michael A. and {Groves}, Brent and
         {Wilson}, Andrew S. and {Ferruit}, Pierre and {P{\'e}contal}, Emmanuel and
         {Binette}, Luc},
        title = "{Spatial Resolution of High-Velocity Filaments in the Narrow-Line Region of NGC 1068: Associated Absorbers Caught in Emission?}",
      journal = {\apj},
     keywords = {Galaxies: Active, Galaxies: Individual: NGC Number: NGC 1068, Galaxies: Jets, Galaxies: Kinematics and Dynamics, Galaxies: Seyfert, Astrophysics},
         year = "2002",
        month = "Apr",
       volume = {568},
       number = {2},
        pages = {627-638},
          doi = {10.1086/338950},
archivePrefix = {arXiv},
       eprint = {astro-ph/0112256},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...568..627C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rupke05,
       author = {{Rupke}, David S. and {Veilleux}, Sylvain and {Sanders}, D.~B.},
        title = "{Outflows in Infrared-Luminous Starbursts at z \&lt; 0.5. II. Analysis and Discussion}",
      journal = {\apjs},
     keywords = {Galaxies: Starburst, Infrared: Galaxies, ISM: Jets and Outflows, ISM: Kinematics and Dynamics, Astrophysics},
         year = "2005",
        month = "Sep",
       volume = {160},
       number = {1},
        pages = {115-148},
          doi = {10.1086/432889},
archivePrefix = {arXiv},
       eprint = {astro-ph/0506611},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJS..160..115R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rupke13,
       author = {{Rupke}, David S.~N. and {Veilleux}, Sylvain},
        title = "{The Multiphase Structure and Power Sources of Galactic Winds in Major Mergers}",
      journal = {\apj},
     keywords = {galaxies: evolution, galaxies: interactions, galaxies: ISM, galaxies: kinematics and dynamics, ISM: jets and outflows, quasars: general, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2013",
        month = "May",
       volume = {768},
       number = {1},
          eid = {75},
        pages = {75},
          doi = {10.1088/0004-637X/768/1/75},
archivePrefix = {arXiv},
       eprint = {1303.6866},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...768...75R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rich11,
       author = {{Rich}, J.~A. and {Kewley}, L.~J. and {Dopita}, M.~A.},
        title = "{Galaxy-wide Shocks in Late-merger Stage Luminous Infrared Galaxies}",
      journal = {\apj},
     keywords = {galaxies: evolution, galaxies: individual: NGC 3256 IC 1623, galaxies: ISM, shock waves, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2011",
        month = "Jun",
       volume = {734},
       number = {2},
          eid = {87},
        pages = {87},
          doi = {10.1088/0004-637X/734/2/87},
archivePrefix = {arXiv},
       eprint = {1104.1177},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...734...87R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Davies17,
       author = {{Davies}, Rebecca L. and {Groves}, Brent and {Kewley}, Lisa J. and
         {Medling}, Anne M. and {Shastri}, Prajval and {Maithil}, Jaya and
         {Kharb}, Preeti and {Banfield}, Julie and {Longbottom}, Fergus and
         {Dopita}, Michael A. and {Hampton}, Elise J. and
         {Scharw{\"a}chter}, Julia and {Sutherland}, Ralph and {Jin}, Chichuan and
         {Zaw}, Ingyin and {James}, Bethan and {Juneau}, St{\'e}phanie},
        title = "{Dissecting galaxies: separating star formation, shock excitation and AGN activity in the central region of NGC 613}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: ISM, galaxies: Seyfert, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Oct",
       volume = {470},
       number = {4},
        pages = {4974-4988},
          doi = {10.1093/mnras/stx1559},
archivePrefix = {arXiv},
       eprint = {1707.03404},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.470.4974D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rich10,
       author = {{Rich}, J.~A. and {Dopita}, M.~A. and {Kewley}, L.~J. and
         {Rupke}, D.~S.~N.},
        title = "{NGC 839: Shocks in an M82-like Superwind}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: evolution, galaxies: individual: NGC 839, galaxies: ISM, ISM: jets and outflows, shock waves, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2010",
        month = "Sep",
       volume = {721},
       number = {1},
        pages = {505-517},
          doi = {10.1088/0004-637X/721/1/505},
archivePrefix = {arXiv},
       eprint = {1007.3495},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...721..505R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kewley13,
       author = {{Kewley}, Lisa J. and {Dopita}, Michael A. and {Leitherer}, Claus and
         {Dav{\'e}}, Romeel and {Yuan}, Tiantian and {Allen}, Mark and
         {Groves}, Brent and {Sutherland}, Ralph},
        title = "{Theoretical Evolution of Optical Strong Lines across Cosmic Time}",
      journal = {\apj},
     keywords = {galaxies: abundances, galaxies: fundamental parameters, galaxies: starburst, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2013",
        month = "Sep",
       volume = {774},
       number = {2},
          eid = {100},
        pages = {100},
          doi = {10.1088/0004-637X/774/2/100},
archivePrefix = {arXiv},
       eprint = {1307.0508},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...774..100K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DAgostino192,
       author = {{D'Agostino}, Joshua J. and {Kewley}, Lisa J. and {Groves}, Brent A. and
         {Medling}, Anne and {Dopita}, Michael A. and {Thomas}, Adam D.},
        title = "{A new diagnostic to separate line emission from star formation, shocks, and AGNs simultaneously in IFU data}",
      journal = {\mnras},
     keywords = {ISM: jets and outflows, galaxies: active, galaxies: evolution, galaxies: ISM, galaxies: Seyfert, galaxies: star formation, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "May",
       volume = {485},
       number = {1},
        pages = {L38-L42},
          doi = {10.1093/mnrasl/slz028},
archivePrefix = {arXiv},
       eprint = {1902.10295},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.485L..38D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{DAgostino191,
       author = {{D'Agostino}, Joshua J. and {Kewley}, Lisa J. and {Groves}, Brent A. and
         {Medling}, Anne M. and {Di Teodoro}, Enrico and {Dopita}, Michael A. and
         {Thomas}, Adam D. and {Sutherland}, Ralph S. and
         {Garcia-Burillo}, Santiago},
        title = "{Separating line emission from star formation, shocks, and AGN ionization in NGC 1068}",
      journal = {\mnras},
     keywords = {ISM: jets and outflows, galaxies: active, galaxies: evolution, galaxies: ISM, galaxies: Seyfert, galaxies: star formation, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Aug",
       volume = {487},
       number = {3},
        pages = {4153-4168},
          doi = {10.1093/mnras/stz1611},
archivePrefix = {arXiv},
       eprint = {1906.07907},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.487.4153D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kormendy13,
       author = {{Kormendy}, John and {Ho}, Luis C.},
        title = "{Coevolution (Or Not) of Supermassive Black Holes and Host Galaxies}",
      journal = {\araa},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2013",
        month = "Aug",
       volume = {51},
       number = {1},
        pages = {511-653},
          doi = {10.1146/annurev-astro-082708-101811},
archivePrefix = {arXiv},
       eprint = {1304.7762},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ARA&A..51..511K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Tremmel17,
       author = {{Tremmel}, M. and {Karcher}, M. and {Governato}, F. and {Volonteri}, M. and
         {Quinn}, T.~R. and {Pontzen}, A. and {Anderson}, L. and {Bellovary}, J.},
        title = "{The Romulus cosmological simulations: a physical approach to the formation, dynamics and accretion models of SMBHs}",
      journal = {\mnras},
     keywords = {methods: numerical, galaxies: general, quasars: supermassive black holes, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Sep",
       volume = {470},
       number = {1},
        pages = {1121-1139},
          doi = {10.1093/mnras/stx1160},
archivePrefix = {arXiv},
       eprint = {1607.02151},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.470.1121T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Satyapal14,
       author = {{Satyapal}, S. and {Secrest}, N.~J. and {McAlpine}, W. and
         {Ellison}, S.~L. and {Fischer}, J. and {Rosenberg}, J.~L.},
        title = "{Discovery of a Population of Bulgeless Galaxies with Extremely Red Mid-IR Colors: Obscured AGN Activity in the Low-mass Regime?}",
      journal = {\apj},
     keywords = {black hole physics, galaxies: active, galaxies: spiral, infrared: galaxies, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2014",
        month = "Apr",
       volume = {784},
       number = {2},
          eid = {113},
        pages = {113},
          doi = {10.1088/0004-637X/784/2/113},
archivePrefix = {arXiv},
       eprint = {1401.5483},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...784..113S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Moran14,
       author = {{Moran}, Edward C. and {Shahinyan}, Karlen and {Sugarman}, Hannah R. and
         {V{\'e}lez}, Darik O. and {Eracleous}, Michael},
        title = "{Black Holes At the Centers of Nearby Dwarf Galaxies}",
      journal = {\aj},
     keywords = {galaxies: active, galaxies: dwarf, galaxies: Seyfert, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2014",
        month = "Dec",
       volume = {148},
       number = {6},
          eid = {136},
        pages = {136},
          doi = {10.1088/0004-6256/148/6/136},
archivePrefix = {arXiv},
       eprint = {1408.4451},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014AJ....148..136M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Dalcanton04,
       author = {{Dalcanton}, Julianne J. and {Yoachim}, Peter and
         {Bernstein}, Rebecca A.},
        title = "{The Formation of Dust Lanes: Implications for Galaxy Evolution}",
      journal = {\apj},
     keywords = {ISM: Dust, Extinction, Galaxies: Formation, Galaxies: ISM, Galaxies: Spiral, ISM: Structure, Stars: Formation, Astrophysics},
         year = "2004",
        month = "Jun",
       volume = {608},
       number = {1},
        pages = {189-207},
          doi = {10.1086/386358},
archivePrefix = {arXiv},
       eprint = {astro-ph/0402472},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...608..189D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Levesque10,
       author = {{Levesque}, Emily M. and {Kewley}, Lisa J. and {Larson}, Kirsten L.},
        title = "{Theoretical Modeling of Star-Forming Galaxies. I. Emission-Line Diagnostic Grids for Local and Low-Metallicity Galaxies}",
      journal = {\aj},
     keywords = {galaxies: ISM, galaxies: starburst, Astrophysics - Astrophysics of Galaxies},
         year = "2010",
        month = "Feb",
       volume = {139},
       number = {2},
        pages = {712-727},
          doi = {10.1088/0004-6256/139/2/712},
archivePrefix = {arXiv},
       eprint = {0908.0460},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010AJ....139..712L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Gutkin16,
       author = {{Gutkin}, Julia and {Charlot}, St{\'e}phane and {Bruzual}, Gustavo},
        title = "{Modelling the nebular emission from primeval to present-day star-forming galaxies}",
      journal = {\mnras},
     keywords = {galaxies: abundances, galaxies: general, galaxies: high-redshift, galaxies: ISM, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Oct",
       volume = {462},
       number = {2},
        pages = {1757-1774},
          doi = {10.1093/mnras/stw1716},
archivePrefix = {arXiv},
       eprint = {1607.06086},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.462.1757G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{DeCia16,
       author = {{De Cia}, A. and {Ledoux}, C. and {Mattsson}, L. and {Petitjean}, P. and
         {Srianand}, R. and {Gavignaud}, I. and {Jenkins}, E.~B.},
        title = "{Dust-depletion sequences in damped Lyman-{\ensuremath{\alpha}} absorbers. A unified picture from low-metallicity systems to the Galaxy}",
      journal = {\aap},
     keywords = {ISM: abundances, dust, extinction, quasars: absorption lines, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = "2016",
        month = "Dec",
       volume = {596},
          eid = {A97},
        pages = {A97},
          doi = {10.1051/0004-6361/201527895},
archivePrefix = {arXiv},
       eprint = {1608.08621},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...596A..97D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Pilyugin14,
       author = {{Pilyugin}, L.~S. and {Grebel}, E.~K. and {Zinchenko}, I.~A. and
         {Kniazev}, A.~Y.},
        title = "{The Abundance Properties of Nearby Late-Type Galaxies. II. the Relation between Abundance Distributions and Surface Brightness Profiles}",
      journal = {\aj},
     keywords = {galaxies: abundances, galaxies: photometry, galaxies: spiral, Astrophysics - Astrophysics of Galaxies},
         year = "2014",
        month = "Dec",
       volume = {148},
       number = {6},
          eid = {134},
        pages = {134},
          doi = {10.1088/0004-6256/148/6/134},
archivePrefix = {arXiv},
       eprint = {1408.6413},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014AJ....148..134P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Cresci18,
       author = {{Cresci}, Giovanni and {Mannucci}, Filippo and {Curti}, Mirko},
        title = "{The ``Fundamental Metallicity Relation'' in CALIFA, SDSS-IV MaNGA and high-z galaxies}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Nov",
          eid = {arXiv:1811.06015},
        pages = {arXiv:1811.06015},
archivePrefix = {arXiv},
       eprint = {1811.06015},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv181106015C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Salim14,
       author = {{Salim}, Samir and {Lee}, Janice C. and {Ly}, Chun and
         {Brinchmann}, Jarle and {Dav{\'e}}, Romeel and {Dickinson}, Mark and
         {Salzer}, John J. and {Charlot}, St{\'e}phane},
        title = "{A Critical Look at the Mass-Metallicity-Star Formation Rate Relation in the Local Universe. I. An Improved Analysis Framework and Confounding Systematics}",
      journal = {\apj},
     keywords = {galaxies: abundances, galaxies: evolution, galaxies: fundamental parameters, Astrophysics - Astrophysics of Galaxies},
         year = "2014",
        month = "Dec",
       volume = {797},
       number = {2},
          eid = {126},
        pages = {126},
          doi = {10.1088/0004-637X/797/2/126},
archivePrefix = {arXiv},
       eprint = {1411.7391},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...797..126S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yates12,
       author = {{Yates}, Robert M. and {Kauffmann}, Guinevere and {Guo}, Qi},
        title = "{The relation between metallicity, stellar mass and star formation in galaxies: an analysis of observational and model data}",
      journal = {\mnras},
     keywords = {ISM: abundances, galaxies: abundances, galaxies: evolution, galaxies: fundamental parameters, galaxies: star formation, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "May",
       volume = {422},
       number = {1},
        pages = {215-231},
          doi = {10.1111/j.1365-2966.2012.20595.x},
archivePrefix = {arXiv},
       eprint = {1107.3145},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.422..215Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lara10,
       author = {{Lara-L{\'o}pez}, M.~A. and {Cepa}, J. and {Bongiovanni}, A. and
         {P{\'e}rez Garc{\'\i}a}, A.~M. and {Ederoclite}, A. and
         {Casta{\~n}eda}, H. and {Fern{\'a}ndez Lorenzo}, M. and
         {Povi{\'c}}, M. and {S{\'a}nchez-Portal}, M.},
        title = "{A fundamental plane for field star-forming galaxies}",
      journal = {\aap},
     keywords = {galaxies: fundamental parameters, galaxies: abundances, galaxies: starburst, galaxies: star formation, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2010",
        month = "Oct",
       volume = {521},
          eid = {L53},
        pages = {L53},
          doi = {10.1051/0004-6361/201014803},
archivePrefix = {arXiv},
       eprint = {1005.0509},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...521L..53L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mannucci11,
       author = {{Mannucci}, F. and {Salvaterra}, R. and {Campisi}, M.~A.},
        title = "{The metallicity of the long GRB hosts and the fundamental metallicity relation of low-mass galaxies}",
      journal = {\mnras},
     keywords = {galaxies: abundances, galaxies: star formation, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2011",
        month = "Jun",
       volume = {414},
       number = {2},
        pages = {1263-1268},
          doi = {10.1111/j.1365-2966.2011.18459.x},
archivePrefix = {arXiv},
       eprint = {1011.4506},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.414.1263M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bellovary19,
       author = {{Bellovary}, Jillian M. and {Cleary}, Colleen E. and {Munshi}, Ferah and
         {Tremmel}, Michael and {Christensen}, Charlotte R. and
         {Brooks}, Alyson and {Quinn}, Thomas R.},
        title = "{Multimessenger signatures of massive black holes in dwarf galaxies}",
      journal = {\mnras},
     keywords = {black hole physics, gravitational waves, galaxies: dwarf, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2019",
        month = "Jan",
       volume = {482},
       number = {3},
        pages = {2913-2923},
          doi = {10.1093/mnras/sty2842},
archivePrefix = {arXiv},
       eprint = {1806.00471},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.482.2913B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Stern12,
       author = {{Stern}, Daniel and {Assef}, Roberto J. and {Benford}, Dominic J. and
         {Blain}, Andrew and {Cutri}, Roc and {Dey}, Arjun and
         {Eisenhardt}, Peter and {Griffith}, Roger L. and {Jarrett}, T.~H. and
         {Lake}, Sean and {Masci}, Frank and {Petty}, Sara and
         {Stanford}, S.~A. and {Tsai}, Chao-Wei and {Wright}, E.~L. and
         {Yan}, Lin and {Harrison}, Fiona and {Madsen}, Kristin},
        title = "{Mid-infrared Selection of Active Galactic Nuclei with the Wide-Field Infrared Survey Explorer. I. Characterizing WISE-selected Active Galactic Nuclei in COSMOS}",
      journal = {\apj},
     keywords = {galaxies: active, infrared: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "Jul",
       volume = {753},
       number = {1},
          eid = {30},
        pages = {30},
          doi = {10.1088/0004-637X/753/1/30},
archivePrefix = {arXiv},
       eprint = {1205.0811},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...753...30S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jarrett11,
       author = {{Jarrett}, T.~H. and {Cohen}, M. and {Masci}, F. and {Wright}, E. and
         {Stern}, D. and {Benford}, D. and {Blain}, A. and {Carey}, S. and
         {Cutri}, R.~M. and {Eisenhardt}, P. and {Lonsdale}, C. and
         {Mainzer}, A. and {Marsh}, K. and {Padgett}, D. and {Petty}, S. and
         {Ressler}, M. and {Skrutskie}, M. and {Stanford}, S. and {Surace}, J. and
         {Tsai}, C.~W. and {Wheelock}, S. and {Yan}, D.~L.},
        title = "{The Spitzer-WISE Survey of the Ecliptic Poles}",
      journal = {\apj},
     keywords = {catalogs, galaxies: photometry, galaxies: statistics, stars: statistics, surveys},
         year = "2011",
        month = "Jul",
       volume = {735},
       number = {2},
          eid = {112},
        pages = {112},
          doi = {10.1088/0004-637X/735/2/112},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...735..112J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Mannucci10,
       author = {{Mannucci}, F. and {Cresci}, G. and {Maiolino}, R. and {Marconi}, A. and
         {Gnerucci}, A.},
        title = "{A fundamental relation between mass, star formation rate and metallicity in local and high-redshift galaxies}",
      journal = {\mnras},
     keywords = {galaxies: abundances, galaxies: formation, galaxies: high-redshift, galaxies: starburst, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2010",
        month = "Nov",
       volume = {408},
       number = {4},
        pages = {2115-2127},
          doi = {10.1111/j.1365-2966.2010.17291.x},
archivePrefix = {arXiv},
       eprint = {1005.0006},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.408.2115M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kannappan09,
       author = {{Kannappan}, Sheila J. and {Guie}, Jocelly M. and {Baker}, Andrew J.},
        title = "{E/S0 Galaxies on the Blue Color-Stellar Mass Sequence at z = 0: Fading Mergers or Future Spirals?}",
      journal = {\aj},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = "2009",
        month = "Aug",
       volume = {138},
       number = {2},
        pages = {579-597},
          doi = {10.1088/0004-6256/138/2/579},
archivePrefix = {arXiv},
       eprint = {0903.3695},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009AJ....138..579K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Geha12,
       author = {{Geha}, M. and {Blanton}, M.~R. and {Yan}, R. and {Tinker}, J.~L.},
        title = "{A Stellar Mass Threshold for Quenching of Field Galaxies}",
      journal = {\apj},
     keywords = {galaxies: dwarf, galaxies: stellar content, methods: statistical, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "Sep",
       volume = {757},
       number = {1},
          eid = {85},
        pages = {85},
          doi = {10.1088/0004-637X/757/1/85},
archivePrefix = {arXiv},
       eprint = {1206.3573},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...757...85G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Denicolo02,
       author = {{Denicol{\'o}}, Glenda and {Terlevich}, Roberto and {Terlevich}, Elena},
        title = "{New light on the search for low-metallicity galaxies - I. The N2 calibrator}",
      journal = {\mnras},
     keywords = {GALAXIES: ABUNDANCES, GALAXIES: EVOLUTION, GALAXIES: STELLAR CONTENT, Astrophysics},
         year = "2002",
        month = "Feb",
       volume = {330},
       number = {1},
        pages = {69-74},
          doi = {10.1046/j.1365-8711.2002.05041.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0110356},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002MNRAS.330...69D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Ciardi97,
       author = {{Ciardi}, Benedetta and {Ferrara}, Andrea},
        title = "{Ly{\ensuremath{\alpha}} Clouds Associated with Population III Objects in Cold Dark Matter Models}",
      journal = {\apj},
     keywords = {COSMOLOGY: THEORY, DARK MATTER, GALAXIES: QUASARS: ABSORPTION LINES, Cosmology: Theory, Cosmology: Dark Matter, Galaxies: Quasars: Absorption Lines, Astrophysics},
         year = "1997",
        month = "Jul",
       volume = {483},
       number = {1},
        pages = {L5-L8},
          doi = {10.1086/310728},
archivePrefix = {arXiv},
       eprint = {astro-ph/9703112},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...483L...5C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{MacLow99,
       author = {{Mac Low}, Mordecai-Mark and {Ferrara}, Andrea},
        title = "{Starburst-driven Mass Loss from Dwarf Galaxies: Efficiency and Metal Ejection}",
      journal = {\apj},
     keywords = {GALAXIES: EVOLUTION, GALAXIES: STARBURST, GALAXIES: STELLAR CONTENT, HYDRODYNAMICS, STARS: SUPERNOVAE: GENERAL, Galaxies: Evolution, Galaxies: Starburst, Galaxies: Stellar Content, Hydrodynamics, Stars: Supernovae: General, Astrophysics},
         year = "1999",
        month = "Mar",
       volume = {513},
       number = {1},
        pages = {142-155},
          doi = {10.1086/306832},
archivePrefix = {arXiv},
       eprint = {astro-ph/9801237},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...513..142M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bettoni03,
       author = {{Bettoni}, D. and {Galletta}, G. and {Garc{\'\i}a-Burillo}, S.},
        title = "{A new catalogue of ISM content of normal galaxies}",
      journal = {\aap},
     keywords = {catalogs, galaxies: ISM, galaxies: general, infrared: galaxies, radio lines: galaxies, X-rays: galaxies, submillimeter, Astrophysics},
         year = "2003",
        month = "Jul",
       volume = {405},
        pages = {5-14},
          doi = {10.1051/0004-6361:20030557},
archivePrefix = {arXiv},
       eprint = {astro-ph/0304054},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...405....5B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Marzke97,
       author = {{Marzke}, Ronald O. and {da Costa}, L. Nicolaci},
        title = "{The Galaxy Luminosity Function at z\&lt;/=0.05: Dependence on Color}",
      journal = {\aj},
     keywords = {GALAXIES: LUMINOSITY FUNCTION, GALAXIES: EVOLUTION},
         year = "1997",
        month = "Jan",
       volume = {113},
        pages = {185},
          doi = {10.1086/118243},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997AJ....113..185M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Stanway18,
       author = {{Stanway}, E.~R. and {Eldridge}, J.~J.},
        title = "{Re-evaluating old stellar populations}",
      journal = {\mnras},
     keywords = {methods: numerical, binaries: general, galaxies: stellar content, globular clusters: general, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = "2018",
        month = "Sep",
       volume = {479},
       number = {1},
        pages = {75-93},
          doi = {10.1093/mnras/sty1353},
archivePrefix = {arXiv},
       eprint = {1805.08784},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.479...75S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Ferland17,
       author = {{Ferland}, G.~J. and {Chatzikos}, M. and {Guzm{\'a}n}, F. and
         {Lykins}, M.~L. and {van Hoof}, P.~A.~M. and {Williams}, R.~J.~R. and
         {Abel}, N.~P. and {Badnell}, N.~R. and {Keenan}, F.~P. and
         {Porter}, R.~L. and {Stancil}, P.~C.},
        title = "{The 2017 Release Cloudy}",
      journal = {\rmxaa},
     keywords = {atomic processes, galaxies: active, methods: numerical, molecular processes, radiation mechanisms: general, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Oct",
       volume = {53},
        pages = {385-438},
archivePrefix = {arXiv},
       eprint = {1705.10877},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017RMxAA..53..385F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Dekel06,
       author = {{Dekel}, Avishai and {Birnboim}, Yuval},
        title = "{Galaxy bimodality due to cold flows and shock heating}",
      journal = {\mnras},
     keywords = {shock waves, cooling flows, galaxies: evolution, galaxies: formation, galaxies: haloes, dark matter, Astrophysics},
         year = "2006",
        month = "May",
       volume = {368},
       number = {1},
        pages = {2-20},
          doi = {10.1111/j.1365-2966.2006.10145.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0412300},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MNRAS.368....2D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Moran02,
       author = {{Moran}, Edward C. and {Filippenko}, Alexei V. and {Chornock}, Ryan},
        title = "{``Hidden'' Seyfert 2 Galaxies and the X-Ray Background}",
      journal = {\apj},
     keywords = {Galaxies: Seyfert, X-Rays: Diffuse Background, X-Rays: Galaxies, Astrophysics},
         year = "2002",
        month = "Nov",
       volume = {579},
       number = {2},
        pages = {L71-L74},
          doi = {10.1086/345314},
archivePrefix = {arXiv},
       eprint = {astro-ph/0210047},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...579L..71M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Groves04,
       author = {{Groves}, Brent A. and {Dopita}, Michael A. and {Sutherland}, Ralph S.},
        title = "{Dusty, Radiation Pressure-Dominated Photoionization. II. Multiwavelength Emission Line Diagnostics for Narrow-Line Regions}",
      journal = {\apjs},
     keywords = {Galaxies: Active, Galaxies: Seyfert, ISM: General, Line: Formation, Astrophysics},
         year = "2004",
        month = "Jul",
       volume = {153},
       number = {1},
        pages = {75-91},
          doi = {10.1086/421114},
archivePrefix = {arXiv},
       eprint = {astro-ph/0404176},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJS..153...75G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jenkins14,
       author = {{Jenkins}, Edward B.},
        title = "{Depletions of Elements from the Gas Phase: A Guide on Dust Compositions}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Galaxy Astrophysics},
         year = "2014",
        month = "Feb",
          eid = {arXiv:1402.4765},
        pages = {arXiv:1402.4765},
archivePrefix = {arXiv},
       eprint = {1402.4765},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014arXiv1402.4765J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Nicholls17,
       author = {{Nicholls}, David C. and {Sutherland}, Ralph S. and
         {Dopita}, Michael A. and {Kewley}, Lisa J. and {Groves}, Brent A.},
        title = "{Abundance scaling in stars, nebulae and galaxies}",
      journal = {\mnras},
     keywords = {Sun: abundances, Stars: abundances, ISM: abundances, Galaxies: abundances, stars: abundances, galaxies: abundances, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Apr",
       volume = {466},
       number = {4},
        pages = {4403-4422},
          doi = {10.1093/mnras/stw3235},
archivePrefix = {arXiv},
       eprint = {1612.03546},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.466.4403N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Ludwig12,
       author = {{Ludwig}, Randi R. and {Greene}, Jenny E. and {Barth}, Aaron J. and
         {Ho}, Luis C.},
        title = "{Physical Properties of the Narrow-line Region of Low-mass Active Galaxies}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: nuclei, quasars: emission lines, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "Sep",
       volume = {756},
       number = {1},
          eid = {51},
        pages = {51},
          doi = {10.1088/0004-637X/756/1/51},
archivePrefix = {arXiv},
       eprint = {1208.1303},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...756...51L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Groves06,
       author = {{Groves}, Brent A. and {Heckman}, Timothy M. and {Kauffmann}, Guinevere},
        title = "{Emission-line diagnostics of low-metallicity active galactic nuclei}",
      journal = {\mnras},
     keywords = {galaxies: abundances: galaxies: active: galaxies: Seyfert, galaxies: abundances, galaxies: active, galaxies: Seyfert, Astrophysics},
         year = "2006",
        month = "Oct",
       volume = {371},
       number = {4},
        pages = {1559-1569},
          doi = {10.1111/j.1365-2966.2006.10812.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0607311},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MNRAS.371.1559G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Moustakas06,
       author = {{Moustakas}, John and {Kennicutt}, Robert C., Jr. and
         {Tremonti}, Christy A.},
        title = "{Optical Star Formation Rate Indicators}",
      journal = {\apj},
     keywords = {Galaxies: Abundances, Galaxies: Evolution, Galaxies: Formation, Galaxies: ISM, Astrophysics},
         year = "2006",
        month = "May",
       volume = {642},
       number = {2},
        pages = {775-796},
          doi = {10.1086/500964},
archivePrefix = {arXiv},
       eprint = {astro-ph/0511730},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...642..775M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kewley08,
       author = {{Kewley}, Lisa J. and {Ellison}, Sara L.},
        title = "{Metallicity Calibrations and the Mass-Metallicity Relation for Star-forming Galaxies}",
      journal = {\apj},
     keywords = {galaxies: abundances, galaxies: fundamental parameters, galaxies: spiral, galaxies: starburst, techniques: spectroscopic, Astrophysics},
         year = "2008",
        month = "Jul",
       volume = {681},
       number = {2},
        pages = {1183-1204},
          doi = {10.1086/587500},
archivePrefix = {arXiv},
       eprint = {0801.1849},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...681.1183K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Pettini04,
       author = {{Pettini}, Max and {Pagel}, Bernard E.~J.},
        title = "{[OIII]/[NII] as an abundance indicator at high redshift}",
      journal = {\mnras},
     keywords = {ISM: abundances, HII regions, galaxies: abundances, Astrophysics},
         year = "2004",
        month = "Mar",
       volume = {348},
       number = {3},
        pages = {L59-L63},
          doi = {10.1111/j.1365-2966.2004.07591.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0401128},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004MNRAS.348L..59P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kannappan13,
       author = {{Kannappan}, Sheila J. and {Stark}, David V. and {Eckert}, Kathleen D. and
         {Moffett}, Amanda J. and {Wei}, Lisa H. and {Pisano}, D.~J. and
         {Baker}, Andrew J. and {Vogel}, Stuart N. and {Fabricant}, Daniel G. and
         {Laine}, Seppo and {Norris}, Mark A. and {Jogee}, Shardha and
         {Lepore}, Natasha and {Hough}, Loren E. and {Weinberg-Wolf}, Jennifer},
        title = "{Connecting Transitions in Galaxy Properties to Refueling}",
      journal = {\apj},
     keywords = {galaxies: evolution, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2013",
        month = "Nov",
       volume = {777},
       number = {1},
          eid = {42},
        pages = {42},
          doi = {10.1088/0004-637X/777/1/42},
archivePrefix = {arXiv},
       eprint = {1308.3292},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...777...42K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System},
      shorthand = {K13}
}


@ARTICLE{Odonnell94,
       author = {{O'Donnell}, James E.},
        title = "{R v-dependent Optical and Near-Ultraviolet Extinction}",
      journal = {\apj},
     keywords = {Interstellar Extinction, Light (Visible Radiation), Near Infrared Radiation, Ultraviolet Radiation, Astronomical Photometry, Iue, Astrophysics, ISM: DUST, EXTINCTION},
         year = "1994",
        month = "Feb",
       volume = {422},
        pages = {158},
          doi = {10.1086/173713},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1994ApJ...422..158O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Haynes11,
       author = {{Haynes}, Martha P. and {Giovanelli}, Riccardo and {Martin}, Ann M. and
         {Hess}, Kelley M. and {Saintonge}, Am{\'e}lie and
         {Adams}, Elizabeth A.~K. and {Hallenbeck}, Gregory and
         {Hoffman}, G. Lyle and {Huang}, Shan and {Kent}, Brian R. and
         {Koopmann}, Rebecca A. and {Papastergis}, Emmanouil and
         {Stierwalt}, Sabrina and {Balonek}, Thomas J. and {Craig}, David W. and
         {Higdon}, Sarah J.~U. and {Kornreich}, David A. and
         {Miller}, Jeffrey R. and {O'Donoghue}, Aileen A. and
         {Olowin}, Ronald P. and {Rosenberg}, Jessica L. and
         {Spekkens}, Kristine and {Troischt}, Parker and {Wilcots}, Eric M.},
        title = "{The Arecibo Legacy Fast ALFA Survey: The {\ensuremath{\alpha}}.40 H I Source Catalog, Its Characteristics and Their Impact on the Derivation of the H I Mass Function}",
      journal = {\aj},
     keywords = {catalogs, galaxies: distances and redshifts, galaxies: luminosity function, mass function, galaxies: spiral, radio lines: galaxies, surveys, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2011",
        month = "Nov",
       volume = {142},
       number = {5},
          eid = {170},
        pages = {170},
          doi = {10.1088/0004-6256/142/5/170},
archivePrefix = {arXiv},
       eprint = {1109.0027},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011AJ....142..170H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Berlind06,
       author = {{Berlind}, Andreas A. and {Frieman}, Joshua and {Weinberg}, David H. and
         {Blanton}, Michael R. and {Warren}, Michael S. and {Abazajian}, Kevork and
         {Scranton}, Ryan and {Hogg}, David W. and {Scoccimarro}, Roman and
         {Bahcall}, Neta A. and {Brinkmann}, J. and {Gott}, J. Richard, III and
         {Kleinman}, S.~J. and {Krzesinski}, J. and {Lee}, Brian C. and
         {Miller}, Christopher J. and {Nitta}, Atsuko and
         {Schneider}, Donald P. and {Tucker}, Douglas L. and {Zehavi}, Idit and
         {SDSS Collaboration}},
        title = "{Percolation Galaxy Groups and Clusters in the SDSS Redshift Survey: Identification, Catalogs, and the Multiplicity Function}",
      journal = {\apjs},
     keywords = {Galaxies: Clusters: General, Cosmology: Large-Scale Structure of Universe, Astrophysics},
         year = "2006",
        month = "Nov",
       volume = {167},
       number = {1},
        pages = {1-25},
          doi = {10.1086/508170},
archivePrefix = {arXiv},
       eprint = {astro-ph/0601346},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJS..167....1B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Blanton07,
       author = {{Blanton}, Michael R. and {Berlind}, Andreas A.},
        title = "{What Aspects of Galaxy Environment Matter?}",
      journal = {\apj},
     keywords = {Galaxies: Clusters: General, Galaxies: Fundamental Parameters, Galaxies: Statistics, Astrophysics},
         year = "2007",
        month = "Aug",
       volume = {664},
       number = {2},
        pages = {791-803},
          doi = {10.1086/512478},
archivePrefix = {arXiv},
       eprint = {astro-ph/0608353},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...664..791B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Kannappan04,
       author = {{Kannappan}, Sheila J.},
        title = "{Linking Gas Fractions to Bimodalities in Galaxy Properties}",
      journal = {\apj},
     keywords = {Galaxies: Evolution, Astrophysics},
         year = "2004",
        month = "Aug",
       volume = {611},
       number = {2},
        pages = {L89-L92},
          doi = {10.1086/423785},
archivePrefix = {arXiv},
       eprint = {astro-ph/0405136},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...611L..89K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Wilkins12,
       author = {{Wilkins}, Stephen M. and {Gonzalez-Perez}, Violeta and
         {Lacey}, Cedric G. and {Baugh}, Carlton M.},
        title = "{The accuracy of the UV continuum as an indicator of the star formation rate in galaxies}",
      journal = {\mnras},
     keywords = {galaxies: evolution, galaxies: formation, ultraviolet: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2012",
        month = "Dec",
       volume = {427},
       number = {2},
        pages = {1490-1496},
          doi = {10.1111/j.1365-2966.2012.22092.x},
archivePrefix = {arXiv},
       eprint = {1209.3473},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.427.1490W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Stark16,
       author = {{Stark}, David V. and {Kannappan}, Sheila J. and {Eckert}, Kathleen D. and
         {Florez}, Jonathan and {Hall}, Kirsten R. and {Watson}, Linda C. and
         {Hoversten}, Erik A. and {Burchett}, Joseph N. and {Guynn}, David T. and
         {Baker}, Ashley D. and {Moffett}, Amanda J. and {Berlind}, Andreas A. and
         {Norris}, Mark A. and {Haynes}, Martha P. and {Giovanelli}, Riccardo and
         {Leroy}, Adam K. and {Pisano}, D.~J. and {Wei}, Lisa H. and
         {Gonzalez}, Roberto E. and {Calderon}, Victor F.},
        title = "{The RESOLVE Survey Atomic Gas Census and Environmental Influences on Galaxy Gas Reservoirs}",
      journal = {\apj},
     keywords = {galaxies: evolution, galaxies: ISM, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Dec",
       volume = {832},
       number = {2},
          eid = {126},
        pages = {126},
          doi = {10.3847/0004-637X/832/2/126},
archivePrefix = {arXiv},
       eprint = {1610.06932},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...832..126S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Eckert16,
       author = {{Eckert}, Kathleen D. and {Kannappan}, Sheila J. and {Stark}, David V. and
         {Moffett}, Amanda J. and {Berlind}, Andreas A. and {Norris}, Mark A.},
        title = "{RESOLVE and ECO: The Halo Mass-dependent Shape of Galaxy Stellar and Baryonic Mass Functions}",
      journal = {\apj},
     keywords = {galaxies: luminosity function, mass function, methods: statistical, surveys, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Jun",
       volume = {824},
       number = {2},
          eid = {124},
        pages = {124},
          doi = {10.3847/0004-637X/824/2/124},
archivePrefix = {arXiv},
       eprint = {1604.03957},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...824..124E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Acker89,
   author = {{Acker}, A. and {K{\"o}ppen}, J. and {Samland}, M. and {Stenholm}, B.
	},
    title = "{On the theoretical ratio of some nebular lines.}",
  journal = {The Messenger},
 keywords = {Planetary Nebulae: Spectra},
     year = 1989,
    month = dec,
   volume = 58,
    pages = {44-46},
   adsurl = {http://adsabs.harvard.edu/abs/1989Msngr..58...44A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kauffmann03,
       author = {{Kauffmann}, Guinevere and {Heckman}, Timothy M. and
         {Tremonti}, Christy and {Brinchmann}, Jarle and
         {Charlot}, St{\'e}phane and {White}, Simon D.~M. and
         {Ridgway}, Susan E. and {Brinkmann}, Jon and {Fukugita}, Masataka and
         {Hall}, Patrick B. and {Ivezi{\'c}}, {\v{Z}}eljko and
         {Richards}, Gordon T. and {Schneider}, Donald P.},
        title = "{The host galaxies of active galactic nuclei}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: Seyfert, galaxies: starburst, galaxies: stellar content, galaxies: structure, Astrophysics},
         year = "2003",
        month = "Dec",
       volume = {346},
        pages = {1055-1077},
          doi = {10.1111/j.1365-2966.2003.07154.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0304239},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2003MNRAS.346.1055K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Kannappan08,
       author = {{Kannappan}, Sheila J. and {Wei}, Lisa H.},
        title = "{Galaxy Gas Fractions, Characteristic Mass Scales, and the RESOLVE Survey}",
     keywords = {97.10.Bt, 98.38.-j, 98.62.Mw, 98.65.Cw, 95.55.-n, 95.75.Fg, Star formation, Interstellar medium  and nebulae in Milky Way, Infall accretion and accretion disks, Galaxy clusters, Astronomical and space-research instrumentation, Spectroscopy and spectrophotometry},
    booktitle = {The Evolution of Galaxies Through the Neutral Hydrogen Window},
         year = "2008",
       editor = {{Minchin}, Robert and {Momjian}, Emmanuel},
       series = {American Institute of Physics Conference Series},
       volume = {1035},
        month = "Aug",
        pages = {163-168},
          doi = {10.1063/1.2973572},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2008AIPC.1035..163K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Moffett15,
       author = {{Moffett}, Amanda J. and {Kannappan}, Sheila J. and
         {Berlind}, Andreas A. and {Eckert}, Kathleen D. and {Stark}, David V. and
         {Hendel}, David and {Norris}, Mark A. and {Grogin}, Norman A.},
        title = "{ECO and RESOLVE: Galaxy Disk Growth in Environmental Context}",
      journal = {\apj},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, ultraviolet: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = "2015",
        month = "Oct",
       volume = {812},
          eid = {89},
        pages = {89},
          doi = {10.1088/0004-637X/812/2/89},
archivePrefix = {arXiv},
       eprint = {1508.00948},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2015ApJ...812...89M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Blanc15,
       author = {{Blanc}, Guillermo A. and {Kewley}, Lisa and
         {Vogt}, Fr{\'e}d{\'e}ric P.~A. and {Dopita}, Michael A.},
        title = "{IZI: Inferring the Gas Phase Metallicity (Z) and Ionization Parameter (q) of Ionized Nebulae Using Bayesian Statistics}",
      journal = {\apj},
     keywords = {astrochemistry, galaxies: abundances, galaxies: ISM, H II regions, ISM: abundances, Astrophysics - Astrophysics of Galaxies},
         year = "2015",
        month = "Jan",
       volume = {798},
          eid = {99},
        pages = {99},
          doi = {10.1088/0004-637X/798/2/99},
archivePrefix = {arXiv},
       eprint = {1410.8146},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2015ApJ...798...99B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Thomas18,
       author = {{Thomas}, Adam D. and {Dopita}, Michael A. and {Kewley}, Lisa J. and
         {Groves}, Brent A. and {Sutherland}, Ralph S. and {Hopkins}, Andrew M. and
         {Blanc}, Guillermo A.},
        title = "{Interrogating Seyferts with NebulaBayes: Spatially Probing the Narrow-line Region Radiation Fields and Chemical Abundances}",
      journal = {\apj},
     keywords = {galaxies: abundances, galaxies: active, galaxies: ISM, galaxies: Seyfert, ISM: abundances, quasars: emission lines, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Apr",
       volume = {856},
          eid = {89},
        pages = {89},
          doi = {10.3847/1538-4357/aab3db},
archivePrefix = {arXiv},
       eprint = {1803.00740},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2018ApJ...856...89T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gordon03,
       author = {{Gordon}, Karl D. and {Clayton}, Geoffrey C. and {Misselt}, K.~A. and {Land
        olt}, Arlo U. and {Wolff}, Michael J.},
        title = "{A Quantitative Comparison of the Small Magellanic Cloud, Large Magellanic Cloud, and Milky Way Ultraviolet to Near-Infrared Extinction Curves}",
      journal = {\apj},
     keywords = {ISM: Dust, Extinction, Galaxies: ISM, Galaxies: Magellanic Clouds, Ultraviolet: ISM, Astrophysics},
         year = "2003",
        month = "Sep",
       volume = {594},
        pages = {279-293},
          doi = {10.1086/376774},
archivePrefix = {arXiv},
       eprint = {astro-ph/0305257},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2003ApJ...594..279G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{Osterbrock06,
       author = {{Osterbrock}, Donald E. and {Ferland}, Gary J.},
        title = "{Astrophysics of gaseous nebulae and active galactic nuclei}",
    booktitle = {Astrophysics of gaseous nebulae and active galactic nuclei, 2nd. ed. by D.E. Osterbrock and G.J. Ferland. Sausalito, CA: University Science Books, 2006},
         year = "2006",
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2006agna.book.....O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Dominguez13,
       author = {{Dom{\'\i}nguez}, A. and {Siana}, B. and {Henry}, A.~L. and
         {Scarlata}, C. and {Bedregal}, A.~G. and {Malkan}, M. and {Atek}, H. and
         {Ross}, N.~R. and {Colbert}, J.~W. and {Teplitz}, H.~I. and
         {Rafelski}, M. and {McCarthy}, P. and {Bunker}, A. and {Hathi}, N.~P. and
         {Dressler}, A. and {Martin}, C.~L. and {Masters}, D.},
        title = "{Dust Extinction from Balmer Decrements of Star-forming Galaxies at 0.75 \&lt;= z \&lt;= 1.5 with Hubble Space Telescope/Wide-Field-Camera 3 Spectroscopy from the WFC3 Infrared Spectroscopic Parallel Survey}",
      journal = {\apj},
     keywords = {dust, extinction, galaxies: evolution, galaxies: high-redshift, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2013",
        month = "Feb",
       volume = {763},
          eid = {145},
        pages = {145},
          doi = {10.1088/0004-637X/763/2/145},
archivePrefix = {arXiv},
       eprint = {1206.1867},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2013ApJ...763..145D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Alam15,
       author = {{Alam}, Shadab and {Albareti}, Franco D. and {Allende Prieto}, Carlos and
         {Anders}, F. and {Anderson}, Scott F. and {Anderton}, Timothy and
         {Andrews}, Brett H. and {Armengaud}, Eric and {Aubourg}, {\'E}ric and
         {Bailey}, Stephen and {Basu}, Sarbani and {Bautista}, Julian E. and
         {Beaton}, Rachael L. and {Beers}, Timothy C. and {Bender}, Chad F. and
         {Berlind}, Andreas A. and {Beutler}, Florian and {Bhardwaj}, Vaishali and
         {Bird}, Jonathan C. and {Bizyaev}, Dmitry and {Blake}, Cullen H. and
         {Blanton}, Michael R. and {Blomqvist}, Michael and
         {Bochanski}, John J. and {Bolton}, Adam S. and {Bovy}, Jo and
         {Shelden Bradley}, A. and {Brandt}, W.~N. and {Brauer}, D.~E. and
         {Brinkmann}, J. and {Brown}, Peter J. and {Brownstein}, Joel R. and
         {Burden}, Angela and {Burtin}, Etienne and {Busca}, Nicol{\'a}s G. and
         {Cai}, Zheng and {Capozzi}, Diego and {Carnero Rosell}, Aurelio and
         {Carr}, Michael A. and {Carrera}, Ricardo and {Chambers}, K.~C. and
         {Chaplin}, William James and {Chen}, Yen-Chi and {Chiappini}, Cristina and
         {Chojnowski}, S. Drew and {Chuang}, Chia-Hsun and {Clerc}, Nicolas and
         {Comparat}, Johan and {Covey}, Kevin and {Croft}, Rupert A.~C. and
         {Cuesta}, Antonio J. and {Cunha}, Katia and {da Costa}, Luiz N. and
         {Da Rio}, Nicola and {Davenport}, James R.~A. and {Dawson}, Kyle S. and
         {De Lee}, Nathan and {Delubac}, Timoth{\'e}e and {Deshpande}, Rohit and
         {Dhital}, Saurav and {Dutra-Ferreira}, Let{\'\i}cia and {Dwelly}, Tom and
         {Ealet}, Anne and {Ebelke}, Garrett L. and {Edmondson}, Edward M. and
         {Eisenstein}, Daniel J. and {Ellsworth}, Tristan and
         {Elsworth}, Yvonne and {Epstein}, Courtney R. and {Eracleous}, Michael and
         {Escoffier}, Stephanie and {Esposito}, Massimiliano and
         {Evans}, Michael L. and {Fan}, Xiaohui and {Fern{\'a}ndez-Alvar}, Emma and
         {Feuillet}, Diane and {Filiz Ak}, Nurten and {Finley}, Hayley and
         {Finoguenov}, Alexis and {Flaherty}, Kevin and {Fleming}, Scott W. and
         {Font-Ribera}, Andreu and {Foster}, Jonathan and
         {Frinchaboy}, Peter M. and {Galbraith-Frew}, J.~G. and
         {Garc{\'\i}a}, Rafael A. and {Garc{\'\i}a-Hern{\'a}ndez}, D.~A. and
         {Garc{\'\i}a P{\'e}rez}, Ana E. and {Gaulme}, Patrick and {Ge}, Jian and
         {G{\'e}nova-Santos}, R. and {Georgakakis}, A. and {Ghezzi}, Luan and
         {Gillespie}, Bruce A. and {Girardi}, L{\'e}o and {Goddard}, Daniel and
         {Gontcho}, Satya Gontcho A. and {Gonz{\'a}lez Hern{\'a}ndez}, Jonay I. and
         {Grebel}, Eva K. and {Green}, Paul J. and {Grieb}, Jan Niklas and
         {Grieves}, Nolan and {Gunn}, James E. and {Guo}, Hong and
         {Harding}, Paul and {Hasselquist}, Sten and {Hawley}, Suzanne L. and
         {Hayden}, Michael and {Hearty}, Fred R. and {Hekker}, Saskia and
         {Ho}, Shirley and {Hogg}, David W. and {Holley-Bockelmann}, Kelly and
         {Holtzman}, Jon A. and {Honscheid}, Klaus and {Huber}, Daniel and
         {Huehnerhoff}, Joseph and {Ivans}, Inese I. and {Jiang}, Linhua and
         {Johnson}, Jennifer A. and {Kinemuchi}, Karen and {Kirkby}, David and
         {Kitaura}, Francisco and {Klaene}, Mark A. and {Knapp}, Gillian R. and
         {Kneib}, Jean-Paul and {Koenig}, Xavier P. and {Lam}, Charles R. and
         {Lan}, Ting-Wen and {Lang}, Dustin and {Laurent}, Pierre and
         {Le Goff}, Jean-Marc and {Leauthaud}, Alexie and {Lee}, Khee-Gan and
         {Lee}, Young Sun and {Licquia}, Timothy C. and {Liu}, Jian and
         {Long}, Daniel C. and {L{\'o}pez-Corredoira}, Mart{\'\i}n and
         {Lorenzo-Oliveira}, Diego and {Lucatello}, Sara and {Lundgren}, Britt and
         {Lupton}, Robert H. and {Mack}, Claude E., III and
         {Mahadevan}, Suvrath and {Maia}, Marcio A.~G. and
         {Majewski}, Steven R. and {Malanushenko}, Elena and
         {Malanushenko}, Viktor and {Manchado}, A. and {Manera}, Marc and
         {Mao}, Qingqing and {Maraston}, Claudia and {Marchwinski}, Robert C. and
         {Margala}, Daniel and {Martell}, Sarah L. and {Martig}, Marie and
         {Masters}, Karen L. and {Mathur}, Savita and {McBride}, Cameron K. and
         {McGehee}, Peregrine M. and {McGreer}, Ian D. and
         {McMahon}, Richard G. and {M{\'e}nard}, Brice and
         {Menzel}, Marie-Luise and {Merloni}, Andrea and
         {M{\'e}sz{\'a}ros}, Szabolcs and {Miller}, Adam A. and
         {Miralda-Escud{\'e}}, Jordi and {Miyatake}, Hironao and
         {Montero-Dorta}, Antonio D. and {More}, Surhud and {Morganson}, Eric and
         {Morice-Atkinson}, Xan and {Morrison}, Heather L. and
         {Mosser}, Ben{\^o}it and {Muna}, Demitri and {Myers}, Adam D. and {Nand
        ra}, Kirpal and {Newman}, Jeffrey A. and {Neyrinck}, Mark and
         {Nguyen}, Duy Cuong and {Nichol}, Robert C. and {Nidever}, David L. and
         {Noterdaeme}, Pasquier and {Nuza}, Sebasti{\'a}n E. and
         {O'Connell}, Julia E. and {O'Connell}, Robert W. and {O'Connell}, Ross and
         {Ogando}, Ricardo L.~C. and {Olmstead}, Matthew D. and
         {Oravetz}, Audrey E. and {Oravetz}, Daniel J. and {Osumi}, Keisuke and
         {Owen}, Russell and {Padgett}, Deborah L. and {Padmanabhan}, Nikhil and
         {Paegert}, Martin and {Palanque-Delabrouille}, Nathalie and
         {Pan}, Kaike and {Parejko}, John K. and {P{\^a}ris}, Isabelle and
         {Park}, Changbom and {Pattarakijwanich}, Petchara and
         {Pellejero-Ibanez}, M. and {Pepper}, Joshua and {Percival}, Will J. and
         {P{\'e}rez-Fournon}, Ismael and {Ṕrez-Ra`fols}, Ignasi and
         {Petitjean}, Patrick and {Pieri}, Matthew M. and
         {Pinsonneault}, Marc H. and {Porto de Mello}, Gustavo F. and
         {Prada}, Francisco and {Prakash}, Abhishek and
         {Price-Whelan}, Adrian M. and {Protopapas}, Pavlos and
         {Raddick}, M. Jordan and {Rahman}, Mubdi and {Reid}, Beth A. and
         {Rich}, James and {Rix}, Hans-Walter and {Robin}, Annie C. and
         {Rockosi}, Constance M. and {Rodrigues}, Tha{\'\i}se S. and
         {Rodr{\'\i}guez-Torres}, Sergio and {Roe}, Natalie A. and
         {Ross}, Ashley J. and {Ross}, Nicholas P. and {Rossi}, Graziano and
         {Ruan}, John J. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and
         {Rykoff}, Eli S. and {Salazar-Albornoz}, Salvador and {Salvato}, Mara and
         {Samushia}, Lado and {S{\'a}nchez}, Ariel G. and
         {Santiago}, Bas{\'\i}lio and {Sayres}, Conor and
         {Schiavon}, Ricardo P. and {Schlegel}, David J. and
         {Schmidt}, Sarah J. and {Schneider}, Donald P. and
         {Schultheis}, Mathias and {Schwope}, Axel D. and {Sc{\'o}ccola}, C.~G. and
         {Scott}, Caroline and {Sellgren}, Kris and {Seo}, Hee-Jong and
         {Serenelli}, Aldo and {Shane}, Neville and {Shen}, Yue and
         {Shetrone}, Matthew and {Shu}, Yiping and {Silva Aguirre}, V. and
         {Sivarani}, Thirupathi and {Skrutskie}, M.~F. and {Slosar}, An{\v{z}}e and
         {Smith}, Verne V. and {Sobreira}, Fl{\'a}via and {Souto}, Diogo and
         {Stassun}, Keivan G. and {Steinmetz}, Matthias and {Stello}, Dennis and
         {Strauss}, Michael A. and {Streblyanska}, Alina and {Suzuki}, Nao and
         {Swanson}, Molly E.~C. and {Tan}, Jonathan C. and {Tayar}, Jamie and
         {Terrien}, Ryan C. and {Thakar}, Aniruddha R. and {Thomas}, Daniel and
         {Thomas}, Neil and {Thompson}, Benjamin A. and {Tinker}, Jeremy L. and
         {Tojeiro}, Rita and {Troup}, Nicholas W. and
         {Vargas-Maga{\~n}a}, Mariana and {Vazquez}, Jose A. and {Verde}, Licia and
         {Viel}, Matteo and {Vogt}, Nicole P. and {Wake}, David A. and
         {Wang}, Ji and {Weaver}, Benjamin A. and {Weinberg}, David H. and
         {Weiner}, Benjamin J. and {White}, Martin and {Wilson}, John C. and
         {Wisniewski}, John P. and {Wood-Vasey}, W.~M. and {Ye`che}, Christophe and
         {York}, Donald G. and {Zakamska}, Nadia L. and {Zamora}, O. and
         {Zasowski}, Gail and {Zehavi}, Idit and {Zhao}, Gong-Bo and
         {Zheng}, Zheng and {Zhou}, Xu and {Zhou}, Zhimin and {Zou}, Hu and
         {Zhu}, Guangtun},
        title = "{The Eleventh and Twelfth Data Releases of the Sloan Digital Sky Survey: Final Data from SDSS-III}",
      journal = {The Astrophysical Journal Supplement Series},
     keywords = {atlases, catalogs, surveys, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = "2015",
        month = "Jul",
       volume = {219},
          eid = {12},
        pages = {12},
          doi = {10.1088/0067-0049/219/1/12},
archivePrefix = {arXiv},
       eprint = {1501.00963},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2015ApJS..219...12A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Tremonti04,
       author = {{Tremonti}, Christy A. and {Heckman}, Timothy M. and
         {Kauffmann}, Guinevere and {Brinchmann}, Jarle and
         {Charlot}, St{\'e}phane and {White}, Simon D.~M. and {Seibert}, Mark and
         {Peng}, Eric W. and {Schlegel}, David J. and {Uomoto}, Alan and
         {Fukugita}, Masataka and {Brinkmann}, Jon},
        title = "{The Origin of the Mass-Metallicity Relation: Insights from 53,000 Star-forming Galaxies in the Sloan Digital Sky Survey}",
      journal = {\apj},
     keywords = {Galaxies: Abundances, Galaxies: Evolution, Galaxies: Fundamental Parameters, Galaxies: Statistics, Astrophysics},
         year = "2004",
        month = "Oct",
       volume = {613},
        pages = {898-913},
          doi = {10.1086/423264},
archivePrefix = {arXiv},
       eprint = {astro-ph/0405537},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2004ApJ...613..898T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Hood18,
       author = {{Hood}, Callie E. and {Kannappan}, Sheila J. and {Stark}, David V. and
         {Dell'Antonio}, Ian P. and {Moffett}, Amanda J. and
         {Eckert}, Kathleen D. and {Norris}, Mark A. and {Hendel}, David},
        title = "{The Origin of Faint Tidal Features around Galaxies in the RESOLVE Survey}",
      journal = {\apj},
     keywords = {galaxies: evolution, galaxies: interactions, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Apr",
       volume = {857},
          eid = {144},
        pages = {144},
          doi = {10.3847/1538-4357/aab719},
archivePrefix = {arXiv},
       eprint = {1803.05447},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2018ApJ...857..144H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Eckert15,
       author = {{Eckert}, Kathleen D. and {Kannappan}, Sheila J. and {Stark}, David V. and
         {Moffett}, Amanda J. and {Norris}, Mark A. and {Snyder}, Elaine M. and
         {Hoversten}, Erik A.},
        title = "{RESOLVE Survey Photometry and Volume-limited Calibration of the Photometric Gas Fractions Technique}",
      journal = {\apj},
     keywords = {galaxies: ISM, galaxies: photometry, surveys, Astrophysics - Astrophysics of Galaxies},
         year = "2015",
        month = "Sep",
       volume = {810},
          eid = {166},
        pages = {166},
          doi = {10.1088/0004-637X/810/2/166},
archivePrefix = {arXiv},
       eprint = {1507.08669},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2015ApJ...810..166E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bar17,
       author = {{B{\"a}r}, Rudolf E. and {Weigel}, Anna K. and {Sartori}, Lia F. and
         {Oh}, Kyuseok and {Koss}, Michael and {Schawinski}, Kevin},
        title = "{Active galactic nuclei from He II: a more complete census of AGN in SDSS galaxies yields a new population of low-luminosity AGN in highly star-forming galaxies}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: evolution, galaxies: nuclei, galaxies: Seyfert, galaxies: star formation, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2017",
        month = "Apr",
       volume = {466},
        pages = {2879-2887},
          doi = {10.1093/mnras/stw3283},
archivePrefix = {arXiv},
       eprint = {1612.04815},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2017MNRAS.466.2879B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reines13,
       author = {{Reines}, Amy E. and {Greene}, Jenny E. and {Geha}, Marla},
        title = "{Dwarf Galaxies with Optical Signatures of Active Massive Black Holes}",
      journal = {\apj},
     keywords = {galaxies: active, galaxies: dwarf, galaxies: nuclei, galaxies: Seyfert, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2013",
        month = "Oct",
       volume = {775},
          eid = {116},
        pages = {116},
          doi = {10.1088/0004-637X/775/2/116},
archivePrefix = {arXiv},
       eprint = {1308.0328},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2013ApJ...775..116R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Veilleux87,
       author = {{Veilleux}, Sylvain and {Osterbrock}, Donald E.},
        title = "{Spectral Classification of Emission-Line Galaxies}",
      journal = {The Astrophysical Journal Supplement Series},
     keywords = {Emission Spectra, Seyfert Galaxies, Spectral Line Width, Spectrum Analysis, Active Galaxies, Astronomical Models, Astronomical Spectroscopy, H Ii Regions, Hot Stars, Interstellar Extinction, Photoionization, Star Formation, Astrophysics, GALAXIES: SEYFERT},
         year = "1987",
        month = "Feb",
       volume = {63},
        pages = {295},
          doi = {10.1086/191166},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/1987ApJS...63..295V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kewley2006,
   author = {{Kewley}, L.~J. and {Groves}, B. and {Kauffmann}, G. and {Heckman}, T.
	},
    title = "{The host galaxies and classification of active galactic nuclei}",
  journal = {\mnras},
   eprint = {astro-ph/0605681},
 keywords = {galaxies: active, galaxies: Seyfert, galaxies: starburst},
     year = 2006,
    month = nov,
   volume = 372,
    pages = {961-976},
      doi = {10.1111/j.1365-2966.2006.10859.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.372..961K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Dessauges-Zavadsky00,
       author = {{Dessauges-Zavadsky}, M. and {Pindao}, M. and {Maeder}, A. and
         {Kunth}, D.},
        title = "{Spectral classification of emission-line galaxies}",
      journal = {\aap},
     keywords = {CATALOGS, ISM: H II REGIONS, GALAXIES: ACTIVE, GALAXIES: SEYFERT, GALAXIES: STARBURST},
         year = 2000,
        month = mar,
       volume = {355},
        pages = {89-98},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&A...355...89D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@book{Draine, place={Princeton, NJ}, title={Physics of the interstellar and intergalactic medium}, publisher={Princeton University Press}, author={Draine, Bruce T.}, year={2011}}

@ARTICLE{Kewley01,
       author = {{Kewley}, L.~J. and {Dopita}, M.~A. and {Sutherland}, R.~S. and
         {Heisler}, C.~A. and {Trevena}, J.},
        title = "{Theoretical Modeling of Starburst Galaxies}",
      journal = {\apj},
     keywords = {Galaxies: Starburst, Radiation Mechanisms: Thermal, Astrophysics},
         year = "2001",
        month = "Jul",
       volume = {556},
        pages = {121-140},
          doi = {10.1086/321545},
archivePrefix = {arXiv},
       eprint = {astro-ph/0106324},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2001ApJ...556..121K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Agostino18,
       author = {{Agostino}, Christopher J. and {Salim}, Samir},
        title = "{Crossing the Line: Active Galactic Nuclei in the Star-forming region of the BPT Diagram}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Nov",
          eid = {arXiv:1811.11755},
        pages = {arXiv:1811.11755},
archivePrefix = {arXiv},
       eprint = {1811.11755},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2018arXiv181111755A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Shirazi12,
       author = {{Shirazi}, Maryam and {Brinchmann}, Jarle},
        title = "{Strongly star forming galaxies in the local Universe with nebular He II{\ensuremath{\lambda}}4686 emission}",
      journal = {\mnras},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "Apr",
       volume = {421},
        pages = {1043-1063},
          doi = {10.1111/j.1365-2966.2012.20439.x},
archivePrefix = {arXiv},
       eprint = {1201.1290},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2012MNRAS.421.1043S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Sartori15,
       author = {{Sartori}, Lia F. and {Schawinski}, Kevin and {Treister}, Ezequiel and
         {Trakhtenbrot}, Benny and {Koss}, Michael and {Shirazi}, Maryam and
         {Oh}, Kyuseok},
        title = "{The search for active black holes in nearby low-mass galaxies using optical and mid-IR data}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: dwarf, galaxies: nuclei, galaxies: Seyfert, infrared: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = "2015",
        month = "Dec",
       volume = {454},
        pages = {3722-3742},
          doi = {10.1093/mnras/stv2238},
archivePrefix = {arXiv},
       eprint = {1509.08483},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2015MNRAS.454.3722S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Baldwin81,
       author = {{Baldwin}, J.~A. and {Phillips}, M.~M. and {Terlevich}, R.},
        title = "{Classification parameters for the emission-line spectra of extragalactic objects.}",
      journal = {Publications of the Astronomical Society of the Pacific},
     keywords = {Astronomical Spectroscopy, Emission Spectra, Line Spectra, Quasars, Seyfert Galaxies, Classifications, H Ii Regions, Photoionization, Planetary Nebulae, Shock Heating, Astrophysics},
         year = "1981",
        month = "Feb",
       volume = {93},
        pages = {5-19},
          doi = {10.1086/130766},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/1981PASP...93....5B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Tremmel17,
       author = {{Tremmel}, M. and {Karcher}, M. and {Governato}, F. and {Volonteri}, M. and
         {Quinn}, T.~R. and {Pontzen}, A. and {Anderson}, L. and {Bellovary}, J.},
        title = "{The Romulus cosmological simulations: a physical approach to the formation, dynamics and accretion models of SMBHs}",
      journal = {\mnras},
     keywords = {methods: numerical, galaxies: general, quasars: supermassive black holes, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Sep",
       volume = {470},
       number = {1},
        pages = {1121-1139},
          doi = {10.1093/mnras/stx1160},
archivePrefix = {arXiv},
       eprint = {1607.02151},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.470.1121T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dalcanton04,
       author = {{Dalcanton}, Julianne J. and {Yoachim}, Peter and
         {Bernstein}, Rebecca A.},
        title = "{The Formation of Dust Lanes: Implications for Galaxy Evolution}",
      journal = {\apj},
     keywords = {ISM: Dust, Extinction, Galaxies: Formation, Galaxies: ISM, Galaxies: Spiral, ISM: Structure, Stars: Formation, Astrophysics},
         year = "2004",
        month = "Jun",
       volume = {608},
       number = {1},
        pages = {189-207},
          doi = {10.1086/386358},
archivePrefix = {arXiv},
       eprint = {astro-ph/0402472},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...608..189D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gutkin16,
       author = {{Gutkin}, Julia and {Charlot}, St{\'e}phane and {Bruzual}, Gustavo},
        title = "{Modelling the nebular emission from primeval to present-day star-forming galaxies}",
      journal = {\mnras},
     keywords = {galaxies: abundances, galaxies: general, galaxies: high-redshift, galaxies: ISM, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Oct",
       volume = {462},
       number = {2},
        pages = {1757-1774},
          doi = {10.1093/mnras/stw1716},
archivePrefix = {arXiv},
       eprint = {1607.06086},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016MNRAS.462.1757G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{DeCia16,
       author = {{De Cia}, A. and {Ledoux}, C. and {Mattsson}, L. and {Petitjean}, P. and
         {Srianand}, R. and {Gavignaud}, I. and {Jenkins}, E.~B.},
        title = "{Dust-depletion sequences in damped Lyman-{\ensuremath{\alpha}} absorbers. A unified picture from low-metallicity systems to the Galaxy}",
      journal = {\aap},
     keywords = {ISM: abundances, dust, extinction, quasars: absorption lines, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = "2016",
        month = "Dec",
       volume = {596},
          eid = {A97},
        pages = {A97},
          doi = {10.1051/0004-6361/201527895},
archivePrefix = {arXiv},
       eprint = {1608.08621},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...596A..97D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Pilyugin14,
       author = {{Pilyugin}, L.~S. and {Grebel}, E.~K. and {Zinchenko}, I.~A. and
         {Kniazev}, A.~Y.},
        title = "{The Abundance Properties of Nearby Late-Type Galaxies. II. the Relation between Abundance Distributions and Surface Brightness Profiles}",
      journal = {\aj},
     keywords = {galaxies: abundances, galaxies: photometry, galaxies: spiral, Astrophysics - Astrophysics of Galaxies},
         year = "2014",
        month = "Dec",
       volume = {148},
       number = {6},
          eid = {134},
        pages = {134},
          doi = {10.1088/0004-6256/148/6/134},
archivePrefix = {arXiv},
       eprint = {1408.6413},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014AJ....148..134P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Cresci18,
       author = {{Cresci}, Giovanni and {Mannucci}, Filippo and {Curti}, Mirko},
        title = "{The ``Fundamental Metallicity Relation'' in CALIFA, SDSS-IV MaNGA and high-z galaxies}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Nov",
          eid = {arXiv:1811.06015},
        pages = {arXiv:1811.06015},
archivePrefix = {arXiv},
       eprint = {1811.06015},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv181106015C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Salim14,
       author = {{Salim}, Samir and {Lee}, Janice C. and {Ly}, Chun and
         {Brinchmann}, Jarle and {Dav{\'e}}, Romeel and {Dickinson}, Mark and
         {Salzer}, John J. and {Charlot}, St{\'e}phane},
        title = "{A Critical Look at the Mass-Metallicity-Star Formation Rate Relation in the Local Universe. I. An Improved Analysis Framework and Confounding Systematics}",
      journal = {\apj},
     keywords = {galaxies: abundances, galaxies: evolution, galaxies: fundamental parameters, Astrophysics - Astrophysics of Galaxies},
         year = "2014",
        month = "Dec",
       volume = {797},
       number = {2},
          eid = {126},
        pages = {126},
          doi = {10.1088/0004-637X/797/2/126},
archivePrefix = {arXiv},
       eprint = {1411.7391},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...797..126S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Yates12,
       author = {{Yates}, Robert M. and {Kauffmann}, Guinevere and {Guo}, Qi},
        title = "{The relation between metallicity, stellar mass and star formation in galaxies: an analysis of observational and model data}",
      journal = {\mnras},
     keywords = {ISM: abundances, galaxies: abundances, galaxies: evolution, galaxies: fundamental parameters, galaxies: star formation, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2012",
        month = "May",
       volume = {422},
       number = {1},
        pages = {215-231},
          doi = {10.1111/j.1365-2966.2012.20595.x},
archivePrefix = {arXiv},
       eprint = {1107.3145},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.422..215Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lara10,
       author = {{Lara-L{\'o}pez}, M.~A. and {Cepa}, J. and {Bongiovanni}, A. and
         {P{\'e}rez Garc{\'\i}a}, A.~M. and {Ederoclite}, A. and
         {Casta{\~n}eda}, H. and {Fern{\'a}ndez Lorenzo}, M. and
         {Povi{\'c}}, M. and {S{\'a}nchez-Portal}, M.},
        title = "{A fundamental plane for field star-forming galaxies}",
      journal = {\aap},
     keywords = {galaxies: fundamental parameters, galaxies: abundances, galaxies: starburst, galaxies: star formation, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2010",
        month = "Oct",
       volume = {521},
          eid = {L53},
        pages = {L53},
          doi = {10.1051/0004-6361/201014803},
archivePrefix = {arXiv},
       eprint = {1005.0509},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010A&A...521L..53L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mannucci11,
       author = {{Mannucci}, F. and {Salvaterra}, R. and {Campisi}, M.~A.},
        title = "{The metallicity of the long GRB hosts and the fundamental metallicity relation of low-mass galaxies}",
      journal = {\mnras},
     keywords = {galaxies: abundances, galaxies: star formation, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = "2011",
        month = "Jun",
       volume = {414},
       number = {2},
        pages = {1263-1268},
          doi = {10.1111/j.1365-2966.2011.18459.x},
archivePrefix = {arXiv},
       eprint = {1011.4506},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.414.1263M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Kannappan09,
       author = {{Kannappan}, Sheila J. and {Guie}, Jocelly M. and {Baker}, Andrew J.},
        title = "{E/S0 Galaxies on the Blue Color-Stellar Mass Sequence at z = 0: Fading Mergers or Future Spirals?}",
      journal = {\aj},
     keywords = {galaxies: elliptical and lenticular, cD, galaxies: evolution, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = "2009",
        month = "Aug",
       volume = {138},
       number = {2},
        pages = {579-597},
          doi = {10.1088/0004-6256/138/2/579},
archivePrefix = {arXiv},
       eprint = {0903.3695},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009AJ....138..579K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Denicolo02,
       author = {{Denicol{\'o}}, Glenda and {Terlevich}, Roberto and {Terlevich}, Elena},
        title = "{New light on the search for low-metallicity galaxies - I. The N2 calibrator}",
      journal = {\mnras},
     keywords = {GALAXIES: ABUNDANCES, GALAXIES: EVOLUTION, GALAXIES: STELLAR CONTENT, Astrophysics},
         year = "2002",
        month = "Feb",
       volume = {330},
       number = {1},
        pages = {69-74},
          doi = {10.1046/j.1365-8711.2002.05041.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0110356},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002MNRAS.330...69D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Ciardi97,
       author = {{Ciardi}, Benedetta and {Ferrara}, Andrea},
        title = "{Ly{\ensuremath{\alpha}} Clouds Associated with Population III Objects in Cold Dark Matter Models}",
      journal = {\apj},
     keywords = {COSMOLOGY: THEORY, DARK MATTER, GALAXIES: QUASARS: ABSORPTION LINES, Cosmology: Theory, Cosmology: Dark Matter, Galaxies: Quasars: Absorption Lines, Astrophysics},
         year = "1997",
        month = "Jul",
       volume = {483},
       number = {1},
        pages = {L5-L8},
          doi = {10.1086/310728},
archivePrefix = {arXiv},
       eprint = {astro-ph/9703112},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...483L...5C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{MacLow99,
       author = {{Mac Low}, Mordecai-Mark and {Ferrara}, Andrea},
        title = "{Starburst-driven Mass Loss from Dwarf Galaxies: Efficiency and Metal Ejection}",
      journal = {\apj},
     keywords = {GALAXIES: EVOLUTION, GALAXIES: STARBURST, GALAXIES: STELLAR CONTENT, HYDRODYNAMICS, STARS: SUPERNOVAE: GENERAL, Galaxies: Evolution, Galaxies: Starburst, Galaxies: Stellar Content, Hydrodynamics, Stars: Supernovae: General, Astrophysics},
         year = "1999",
        month = "Mar",
       volume = {513},
       number = {1},
        pages = {142-155},
          doi = {10.1086/306832},
archivePrefix = {arXiv},
       eprint = {astro-ph/9801237},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...513..142M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Bettoni03,
       author = {{Bettoni}, D. and {Galletta}, G. and {Garc{\'\i}a-Burillo}, S.},
        title = "{A new catalogue of ISM content of normal galaxies}",
      journal = {\aap},
     keywords = {catalogs, galaxies: ISM, galaxies: general, infrared: galaxies, radio lines: galaxies, X-rays: galaxies, submillimeter, Astrophysics},
         year = "2003",
        month = "Jul",
       volume = {405},
        pages = {5-14},
          doi = {10.1051/0004-6361:20030557},
archivePrefix = {arXiv},
       eprint = {astro-ph/0304054},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...405....5B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Marzke97,
       author = {{Marzke}, Ronald O. and {da Costa}, L. Nicolaci},
        title = "{The Galaxy Luminosity Function at z\&lt;/=0.05: Dependence on Color}",
      journal = {\aj},
     keywords = {GALAXIES: LUMINOSITY FUNCTION, GALAXIES: EVOLUTION},
         year = "1997",
        month = "Jan",
       volume = {113},
        pages = {185},
          doi = {10.1086/118243},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997AJ....113..185M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Jenkins14,
       author = {{Jenkins}, Edward B.},
        title = "{Depletions of Elements from the Gas Phase: A Guide on Dust Compositions}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Galaxy Astrophysics},
         year = "2014",
        month = "Feb",
          eid = {arXiv:1402.4765},
        pages = {arXiv:1402.4765},
archivePrefix = {arXiv},
       eprint = {1402.4765},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014arXiv1402.4765J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Nicholls17,
       author = {{Nicholls}, David C. and {Sutherland}, Ralph S. and
         {Dopita}, Michael A. and {Kewley}, Lisa J. and {Groves}, Brent A.},
        title = "{Abundance scaling in stars, nebulae and galaxies}",
      journal = {\mnras},
     keywords = {Sun: abundances, Stars: abundances, ISM: abundances, Galaxies: abundances, stars: abundances, galaxies: abundances, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Apr",
       volume = {466},
       number = {4},
        pages = {4403-4422},
          doi = {10.1093/mnras/stw3235},
archivePrefix = {arXiv},
       eprint = {1612.03546},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.466.4403N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Haynes11,
       author = {{Haynes}, Martha P. and {Giovanelli}, Riccardo and {Martin}, Ann M. and
         {Hess}, Kelley M. and {Saintonge}, Am{\'e}lie and
         {Adams}, Elizabeth A.~K. and {Hallenbeck}, Gregory and
         {Hoffman}, G. Lyle and {Huang}, Shan and {Kent}, Brian R. and
         {Koopmann}, Rebecca A. and {Papastergis}, Emmanouil and
         {Stierwalt}, Sabrina and {Balonek}, Thomas J. and {Craig}, David W. and
         {Higdon}, Sarah J.~U. and {Kornreich}, David A. and
         {Miller}, Jeffrey R. and {O'Donoghue}, Aileen A. and
         {Olowin}, Ronald P. and {Rosenberg}, Jessica L. and
         {Spekkens}, Kristine and {Troischt}, Parker and {Wilcots}, Eric M.},
        title = "{The Arecibo Legacy Fast ALFA Survey: The {\ensuremath{\alpha}}.40 H I Source Catalog, Its Characteristics and Their Impact on the Derivation of the H I Mass Function}",
      journal = {\aj},
     keywords = {catalogs, galaxies: distances and redshifts, galaxies: luminosity function, mass function, galaxies: spiral, radio lines: galaxies, surveys, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2011",
        month = "Nov",
       volume = {142},
       number = {5},
          eid = {170},
        pages = {170},
          doi = {10.1088/0004-6256/142/5/170},
archivePrefix = {arXiv},
       eprint = {1109.0027},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011AJ....142..170H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Berlind06,
       author = {{Berlind}, Andreas A. and {Frieman}, Joshua and {Weinberg}, David H. and
         {Blanton}, Michael R. and {Warren}, Michael S. and {Abazajian}, Kevork and
         {Scranton}, Ryan and {Hogg}, David W. and {Scoccimarro}, Roman and
         {Bahcall}, Neta A. and {Brinkmann}, J. and {Gott}, J. Richard, III and
         {Kleinman}, S.~J. and {Krzesinski}, J. and {Lee}, Brian C. and
         {Miller}, Christopher J. and {Nitta}, Atsuko and
         {Schneider}, Donald P. and {Tucker}, Douglas L. and {Zehavi}, Idit and
         {SDSS Collaboration}},
        title = "{Percolation Galaxy Groups and Clusters in the SDSS Redshift Survey: Identification, Catalogs, and the Multiplicity Function}",
      journal = {\apjs},
     keywords = {Galaxies: Clusters: General, Cosmology: Large-Scale Structure of Universe, Astrophysics},
         year = "2006",
        month = "Nov",
       volume = {167},
       number = {1},
        pages = {1-25},
          doi = {10.1086/508170},
archivePrefix = {arXiv},
       eprint = {astro-ph/0601346},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJS..167....1B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Blanton07,
       author = {{Blanton}, Michael R. and {Berlind}, Andreas A.},
        title = "{What Aspects of Galaxy Environment Matter?}",
      journal = {\apj},
     keywords = {Galaxies: Clusters: General, Galaxies: Fundamental Parameters, Galaxies: Statistics, Astrophysics},
         year = "2007",
        month = "Aug",
       volume = {664},
       number = {2},
        pages = {791-803},
          doi = {10.1086/512478},
archivePrefix = {arXiv},
       eprint = {astro-ph/0608353},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...664..791B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Blanc15,
       author = {{Blanc}, Guillermo A. and {Kewley}, Lisa and
         {Vogt}, Fr{\'e}d{\'e}ric P.~A. and {Dopita}, Michael A.},
        title = "{IZI: Inferring the Gas Phase Metallicity (Z) and Ionization Parameter (q) of Ionized Nebulae Using Bayesian Statistics}",
      journal = {\apj},
     keywords = {astrochemistry, galaxies: abundances, galaxies: ISM, H II regions, ISM: abundances, Astrophysics - Astrophysics of Galaxies},
         year = "2015",
        month = "Jan",
       volume = {798},
          eid = {99},
        pages = {99},
          doi = {10.1088/0004-637X/798/2/99},
archivePrefix = {arXiv},
       eprint = {1410.8146},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2015ApJ...798...99B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{Osterbrock06,
       author = {{Osterbrock}, Donald E. and {Ferland}, Gary J.},
        title = "{Astrophysics of gaseous nebulae and active galactic nuclei}",
    booktitle = {Astrophysics of gaseous nebulae and active galactic nuclei, 2nd. ed. by D.E. Osterbrock and G.J. Ferland. Sausalito, CA: University Science Books, 2006},
         year = "2006",
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2006agna.book.....O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Alam15,
       author = {{Alam}, Shadab and {Albareti}, Franco D. and {Allende Prieto}, Carlos and
         {Anders}, F. and {Anderson}, Scott F. and {Anderton}, Timothy and
         {Andrews}, Brett H. and {Armengaud}, Eric and {Aubourg}, {\'E}ric and
         {Bailey}, Stephen and {Basu}, Sarbani and {Bautista}, Julian E. and
         {Beaton}, Rachael L. and {Beers}, Timothy C. and {Bender}, Chad F. and
         {Berlind}, Andreas A. and {Beutler}, Florian and {Bhardwaj}, Vaishali and
         {Bird}, Jonathan C. and {Bizyaev}, Dmitry and {Blake}, Cullen H. and
         {Blanton}, Michael R. and {Blomqvist}, Michael and
         {Bochanski}, John J. and {Bolton}, Adam S. and {Bovy}, Jo and
         {Shelden Bradley}, A. and {Brandt}, W.~N. and {Brauer}, D.~E. and
         {Brinkmann}, J. and {Brown}, Peter J. and {Brownstein}, Joel R. and
         {Burden}, Angela and {Burtin}, Etienne and {Busca}, Nicol{\'a}s G. and
         {Cai}, Zheng and {Capozzi}, Diego and {Carnero Rosell}, Aurelio and
         {Carr}, Michael A. and {Carrera}, Ricardo and {Chambers}, K.~C. and
         {Chaplin}, William James and {Chen}, Yen-Chi and {Chiappini}, Cristina and
         {Chojnowski}, S. Drew and {Chuang}, Chia-Hsun and {Clerc}, Nicolas and
         {Comparat}, Johan and {Covey}, Kevin and {Croft}, Rupert A.~C. and
         {Cuesta}, Antonio J. and {Cunha}, Katia and {da Costa}, Luiz N. and
         {Da Rio}, Nicola and {Davenport}, James R.~A. and {Dawson}, Kyle S. and
         {De Lee}, Nathan and {Delubac}, Timoth{\'e}e and {Deshpande}, Rohit and
         {Dhital}, Saurav and {Dutra-Ferreira}, Let{\'\i}cia and {Dwelly}, Tom and
         {Ealet}, Anne and {Ebelke}, Garrett L. and {Edmondson}, Edward M. and
         {Eisenstein}, Daniel J. and {Ellsworth}, Tristan and
         {Elsworth}, Yvonne and {Epstein}, Courtney R. and {Eracleous}, Michael and
         {Escoffier}, Stephanie and {Esposito}, Massimiliano and
         {Evans}, Michael L. and {Fan}, Xiaohui and {Fern{\'a}ndez-Alvar}, Emma and
         {Feuillet}, Diane and {Filiz Ak}, Nurten and {Finley}, Hayley and
         {Finoguenov}, Alexis and {Flaherty}, Kevin and {Fleming}, Scott W. and
         {Font-Ribera}, Andreu and {Foster}, Jonathan and
         {Frinchaboy}, Peter M. and {Galbraith-Frew}, J.~G. and
         {Garc{\'\i}a}, Rafael A. and {Garc{\'\i}a-Hern{\'a}ndez}, D.~A. and
         {Garc{\'\i}a P{\'e}rez}, Ana E. and {Gaulme}, Patrick and {Ge}, Jian and
         {G{\'e}nova-Santos}, R. and {Georgakakis}, A. and {Ghezzi}, Luan and
         {Gillespie}, Bruce A. and {Girardi}, L{\'e}o and {Goddard}, Daniel and
         {Gontcho}, Satya Gontcho A. and {Gonz{\'a}lez Hern{\'a}ndez}, Jonay I. and
         {Grebel}, Eva K. and {Green}, Paul J. and {Grieb}, Jan Niklas and
         {Grieves}, Nolan and {Gunn}, James E. and {Guo}, Hong and
         {Harding}, Paul and {Hasselquist}, Sten and {Hawley}, Suzanne L. and
         {Hayden}, Michael and {Hearty}, Fred R. and {Hekker}, Saskia and
         {Ho}, Shirley and {Hogg}, David W. and {Holley-Bockelmann}, Kelly and
         {Holtzman}, Jon A. and {Honscheid}, Klaus and {Huber}, Daniel and
         {Huehnerhoff}, Joseph and {Ivans}, Inese I. and {Jiang}, Linhua and
         {Johnson}, Jennifer A. and {Kinemuchi}, Karen and {Kirkby}, David and
         {Kitaura}, Francisco and {Klaene}, Mark A. and {Knapp}, Gillian R. and
         {Kneib}, Jean-Paul and {Koenig}, Xavier P. and {Lam}, Charles R. and
         {Lan}, Ting-Wen and {Lang}, Dustin and {Laurent}, Pierre and
         {Le Goff}, Jean-Marc and {Leauthaud}, Alexie and {Lee}, Khee-Gan and
         {Lee}, Young Sun and {Licquia}, Timothy C. and {Liu}, Jian and
         {Long}, Daniel C. and {L{\'o}pez-Corredoira}, Mart{\'\i}n and
         {Lorenzo-Oliveira}, Diego and {Lucatello}, Sara and {Lundgren}, Britt and
         {Lupton}, Robert H. and {Mack}, Claude E., III and
         {Mahadevan}, Suvrath and {Maia}, Marcio A.~G. and
         {Majewski}, Steven R. and {Malanushenko}, Elena and
         {Malanushenko}, Viktor and {Manchado}, A. and {Manera}, Marc and
         {Mao}, Qingqing and {Maraston}, Claudia and {Marchwinski}, Robert C. and
         {Margala}, Daniel and {Martell}, Sarah L. and {Martig}, Marie and
         {Masters}, Karen L. and {Mathur}, Savita and {McBride}, Cameron K. and
         {McGehee}, Peregrine M. and {McGreer}, Ian D. and
         {McMahon}, Richard G. and {M{\'e}nard}, Brice and
         {Menzel}, Marie-Luise and {Merloni}, Andrea and
         {M{\'e}sz{\'a}ros}, Szabolcs and {Miller}, Adam A. and
         {Miralda-Escud{\'e}}, Jordi and {Miyatake}, Hironao and
         {Montero-Dorta}, Antonio D. and {More}, Surhud and {Morganson}, Eric and
         {Morice-Atkinson}, Xan and {Morrison}, Heather L. and
         {Mosser}, Ben{\^o}it and {Muna}, Demitri and {Myers}, Adam D. and {Nand
        ra}, Kirpal and {Newman}, Jeffrey A. and {Neyrinck}, Mark and
         {Nguyen}, Duy Cuong and {Nichol}, Robert C. and {Nidever}, David L. and
         {Noterdaeme}, Pasquier and {Nuza}, Sebasti{\'a}n E. and
         {O'Connell}, Julia E. and {O'Connell}, Robert W. and {O'Connell}, Ross and
         {Ogando}, Ricardo L.~C. and {Olmstead}, Matthew D. and
         {Oravetz}, Audrey E. and {Oravetz}, Daniel J. and {Osumi}, Keisuke and
         {Owen}, Russell and {Padgett}, Deborah L. and {Padmanabhan}, Nikhil and
         {Paegert}, Martin and {Palanque-Delabrouille}, Nathalie and
         {Pan}, Kaike and {Parejko}, John K. and {P{\^a}ris}, Isabelle and
         {Park}, Changbom and {Pattarakijwanich}, Petchara and
         {Pellejero-Ibanez}, M. and {Pepper}, Joshua and {Percival}, Will J. and
         {P{\'e}rez-Fournon}, Ismael and {Ṕrez-Ra`fols}, Ignasi and
         {Petitjean}, Patrick and {Pieri}, Matthew M. and
         {Pinsonneault}, Marc H. and {Porto de Mello}, Gustavo F. and
         {Prada}, Francisco and {Prakash}, Abhishek and
         {Price-Whelan}, Adrian M. and {Protopapas}, Pavlos and
         {Raddick}, M. Jordan and {Rahman}, Mubdi and {Reid}, Beth A. and
         {Rich}, James and {Rix}, Hans-Walter and {Robin}, Annie C. and
         {Rockosi}, Constance M. and {Rodrigues}, Tha{\'\i}se S. and
         {Rodr{\'\i}guez-Torres}, Sergio and {Roe}, Natalie A. and
         {Ross}, Ashley J. and {Ross}, Nicholas P. and {Rossi}, Graziano and
         {Ruan}, John J. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and
         {Rykoff}, Eli S. and {Salazar-Albornoz}, Salvador and {Salvato}, Mara and
         {Samushia}, Lado and {S{\'a}nchez}, Ariel G. and
         {Santiago}, Bas{\'\i}lio and {Sayres}, Conor and
         {Schiavon}, Ricardo P. and {Schlegel}, David J. and
         {Schmidt}, Sarah J. and {Schneider}, Donald P. and
         {Schultheis}, Mathias and {Schwope}, Axel D. and {Sc{\'o}ccola}, C.~G. and
         {Scott}, Caroline and {Sellgren}, Kris and {Seo}, Hee-Jong and
         {Serenelli}, Aldo and {Shane}, Neville and {Shen}, Yue and
         {Shetrone}, Matthew and {Shu}, Yiping and {Silva Aguirre}, V. and
         {Sivarani}, Thirupathi and {Skrutskie}, M.~F. and {Slosar}, An{\v{z}}e and
         {Smith}, Verne V. and {Sobreira}, Fl{\'a}via and {Souto}, Diogo and
         {Stassun}, Keivan G. and {Steinmetz}, Matthias and {Stello}, Dennis and
         {Strauss}, Michael A. and {Streblyanska}, Alina and {Suzuki}, Nao and
         {Swanson}, Molly E.~C. and {Tan}, Jonathan C. and {Tayar}, Jamie and
         {Terrien}, Ryan C. and {Thakar}, Aniruddha R. and {Thomas}, Daniel and
         {Thomas}, Neil and {Thompson}, Benjamin A. and {Tinker}, Jeremy L. and
         {Tojeiro}, Rita and {Troup}, Nicholas W. and
         {Vargas-Maga{\~n}a}, Mariana and {Vazquez}, Jose A. and {Verde}, Licia and
         {Viel}, Matteo and {Vogt}, Nicole P. and {Wake}, David A. and
         {Wang}, Ji and {Weaver}, Benjamin A. and {Weinberg}, David H. and
         {Weiner}, Benjamin J. and {White}, Martin and {Wilson}, John C. and
         {Wisniewski}, John P. and {Wood-Vasey}, W.~M. and {Ye`che}, Christophe and
         {York}, Donald G. and {Zakamska}, Nadia L. and {Zamora}, O. and
         {Zasowski}, Gail and {Zehavi}, Idit and {Zhao}, Gong-Bo and
         {Zheng}, Zheng and {Zhou}, Xu and {Zhou}, Zhimin and {Zou}, Hu and
         {Zhu}, Guangtun},
        title = "{The Eleventh and Twelfth Data Releases of the Sloan Digital Sky Survey: Final Data from SDSS-III}",
      journal = {The Astrophysical Journal Supplement Series},
     keywords = {atlases, catalogs, surveys, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = "2015",
        month = "Jul",
       volume = {219},
          eid = {12},
        pages = {12},
          doi = {10.1088/0067-0049/219/1/12},
archivePrefix = {arXiv},
       eprint = {1501.00963},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2015ApJS..219...12A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Hood18,
       author = {{Hood}, Callie E. and {Kannappan}, Sheila J. and {Stark}, David V. and
         {Dell'Antonio}, Ian P. and {Moffett}, Amanda J. and
         {Eckert}, Kathleen D. and {Norris}, Mark A. and {Hendel}, David},
        title = "{The Origin of Faint Tidal Features around Galaxies in the RESOLVE Survey}",
      journal = {\apj},
     keywords = {galaxies: evolution, galaxies: interactions, Astrophysics - Astrophysics of Galaxies},
         year = "2018",
        month = "Apr",
       volume = {857},
          eid = {144},
        pages = {144},
          doi = {10.3847/1538-4357/aab719},
archivePrefix = {arXiv},
       eprint = {1803.05447},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2018ApJ...857..144H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bar17,
       author = {{B{\"a}r}, Rudolf E. and {Weigel}, Anna K. and {Sartori}, Lia F. and
         {Oh}, Kyuseok and {Koss}, Michael and {Schawinski}, Kevin},
        title = "{Active galactic nuclei from He II: a more complete census of AGN in SDSS galaxies yields a new population of low-luminosity AGN in highly star-forming galaxies}",
      journal = {\mnras},
     keywords = {galaxies: active, galaxies: evolution, galaxies: nuclei, galaxies: Seyfert, galaxies: star formation, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2017",
        month = "Apr",
       volume = {466},
        pages = {2879-2887},
          doi = {10.1093/mnras/stw3283},
archivePrefix = {arXiv},
       eprint = {1612.04815},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2017MNRAS.466.2879B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


